Untrained CNNs Exceed Backpropagation in V1 Alignment at High Evaluation Resolution: A Systematic RSA Comparison of Four Learning Rules Against Human fMRI

Revision note: the V1 result reported here is not robust to the analysis choices examined in arXiv:2611.15533; see page 1. We compare four learning rules (backpropagation (BP), feedback alignment (FA), predictive coding (PC), and spike-timing-dependent plasticity (STDP)) in identical convolutional networks against human fMRI from THINGS-fMRI (720 stimuli, 3 subjects) using representational similarity analysis (RSA), together with an untrained random-weights baseline that isolates the contribution of architecture. Models are trained on 32 px CIFAR-10 and evaluated at 224 px; results are averaged across 5 seeds, with uncertainty from resampling stimuli. At V1, the untrained baseline exceeds BP rho = 0.053$ vs. $0.022$; rho = +0.031$, 95% CI $[0.019, 0.043]$), and the same holds at V2. This advantage depends on the evaluation resolution: in the 5-seed model set of the resolution study (gap $+0.030$ at 224 px), it vanishes when the models are evaluated at their 32 px training resolution rho = -0.001, 95% CI $[-0.011, 0.009]$; arXiv:2608.12408). At LOC, BP, PC and STDP exceed the untrained baseline, FA is borderline, and the trained rules do not differ from each other. At IT, no two conditions can be distinguished at the low reliability of the data (leave-one-subject-out lower bound 0.021). FA has the lowest alignment at V1. At V1, an untrained network thus matches BP at the training resolution and exceeds it at 224 px; learning-rule differences are resolvable only at an intermediate area.

==> numbers.tex <==
% generated by scripts/paper_v3/make_macros.py -- do not edit
\makeatletter
\expandafter\def\csname nv@acc.bp\endcsname{75.0}
\expandafter\def\csname nv@acc.fa\endcsname{38.8}
\expandafter\def\csname nv@acc.ntest\endcsname{10{,}000}
\expandafter\def\csname nv@acc.pc\endcsname{56.7}
\expandafter\def\csname nv@acc.rnd\endcsname{10.0}
\expandafter\def\csname nv@acc.stdp\endcsname{57.4}
\expandafter\def\csname nv@agree.0102.IT.all\endcsname{0.066}
\expandafter\def\csname nv@agree.0102.IT.cr\endcsname{0.029}
\expandafter\def\csname nv@agree.0102.LOC.all\endcsname{0.062}
\expandafter\def\csname nv@agree.0102.LOC.cr\endcsname{0.023}
\expandafter\def\csname nv@agree.0102.V1.all\endcsname{0.115}
\expandafter\def\csname nv@agree.0102.V1.cr\endcsname{0.097}
\expandafter\def\csname nv@agree.0102.V2.all\endcsname{0.063}
\expandafter\def\csname nv@agree.0102.V2.cr\endcsname{0.041}
\expandafter\def\csname nv@agree.0103.IT.all\endcsname{0.009}
\expandafter\def\csname nv@agree.0103.IT.cr\endcsname{0.010}
\expandafter\def\csname nv@agree.0103.LOC.all\endcsname{0.008}
\expandafter\def\csname nv@agree.0103.LOC.cr\endcsname{0.009}
\expandafter\def\csname nv@agree.0103.V1.all\endcsname{0.014}
\expandafter\def\csname nv@agree.0103.V1.cr\endcsname{0.017}
\expandafter\def\csname nv@agree.0103.V2.all\endcsname{0.007}
\expandafter\def\csname nv@agree.0103.V2.cr\endcsname{0.007}
\expandafter\def\csname nv@agree.0203.IT.all\endcsname{0.007}
\expandafter\def\csname nv@agree.0203.IT.cr\endcsname{0.010}
\expandafter\def\csname nv@agree.0203.LOC.all\endcsname{0.009}
\expandafter\def\csname nv@agree.0203.LOC.cr\endcsname{0.009}
\expandafter\def\csname nv@agree.0203.V1.all\endcsname{0.014}
\expandafter\def\csname nv@agree.0203.V1.cr\endcsname{0.014}
\expandafter\def\csname nv@agree.0203.V2.all\endcsname{0.006}
\expandafter\def\csname nv@agree.0203.V2.cr\endcsname{0.006}
\expandafter\def\csname nv@bl.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@bl.bp.LOC\endcsname{0.012}
\expandafter\def\csname nv@bl.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@bl.bp.V2\endcsname{0.012}
\expandafter\def\csname nv@bl.bp.nmatch\endcsname{3}
\expandafter\def\csname nv@bl.fa.IT\endcsname{0.008}
\expandafter\def\csname nv@bl.fa.LOC\endcsname{0.005}
\expandafter\def\csname nv@bl.fa.V1\endcsname{0.020}
\expandafter\def\csname nv@bl.fa.V2\endcsname{0.014}
\expandafter\def\csname nv@bl.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@bl.pc.LOC\endcsname{0.005}
\expandafter\def\csname nv@bl.pc.V1\endcsname{0.015}
\expandafter\def\csname nv@bl.pc.V2\endcsname{0.013}
\expandafter\def\csname nv@bl.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@bl.rnd.LOC\endcsname{-0.002}
\expandafter\def\csname nv@bl.rnd.V1\endcsname{0.102}
\expandafter\def\csname nv@bl.rnd.V2\endcsname{0.061}
\expandafter\def\csname nv@bl.stdp.IT\endcsname{0.009}
\expandafter\def\csname nv@bl.stdp.LOC\endcsname{0.007}
\expandafter\def\csname nv@bl.stdp.V1\endcsname{0.027}
\expandafter\def\csname nv@bl.stdp.V2\endcsname{0.018}
\expandafter\def\csname nv@blfix.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@blfix.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@blfix.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@blfix.bp.V2\endcsname{0.012}
\expandafter\def\csname nv@blfix.fa.IT\endcsname{0.008}
\expandafter\def\csname nv@blfix.fa.LOC\endcsname{0.004}
\expandafter\def\csname nv@blfix.fa.V1\endcsname{0.009}
\expandafter\def\csname nv@blfix.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@blfix.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@blfix.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@blfix.pc.V1\endcsname{0.012}
\expandafter\def\csname nv@blfix.pc.V2\endcsname{0.006}
\expandafter\def\csname nv@blfix.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@blfix.rnd.LOC\endcsname{-0.003}
\expandafter\def\csname nv@blfix.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@blfix.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@blfix.stdp.IT\endcsname{0.009}
\expandafter\def\csname nv@blfix.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@blfix.stdp.V1\endcsname{0.027}
\expandafter\def\csname nv@blfix.stdp.V2\endcsname{0.015}
\expandafter\def\csname nv@bootseed\endcsname{20261002}
\expandafter\def\csname nv@border.cr.d\endcsname{+0.0044}
\expandafter\def\csname nv@border.cr.hi\endcsname{0.0102}
\expandafter\def\csname nv@border.cr.lo\endcsname{-0.0011}
\expandafter\def\csname nv@border.d\endcsname{+0.0050}
\expandafter\def\csname nv@border.hi\endcsname{0.0102}
\expandafter\def\csname nv@border.lo\endcsname{0.0001}
\expandafter\def\csname nv@cal.B\endcsname{+0.041}
\expandafter\def\csname nv@cal.B.n\endcsname{5/5}
\expandafter\def\csname nv@cal.D\endcsname{+0.033}
\expandafter\def\csname nv@cal.D.n\endcsname{5/5}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT.4\endcsname{+0.0012}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT.hi.4\endcsname{0.0094}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.IT.lo.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC.4\endcsname{+0.0070}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC.hi.4\endcsname{0.0167}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.LOC.lo.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1\endcsname{+0.020}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1.4\endcsname{+0.0199}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1.hi\endcsname{0.027}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1.hi.4\endcsname{0.0269}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V1.lo.4\endcsname{0.0132}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2.4\endcsname{+0.0129}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2.hi.4\endcsname{0.0186}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.bp.fa.V2.lo.4\endcsname{0.0077}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT.4\endcsname{+0.0017}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT.hi.4\endcsname{0.0100}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.IT.lo.4\endcsname{-0.0063}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC.4\endcsname{+0.0064}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC.hi.4\endcsname{0.0160}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.LOC.lo.4\endcsname{-0.0025}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1.4\endcsname{+0.0151}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1.hi.4\endcsname{0.0216}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V1.lo.4\endcsname{0.0091}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2.4\endcsname{+0.0094}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2.hi\endcsname{0.015}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2.hi.4\endcsname{0.0145}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.mr.all.bn.bp.pc.V2.lo.4\endcsname{0.0049}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT.4\endcsname{+0.0049}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT.hi.4\endcsname{0.0187}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.IT.lo.4\endcsname{-0.0082}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC\endcsname{+0.018}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC.4\endcsname{+0.0177}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC.hi\endcsname{0.032}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC.hi.4\endcsname{0.0320}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC.lo\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.LOC.lo.4\endcsname{0.0036}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1\endcsname{-0.044}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1.4\endcsname{-0.0441}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1.hi\endcsname{-0.027}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1.hi.4\endcsname{-0.0268}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1.lo\endcsname{-0.061}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V1.lo.4\endcsname{-0.0613}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2.4\endcsname{-0.0264}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2.hi\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2.hi.4\endcsname{-0.0120}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2.lo\endcsname{-0.041}
\expandafter\def\csname nv@d.mr.all.bn.bp.rnd.V2.lo.4\endcsname{-0.0413}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT.hi.4\endcsname{0.0067}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.IT.lo.4\endcsname{-0.0081}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC.4\endcsname{+0.0069}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC.hi.4\endcsname{0.0166}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.LOC.lo.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1.hi.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V1.lo.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2.hi.4\endcsname{0.0007}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.bp.stdp.V2.lo.4\endcsname{-0.0081}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT.hi.4\endcsname{0.0073}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.IT.lo.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC.4\endcsname{-0.0070}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC.hi.4\endcsname{0.0019}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.LOC.lo.4\endcsname{-0.0167}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1.4\endcsname{-0.0199}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1.hi\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1.hi.4\endcsname{-0.0132}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1.lo\endcsname{-0.027}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V1.lo.4\endcsname{-0.0269}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2.4\endcsname{-0.0129}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2.hi.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.bn.fa.bp.V2.lo.4\endcsname{-0.0186}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT.hi.4\endcsname{0.0067}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.IT.lo.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.LOC.lo.4\endcsname{-0.0043}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1.hi.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V1.lo.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2.hi.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.fa.pc.V2.lo.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT.hi.4\endcsname{0.0158}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.IT.lo.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC.4\endcsname{+0.0107}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC.hi.4\endcsname{0.0219}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC.lo\endcsname{0.000}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.LOC.lo.4\endcsname{0.0002}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1\endcsname{-0.064}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1.4\endcsname{-0.0639}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1.hi\endcsname{-0.045}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1.hi.4\endcsname{-0.0449}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1.lo\endcsname{-0.083}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V1.lo.4\endcsname{-0.0832}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2\endcsname{-0.039}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2.4\endcsname{-0.0394}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2.hi\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2.hi.4\endcsname{-0.0241}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.mr.all.bn.fa.rnd.V2.lo.4\endcsname{-0.0553}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT.hi.4\endcsname{0.0040}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.IT.lo.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC.hi.4\endcsname{0.0062}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.LOC.lo.4\endcsname{-0.0056}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1.4\endcsname{-0.0257}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1.hi.4\endcsname{-0.0188}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1.lo\endcsname{-0.033}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V1.lo.4\endcsname{-0.0334}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2.4\endcsname{-0.0167}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2.hi\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2.hi.4\endcsname{-0.0118}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.bn.fa.stdp.V2.lo.4\endcsname{-0.0222}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT.hi.4\endcsname{0.0063}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.IT.lo.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC.4\endcsname{-0.0064}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC.hi.4\endcsname{0.0025}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.LOC.lo.4\endcsname{-0.0160}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1.hi.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V1.lo.4\endcsname{-0.0216}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2.hi.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.bn.pc.bp.V2.lo.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT.hi.4\endcsname{0.0052}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.IT.lo.4\endcsname{-0.0067}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC.4\endcsname{+0.0006}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC.hi.4\endcsname{0.0043}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.LOC.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1.4\endcsname{+0.0048}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1.hi.4\endcsname{0.0078}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V1.lo.4\endcsname{0.0017}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2\endcsname{+0.003}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2.4\endcsname{+0.0035}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2.hi.4\endcsname{0.0059}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2.lo\endcsname{0.001}
\expandafter\def\csname nv@d.mr.all.bn.pc.fa.V2.lo.4\endcsname{0.0011}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT.4\endcsname{+0.0032}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT.hi.4\endcsname{0.0145}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.IT.lo.4\endcsname{-0.0082}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC.4\endcsname{+0.0113}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC.hi.4\endcsname{0.0212}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.LOC.lo.4\endcsname{0.0015}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1\endcsname{-0.059}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1.4\endcsname{-0.0591}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1.hi\endcsname{-0.042}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1.hi.4\endcsname{-0.0418}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1.lo\endcsname{-0.076}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V1.lo.4\endcsname{-0.0761}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2\endcsname{-0.036}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2.4\endcsname{-0.0359}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2.hi\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2.hi.4\endcsname{-0.0222}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2.lo\endcsname{-0.050}
\expandafter\def\csname nv@d.mr.all.bn.pc.rnd.V2.lo.4\endcsname{-0.0501}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT.4\endcsname{-0.0022}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT.hi.4\endcsname{0.0028}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.IT.lo.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC.hi.4\endcsname{0.0053}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.LOC.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1.4\endcsname{-0.0209}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1.hi.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1.lo\endcsname{-0.027}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V1.lo.4\endcsname{-0.0268}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2.4\endcsname{-0.0133}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2.hi.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.all.bn.pc.stdp.V2.lo.4\endcsname{-0.0179}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT.hi.4\endcsname{0.0082}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.IT.lo.4\endcsname{-0.0187}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC.4\endcsname{-0.0177}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC.hi.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC.lo\endcsname{-0.032}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.LOC.lo.4\endcsname{-0.0320}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1\endcsname{+0.044}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1.4\endcsname{+0.0441}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1.hi\endcsname{0.061}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1.hi.4\endcsname{0.0613}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1.lo\endcsname{0.027}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V1.lo.4\endcsname{0.0268}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2\endcsname{+0.026}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2.4\endcsname{+0.0264}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2.hi\endcsname{0.041}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2.hi.4\endcsname{0.0413}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2.lo\endcsname{0.012}
\expandafter\def\csname nv@d.mr.all.bn.rnd.bp.V2.lo.4\endcsname{0.0120}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT.hi.4\endcsname{0.0074}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.IT.lo.4\endcsname{-0.0158}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC.4\endcsname{-0.0107}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC.hi.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.LOC.lo.4\endcsname{-0.0219}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1\endcsname{+0.064}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1.4\endcsname{+0.0639}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1.hi\endcsname{0.083}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1.hi.4\endcsname{0.0832}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1.lo\endcsname{0.045}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V1.lo.4\endcsname{0.0449}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2\endcsname{+0.039}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2.4\endcsname{+0.0394}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2.hi\endcsname{0.055}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2.hi.4\endcsname{0.0553}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2.lo\endcsname{0.024}
\expandafter\def\csname nv@d.mr.all.bn.rnd.fa.V2.lo.4\endcsname{0.0241}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT.hi.4\endcsname{0.0082}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.IT.lo.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC.4\endcsname{-0.0113}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC.hi.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.LOC.lo.4\endcsname{-0.0212}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1\endcsname{+0.059}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1.4\endcsname{+0.0591}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1.hi\endcsname{0.076}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1.hi.4\endcsname{0.0761}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1.lo\endcsname{0.042}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V1.lo.4\endcsname{0.0418}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2\endcsname{+0.036}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2.4\endcsname{+0.0359}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2.hi\endcsname{0.050}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2.hi.4\endcsname{0.0501}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2.lo\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.bn.rnd.pc.V2.lo.4\endcsname{0.0222}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT.hi.4\endcsname{0.0052}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.IT.lo.4\endcsname{-0.0167}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC.4\endcsname{-0.0108}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC.hi.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.LOC.lo.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1\endcsname{+0.038}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1.4\endcsname{+0.0382}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1.hi\endcsname{0.055}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1.hi.4\endcsname{0.0547}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1.lo\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V1.lo.4\endcsname{0.0224}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2\endcsname{+0.023}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2.4\endcsname{+0.0226}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2.hi\endcsname{0.037}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2.hi.4\endcsname{0.0366}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.bn.rnd.stdp.V2.lo.4\endcsname{0.0089}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT.hi.4\endcsname{0.0081}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.IT.lo.4\endcsname{-0.0067}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC.4\endcsname{-0.0069}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC.hi.4\endcsname{0.0020}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.LOC.lo.4\endcsname{-0.0166}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1.4\endcsname{+0.0058}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1.hi.4\endcsname{0.0115}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V1.lo.4\endcsname{0.0001}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2\endcsname{+0.004}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2.4\endcsname{+0.0038}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2.hi.4\endcsname{0.0081}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.bn.stdp.bp.V2.lo.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT.hi.4\endcsname{0.0077}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.IT.lo.4\endcsname{-0.0040}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC.hi.4\endcsname{0.0056}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.LOC.lo.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1\endcsname{+0.026}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1.4\endcsname{+0.0257}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1.hi\endcsname{0.033}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1.hi.4\endcsname{0.0334}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V1.lo.4\endcsname{0.0188}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2.4\endcsname{+0.0167}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2.hi.4\endcsname{0.0222}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2.lo\endcsname{0.012}
\expandafter\def\csname nv@d.mr.all.bn.stdp.fa.V2.lo.4\endcsname{0.0118}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT.4\endcsname{+0.0022}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT.hi.4\endcsname{0.0077}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.IT.lo.4\endcsname{-0.0028}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.LOC.lo.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1\endcsname{+0.021}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1.4\endcsname{+0.0209}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1.hi\endcsname{0.027}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1.hi.4\endcsname{0.0268}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1.lo\endcsname{0.015}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V1.lo.4\endcsname{0.0151}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2.4\endcsname{+0.0133}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2.hi.4\endcsname{0.0179}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.bn.stdp.pc.V2.lo.4\endcsname{0.0090}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT.4\endcsname{+0.0053}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT.hi.4\endcsname{0.0167}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.IT.lo.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC.4\endcsname{+0.0108}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC.hi\endcsname{0.020}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC.hi.4\endcsname{0.0202}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.LOC.lo.4\endcsname{0.0012}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1\endcsname{-0.038}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1.4\endcsname{-0.0382}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1.hi\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1.hi.4\endcsname{-0.0224}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V1.lo.4\endcsname{-0.0547}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2.hi.4\endcsname{-0.0089}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2.lo\endcsname{-0.037}
\expandafter\def\csname nv@d.mr.all.bn.stdp.rnd.V2.lo.4\endcsname{-0.0366}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT.4\endcsname{+0.0017}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT.hi.4\endcsname{0.0106}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.IT.lo.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC.4\endcsname{+0.0060}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC.hi.4\endcsname{0.0161}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.LOC.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1\endcsname{+0.022}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1.4\endcsname{+0.0217}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1.hi\endcsname{0.030}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1.hi.4\endcsname{0.0296}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1.lo\endcsname{0.014}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V1.lo.4\endcsname{0.0143}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2.4\endcsname{+0.0145}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2.hi.4\endcsname{0.0211}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.ref.bp.fa.V2.lo.4\endcsname{0.0087}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT.hi.4\endcsname{0.0092}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.IT.lo.4\endcsname{-0.0112}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC.4\endcsname{+0.0056}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC.hi.4\endcsname{0.0180}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.LOC.lo.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1.hi.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1.lo\endcsname{-0.037}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V1.lo.4\endcsname{-0.0368}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2.hi.4\endcsname{0.0029}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.ref.bp.pc.V2.lo.4\endcsname{-0.0213}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT.4\endcsname{+0.0055}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT.hi.4\endcsname{0.0190}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.IT.lo.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC\endcsname{+0.017}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC.4\endcsname{+0.0167}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC.hi\endcsname{0.031}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC.hi.4\endcsname{0.0314}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.LOC.lo.4\endcsname{0.0026}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1\endcsname{-0.042}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1.4\endcsname{-0.0420}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1.hi\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1.hi.4\endcsname{-0.0241}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V1.lo.4\endcsname{-0.0594}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2\endcsname{-0.025}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2.4\endcsname{-0.0249}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2.hi\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2.hi.4\endcsname{-0.0107}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2.lo\endcsname{-0.040}
\expandafter\def\csname nv@d.mr.all.ref.bp.rnd.V2.lo.4\endcsname{-0.0397}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT.4\endcsname{+0.0014}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT.hi.4\endcsname{0.0120}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.IT.lo.4\endcsname{-0.0096}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC.4\endcsname{+0.0058}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC.hi.4\endcsname{0.0170}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.LOC.lo.4\endcsname{-0.0055}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1\endcsname{-0.031}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1.4\endcsname{-0.0307}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1.hi.4\endcsname{-0.0190}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1.lo\endcsname{-0.042}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V1.lo.4\endcsname{-0.0419}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2.4\endcsname{-0.0173}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2.hi.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2.lo\endcsname{-0.027}
\expandafter\def\csname nv@d.mr.all.ref.bp.stdp.V2.lo.4\endcsname{-0.0271}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT.hi.4\endcsname{0.0074}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.IT.lo.4\endcsname{-0.0106}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.LOC.lo.4\endcsname{-0.0161}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1.4\endcsname{-0.0217}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1.hi.4\endcsname{-0.0143}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1.lo\endcsname{-0.030}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V1.lo.4\endcsname{-0.0296}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2.hi.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.ref.fa.bp.V2.lo.4\endcsname{-0.0211}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT.hi.4\endcsname{0.0065}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.IT.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC.hi.4\endcsname{0.0092}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.LOC.lo.4\endcsname{-0.0098}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1\endcsname{-0.044}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1.4\endcsname{-0.0443}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1.hi\endcsname{-0.031}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1.hi.4\endcsname{-0.0305}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V1.lo.4\endcsname{-0.0588}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2.4\endcsname{-0.0240}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2.hi\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2.hi.4\endcsname{-0.0118}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.mr.all.ref.fa.pc.V2.lo.4\endcsname{-0.0356}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT.4\endcsname{+0.0038}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT.hi.4\endcsname{0.0155}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.IT.lo.4\endcsname{-0.0072}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC.4\endcsname{+0.0107}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC.hi.4\endcsname{0.0220}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC.lo\endcsname{0.000}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.LOC.lo.4\endcsname{0.0003}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1\endcsname{-0.064}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1.4\endcsname{-0.0637}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1.hi\endcsname{-0.045}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1.hi.4\endcsname{-0.0449}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1.lo\endcsname{-0.083}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V1.lo.4\endcsname{-0.0828}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2\endcsname{-0.039}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2.4\endcsname{-0.0394}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2.hi\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2.hi.4\endcsname{-0.0243}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.mr.all.ref.fa.rnd.V2.lo.4\endcsname{-0.0552}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT.hi.4\endcsname{0.0091}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.IT.lo.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC.hi.4\endcsname{0.0077}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.LOC.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1\endcsname{-0.052}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1.4\endcsname{-0.0524}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1.hi\endcsname{-0.040}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1.hi.4\endcsname{-0.0395}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1.lo\endcsname{-0.066}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V1.lo.4\endcsname{-0.0662}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2\endcsname{-0.032}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2.4\endcsname{-0.0318}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2.hi\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2.hi.4\endcsname{-0.0213}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2.lo\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.all.ref.fa.stdp.V2.lo.4\endcsname{-0.0427}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT.hi.4\endcsname{0.0112}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.IT.lo.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC.4\endcsname{-0.0056}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC.hi.4\endcsname{0.0076}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.LOC.lo.4\endcsname{-0.0180}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1\endcsname{+0.023}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1.4\endcsname{+0.0226}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1.hi\endcsname{0.037}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1.hi.4\endcsname{0.0368}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V1.lo.4\endcsname{0.0090}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2.4\endcsname{+0.0094}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2.hi.4\endcsname{0.0213}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.pc.bp.V2.lo.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT.4\endcsname{+0.0021}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.IT.lo.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC.hi.4\endcsname{0.0098}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.LOC.lo.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1\endcsname{+0.044}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1.4\endcsname{+0.0443}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1.hi\endcsname{0.059}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1.hi.4\endcsname{0.0588}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1.lo\endcsname{0.031}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V1.lo.4\endcsname{0.0305}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2\endcsname{+0.024}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2.4\endcsname{+0.0240}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2.hi.4\endcsname{0.0356}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2.lo\endcsname{0.012}
\expandafter\def\csname nv@d.mr.all.ref.pc.fa.V2.lo.4\endcsname{0.0118}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT.4\endcsname{+0.0059}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT.hi.4\endcsname{0.0151}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.IT.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC.4\endcsname{+0.0111}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC.hi.4\endcsname{0.0192}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.LOC.lo.4\endcsname{0.0026}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1.4\endcsname{-0.0194}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1.hi.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1.lo\endcsname{-0.029}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V1.lo.4\endcsname{-0.0286}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2.4\endcsname{-0.0154}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2.hi.4\endcsname{-0.0067}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.all.ref.pc.rnd.V2.lo.4\endcsname{-0.0239}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT.hi.4\endcsname{0.0066}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.IT.lo.4\endcsname{-0.0025}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.LOC.lo.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1.4\endcsname{-0.0081}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1.hi.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V1.lo.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2.hi.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.all.ref.pc.stdp.V2.lo.4\endcsname{-0.0132}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT.4\endcsname{-0.0055}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT.hi.4\endcsname{0.0076}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.IT.lo.4\endcsname{-0.0190}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC.4\endcsname{-0.0167}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC.hi.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC.lo\endcsname{-0.031}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.LOC.lo.4\endcsname{-0.0314}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1\endcsname{+0.042}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1.4\endcsname{+0.0420}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1.hi\endcsname{0.059}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1.hi.4\endcsname{0.0594}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1.lo\endcsname{0.024}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V1.lo.4\endcsname{0.0241}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2\endcsname{+0.025}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2.4\endcsname{+0.0249}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2.hi\endcsname{0.040}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2.hi.4\endcsname{0.0397}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2.lo\endcsname{0.011}
\expandafter\def\csname nv@d.mr.all.ref.rnd.bp.V2.lo.4\endcsname{0.0107}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT.hi.4\endcsname{0.0072}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.IT.lo.4\endcsname{-0.0155}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC.4\endcsname{-0.0107}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC.hi.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.LOC.lo.4\endcsname{-0.0220}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1\endcsname{+0.064}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1.4\endcsname{+0.0637}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1.hi\endcsname{0.083}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1.hi.4\endcsname{0.0828}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1.lo\endcsname{0.045}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V1.lo.4\endcsname{0.0449}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2\endcsname{+0.039}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2.4\endcsname{+0.0394}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2.hi\endcsname{0.055}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2.hi.4\endcsname{0.0552}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2.lo\endcsname{0.024}
\expandafter\def\csname nv@d.mr.all.ref.rnd.fa.V2.lo.4\endcsname{0.0243}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.IT.lo.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC.4\endcsname{-0.0111}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC.hi.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.LOC.lo.4\endcsname{-0.0192}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1\endcsname{+0.019}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1.4\endcsname{+0.0194}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1.hi\endcsname{0.029}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1.hi.4\endcsname{0.0286}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V1.lo.4\endcsname{0.0100}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2.4\endcsname{+0.0154}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2.hi\endcsname{0.024}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2.hi.4\endcsname{0.0239}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.rnd.pc.V2.lo.4\endcsname{0.0067}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.IT.lo.4\endcsname{-0.0125}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC.4\endcsname{-0.0108}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC.hi.4\endcsname{-0.0022}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.LOC.lo.4\endcsname{-0.0194}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1.4\endcsname{+0.0113}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1.hi.4\endcsname{0.0215}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V1.lo.4\endcsname{0.0000}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2.4\endcsname{+0.0076}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2.hi.4\endcsname{0.0174}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.rnd.stdp.V2.lo.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT.hi.4\endcsname{0.0096}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.IT.lo.4\endcsname{-0.0120}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC.hi.4\endcsname{0.0055}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.LOC.lo.4\endcsname{-0.0170}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1\endcsname{+0.031}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1.4\endcsname{+0.0307}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1.hi\endcsname{0.042}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1.hi.4\endcsname{0.0419}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V1.lo.4\endcsname{0.0190}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2.4\endcsname{+0.0173}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2.hi\endcsname{0.027}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2.hi.4\endcsname{0.0271}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.stdp.bp.V2.lo.4\endcsname{0.0074}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT.hi.4\endcsname{0.0104}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.IT.lo.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.LOC.lo.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1\endcsname{+0.052}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1.4\endcsname{+0.0524}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1.hi\endcsname{0.066}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1.hi.4\endcsname{0.0662}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1.lo\endcsname{0.040}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V1.lo.4\endcsname{0.0395}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2\endcsname{+0.032}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2.4\endcsname{+0.0318}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2.hi\endcsname{0.043}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2.hi.4\endcsname{0.0427}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2.lo\endcsname{0.021}
\expandafter\def\csname nv@d.mr.all.ref.stdp.fa.V2.lo.4\endcsname{0.0213}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT.hi.4\endcsname{0.0025}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.IT.lo.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC.hi.4\endcsname{0.0038}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.LOC.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1.4\endcsname{+0.0081}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1.hi\endcsname{0.014}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1.hi.4\endcsname{0.0140}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V1.lo.4\endcsname{0.0024}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2.4\endcsname{+0.0079}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2.hi.4\endcsname{0.0132}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.all.ref.stdp.pc.V2.lo.4\endcsname{0.0029}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT.4\endcsname{+0.0041}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT.hi.4\endcsname{0.0125}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.IT.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC.4\endcsname{+0.0108}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC.hi.4\endcsname{0.0194}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.LOC.lo.4\endcsname{0.0022}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1.4\endcsname{-0.0113}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1.hi.4\endcsname{-0.0000}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V1.lo.4\endcsname{-0.0215}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2.hi.4\endcsname{0.0024}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.all.ref.stdp.rnd.V2.lo.4\endcsname{-0.0174}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT.4\endcsname{+0.0009}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT.hi.4\endcsname{0.0103}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.IT.lo.4\endcsname{-0.0084}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC.4\endcsname{+0.0070}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC.hi.4\endcsname{0.0176}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.LOC.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1\endcsname{+0.021}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1.4\endcsname{+0.0206}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1.hi\endcsname{0.028}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1.hi.4\endcsname{0.0279}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1.lo\endcsname{0.014}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V1.lo.4\endcsname{0.0137}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2.4\endcsname{+0.0134}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2.hi\endcsname{0.020}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2.hi.4\endcsname{0.0198}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.bp.fa.V2.lo.4\endcsname{0.0076}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT.4\endcsname{+0.0019}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT.hi.4\endcsname{0.0108}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.IT.lo.4\endcsname{-0.0070}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC.4\endcsname{+0.0063}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC.hi.4\endcsname{0.0171}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.LOC.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1\endcsname{+0.016}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1.4\endcsname{+0.0158}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1.hi\endcsname{0.023}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1.hi.4\endcsname{0.0227}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V1.lo.4\endcsname{0.0094}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2.4\endcsname{+0.0100}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2.hi.4\endcsname{0.0158}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.bp.pc.V2.lo.4\endcsname{0.0051}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT\endcsname{+0.009}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT.4\endcsname{+0.0087}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT.hi\endcsname{0.023}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT.hi.4\endcsname{0.0234}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.IT.lo.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC\endcsname{+0.020}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC.4\endcsname{+0.0205}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC.hi\endcsname{0.037}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC.hi.4\endcsname{0.0372}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC.lo\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.LOC.lo.4\endcsname{0.0047}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1.4\endcsname{-0.0426}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1.hi\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1.hi.4\endcsname{-0.0245}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1.lo\endcsname{-0.060}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V1.lo.4\endcsname{-0.0597}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2\endcsname{-0.025}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2.4\endcsname{-0.0249}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2.hi.4\endcsname{-0.0099}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2.lo\endcsname{-0.040}
\expandafter\def\csname nv@d.mr.cr.bn.bp.rnd.V2.lo.4\endcsname{-0.0398}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT.hi.4\endcsname{0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.IT.lo.4\endcsname{-0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC.4\endcsname{+0.0068}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC.hi.4\endcsname{0.0177}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.LOC.lo.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1.hi\endcsname{0.000}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1.hi.4\endcsname{0.0005}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V1.lo.4\endcsname{-0.0113}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2.hi.4\endcsname{0.0015}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.bp.stdp.V2.lo.4\endcsname{-0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT.hi.4\endcsname{0.0084}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.IT.lo.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC.4\endcsname{-0.0070}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.LOC.lo.4\endcsname{-0.0176}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1.4\endcsname{-0.0206}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1.hi.4\endcsname{-0.0137}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1.lo\endcsname{-0.028}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V1.lo.4\endcsname{-0.0279}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2.4\endcsname{-0.0134}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2.hi.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.bn.fa.bp.V2.lo.4\endcsname{-0.0198}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT.4\endcsname{+0.0011}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT.hi.4\endcsname{0.0086}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.IT.lo.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.LOC.lo.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1.hi.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V1.lo.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2.hi.4\endcsname{-0.0008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.fa.pc.V2.lo.4\endcsname{-0.0057}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT.4\endcsname{+0.0078}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT.hi.4\endcsname{0.0212}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.IT.lo.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC.4\endcsname{+0.0135}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC.hi\endcsname{0.026}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC.hi.4\endcsname{0.0260}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.LOC.lo.4\endcsname{0.0017}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1\endcsname{-0.063}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1.4\endcsname{-0.0631}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1.hi\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1.hi.4\endcsname{-0.0435}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1.lo\endcsname{-0.083}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V1.lo.4\endcsname{-0.0828}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2\endcsname{-0.038}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2.4\endcsname{-0.0383}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2.hi\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2.hi.4\endcsname{-0.0222}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.mr.cr.bn.fa.rnd.V2.lo.4\endcsname{-0.0549}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT.hi.4\endcsname{0.0059}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC.hi.4\endcsname{0.0062}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.LOC.lo.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1.4\endcsname{-0.0258}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1.hi.4\endcsname{-0.0187}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1.lo\endcsname{-0.033}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V1.lo.4\endcsname{-0.0334}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2.4\endcsname{-0.0168}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2.hi\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2.hi.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.bn.fa.stdp.V2.lo.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT.hi.4\endcsname{0.0070}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.IT.lo.4\endcsname{-0.0108}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC.4\endcsname{-0.0063}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.LOC.lo.4\endcsname{-0.0171}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1.4\endcsname{-0.0158}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1.hi.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V1.lo.4\endcsname{-0.0227}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2.hi.4\endcsname{-0.0051}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.cr.bn.pc.bp.V2.lo.4\endcsname{-0.0158}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT.hi.4\endcsname{0.0058}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.IT.lo.4\endcsname{-0.0086}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC.4\endcsname{+0.0007}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC.hi.4\endcsname{0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.LOC.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1.4\endcsname{+0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1.hi.4\endcsname{0.0079}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V1.lo.4\endcsname{0.0014}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2\endcsname{+0.003}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2.4\endcsname{+0.0033}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2.hi.4\endcsname{0.0057}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2.lo\endcsname{0.001}
\expandafter\def\csname nv@d.mr.cr.bn.pc.fa.V2.lo.4\endcsname{0.0008}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT.4\endcsname{+0.0067}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT.hi\endcsname{0.019}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT.hi.4\endcsname{0.0195}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.IT.lo.4\endcsname{-0.0061}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC\endcsname{+0.014}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC.4\endcsname{+0.0141}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC.hi\endcsname{0.025}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC.hi.4\endcsname{0.0248}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC.lo\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.LOC.lo.4\endcsname{0.0038}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1\endcsname{-0.058}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1.4\endcsname{-0.0583}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1.hi\endcsname{-0.041}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1.hi.4\endcsname{-0.0407}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1.lo\endcsname{-0.076}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V1.lo.4\endcsname{-0.0760}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2\endcsname{-0.035}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2.4\endcsname{-0.0349}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2.hi\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2.hi.4\endcsname{-0.0201}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2.lo\endcsname{-0.050}
\expandafter\def\csname nv@d.mr.cr.bn.pc.rnd.V2.lo.4\endcsname{-0.0501}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC.hi.4\endcsname{0.0055}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.LOC.lo.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1.4\endcsname{-0.0210}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1.hi.4\endcsname{-0.0152}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1.lo\endcsname{-0.027}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V1.lo.4\endcsname{-0.0271}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2.4\endcsname{-0.0135}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2.hi.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.cr.bn.pc.stdp.V2.lo.4\endcsname{-0.0184}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT.hi.4\endcsname{0.0058}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.IT.lo.4\endcsname{-0.0234}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC.4\endcsname{-0.0205}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC.hi.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC.lo\endcsname{-0.037}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.LOC.lo.4\endcsname{-0.0372}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1\endcsname{+0.043}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1.4\endcsname{+0.0426}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1.hi\endcsname{0.060}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1.hi.4\endcsname{0.0597}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1.lo\endcsname{0.024}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V1.lo.4\endcsname{0.0245}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2\endcsname{+0.025}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2.4\endcsname{+0.0249}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2.hi\endcsname{0.040}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2.hi.4\endcsname{0.0398}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2.lo\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.bp.V2.lo.4\endcsname{0.0099}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT.hi.4\endcsname{0.0048}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.IT.lo.4\endcsname{-0.0212}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC.4\endcsname{-0.0135}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC.hi.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.LOC.lo.4\endcsname{-0.0260}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1\endcsname{+0.063}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1.4\endcsname{+0.0631}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1.hi\endcsname{0.083}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1.hi.4\endcsname{0.0828}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1.lo\endcsname{0.043}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V1.lo.4\endcsname{0.0435}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2\endcsname{+0.038}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2.4\endcsname{+0.0383}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2.hi\endcsname{0.055}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2.hi.4\endcsname{0.0549}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2.lo\endcsname{0.022}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.fa.V2.lo.4\endcsname{0.0222}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT.4\endcsname{-0.0067}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT.hi.4\endcsname{0.0061}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.IT.lo.4\endcsname{-0.0195}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC.4\endcsname{-0.0141}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC.hi.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.LOC.lo.4\endcsname{-0.0248}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1\endcsname{+0.058}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1.4\endcsname{+0.0583}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1.hi\endcsname{0.076}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1.hi.4\endcsname{0.0760}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1.lo\endcsname{0.041}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V1.lo.4\endcsname{0.0407}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2\endcsname{+0.035}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2.4\endcsname{+0.0349}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2.hi\endcsname{0.050}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2.hi.4\endcsname{0.0501}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2.lo\endcsname{0.020}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.pc.V2.lo.4\endcsname{0.0201}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT.4\endcsname{-0.0085}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT.hi.4\endcsname{0.0040}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.IT.lo.4\endcsname{-0.0208}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC.4\endcsname{-0.0136}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC.hi.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.LOC.lo.4\endcsname{-0.0243}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1\endcsname{+0.037}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1.4\endcsname{+0.0374}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1.hi\endcsname{0.054}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1.hi.4\endcsname{0.0538}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1.lo\endcsname{0.021}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V1.lo.4\endcsname{0.0206}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2\endcsname{+0.021}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2.4\endcsname{+0.0215}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2.hi.4\endcsname{0.0357}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.mr.cr.bn.rnd.stdp.V2.lo.4\endcsname{0.0072}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT.hi.4\endcsname{0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.IT.lo.4\endcsname{-0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC.hi.4\endcsname{0.0029}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.LOC.lo.4\endcsname{-0.0177}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1.hi.4\endcsname{0.0113}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V1.lo.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2\endcsname{+0.003}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2.4\endcsname{+0.0034}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2.hi.4\endcsname{0.0080}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.bp.V2.lo.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT.4\endcsname{+0.0007}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.IT.lo.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC.hi.4\endcsname{0.0059}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.LOC.lo.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1\endcsname{+0.026}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1.4\endcsname{+0.0258}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1.hi\endcsname{0.033}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1.hi.4\endcsname{0.0334}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V1.lo.4\endcsname{0.0187}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2.4\endcsname{+0.0168}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2.hi\endcsname{0.023}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2.hi.4\endcsname{0.0226}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2.lo\endcsname{0.012}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.fa.V2.lo.4\endcsname{0.0115}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.IT.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC.hi.4\endcsname{0.0047}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.LOC.lo.4\endcsname{-0.0055}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1\endcsname{+0.021}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1.4\endcsname{+0.0210}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1.hi\endcsname{0.027}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1.hi.4\endcsname{0.0271}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1.lo\endcsname{0.015}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V1.lo.4\endcsname{0.0152}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2.4\endcsname{+0.0135}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2.hi.4\endcsname{0.0184}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.pc.V2.lo.4\endcsname{0.0092}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT.4\endcsname{+0.0085}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT.hi.4\endcsname{0.0208}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.IT.lo.4\endcsname{-0.0040}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC\endcsname{+0.014}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC.4\endcsname{+0.0136}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC.hi\endcsname{0.024}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC.hi.4\endcsname{0.0243}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.LOC.lo.4\endcsname{0.0024}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1\endcsname{-0.037}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1.4\endcsname{-0.0374}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1.hi\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1.hi.4\endcsname{-0.0206}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1.lo\endcsname{-0.054}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V1.lo.4\endcsname{-0.0538}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2.4\endcsname{-0.0215}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2.hi.4\endcsname{-0.0072}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.mr.cr.bn.stdp.rnd.V2.lo.4\endcsname{-0.0357}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT.4\endcsname{+0.0013}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT.hi.4\endcsname{0.0113}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.IT.lo.4\endcsname{-0.0086}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC.4\endcsname{+0.0060}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC.hi.4\endcsname{0.0171}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.LOC.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1\endcsname{+0.023}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1.4\endcsname{+0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1.hi\endcsname{0.031}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1.hi.4\endcsname{0.0309}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1.lo\endcsname{0.015}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V1.lo.4\endcsname{0.0149}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2.4\endcsname{+0.0151}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2.hi.4\endcsname{0.0223}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.bp.fa.V2.lo.4\endcsname{0.0087}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT.hi.4\endcsname{0.0123}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.IT.lo.4\endcsname{-0.0099}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC.4\endcsname{+0.0074}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC.hi\endcsname{0.023}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC.hi.4\endcsname{0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.LOC.lo.4\endcsname{-0.0064}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1.hi.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1.lo\endcsname{-0.034}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V1.lo.4\endcsname{-0.0342}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.ref.bp.pc.V2.lo.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT\endcsname{+0.009}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT.4\endcsname{+0.0091}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT.hi\endcsname{0.024}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT.hi.4\endcsname{0.0245}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.IT.lo.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC\endcsname{+0.019}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC.4\endcsname{+0.0195}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC.hi\endcsname{0.036}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC.hi.4\endcsname{0.0363}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC.lo\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.LOC.lo.4\endcsname{0.0037}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1\endcsname{-0.040}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1.4\endcsname{-0.0404}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1.hi\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1.hi.4\endcsname{-0.0218}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V1.lo.4\endcsname{-0.0581}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2.4\endcsname{-0.0233}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2.hi.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2.lo\endcsname{-0.038}
\expandafter\def\csname nv@d.mr.cr.ref.bp.rnd.V2.lo.4\endcsname{-0.0383}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT.4\endcsname{+0.0040}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT.hi.4\endcsname{0.0157}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.IT.lo.4\endcsname{-0.0085}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC.4\endcsname{+0.0072}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC.hi\endcsname{0.020}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC.hi.4\endcsname{0.0203}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.LOC.lo.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1\endcsname{-0.028}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1.4\endcsname{-0.0285}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1.hi.4\endcsname{-0.0161}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1.lo\endcsname{-0.040}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V1.lo.4\endcsname{-0.0400}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2.4\endcsname{-0.0159}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2.hi.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.cr.ref.bp.stdp.V2.lo.4\endcsname{-0.0259}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT.hi.4\endcsname{0.0086}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.IT.lo.4\endcsname{-0.0113}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.LOC.lo.4\endcsname{-0.0171}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1.hi.4\endcsname{-0.0149}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1.lo\endcsname{-0.031}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V1.lo.4\endcsname{-0.0309}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2.hi.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.cr.ref.fa.bp.V2.lo.4\endcsname{-0.0223}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.IT.lo.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC.4\endcsname{+0.0014}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC.hi.4\endcsname{0.0120}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.LOC.lo.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1.4\endcsname{-0.0428}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1.hi\endcsname{-0.028}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1.hi.4\endcsname{-0.0284}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1.lo\endcsname{-0.057}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V1.lo.4\endcsname{-0.0574}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2.4\endcsname{-0.0229}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2.hi.4\endcsname{-0.0098}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.mr.cr.ref.fa.pc.V2.lo.4\endcsname{-0.0355}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT.4\endcsname{+0.0079}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT.hi.4\endcsname{0.0210}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.IT.lo.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC\endcsname{+0.013}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC.4\endcsname{+0.0134}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC.hi\endcsname{0.026}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC.hi.4\endcsname{0.0259}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.LOC.lo.4\endcsname{0.0018}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1\endcsname{-0.063}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1.4\endcsname{-0.0630}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1.hi\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1.hi.4\endcsname{-0.0433}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1.lo\endcsname{-0.082}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V1.lo.4\endcsname{-0.0825}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2\endcsname{-0.038}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2.4\endcsname{-0.0384}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2.hi\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2.hi.4\endcsname{-0.0225}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.mr.cr.ref.fa.rnd.V2.lo.4\endcsname{-0.0549}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT.4\endcsname{+0.0027}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT.hi.4\endcsname{0.0133}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.IT.lo.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC.4\endcsname{+0.0012}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.LOC.lo.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1\endcsname{-0.051}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1.4\endcsname{-0.0511}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1.hi\endcsname{-0.038}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1.hi.4\endcsname{-0.0375}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1.lo\endcsname{-0.065}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V1.lo.4\endcsname{-0.0654}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2\endcsname{-0.031}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2.4\endcsname{-0.0310}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2.hi\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2.hi.4\endcsname{-0.0198}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2.lo\endcsname{-0.043}
\expandafter\def\csname nv@d.mr.cr.ref.fa.stdp.V2.lo.4\endcsname{-0.0428}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT.hi.4\endcsname{0.0099}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.IT.lo.4\endcsname{-0.0123}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC.hi.4\endcsname{0.0064}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.LOC.lo.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1\endcsname{+0.020}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1.4\endcsname{+0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1.hi\endcsname{0.034}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1.hi.4\endcsname{0.0342}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1.lo\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V1.lo.4\endcsname{0.0059}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2.4\endcsname{+0.0078}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2.hi\endcsname{0.020}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2.hi.4\endcsname{0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.pc.bp.V2.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT.hi.4\endcsname{0.0092}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.IT.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC.hi.4\endcsname{0.0087}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.LOC.lo.4\endcsname{-0.0120}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1\endcsname{+0.043}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1.4\endcsname{+0.0428}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1.hi\endcsname{0.057}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1.hi.4\endcsname{0.0574}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1.lo\endcsname{0.028}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V1.lo.4\endcsname{0.0284}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2\endcsname{+0.023}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2.4\endcsname{+0.0229}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2.hi.4\endcsname{0.0355}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2.lo\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.ref.pc.fa.V2.lo.4\endcsname{0.0098}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT.4\endcsname{+0.0075}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT.hi\endcsname{0.018}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT.hi.4\endcsname{0.0180}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.IT.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC\endcsname{+0.012}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC.4\endcsname{+0.0121}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC.hi.4\endcsname{0.0213}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.LOC.lo.4\endcsname{0.0029}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1.hi.4\endcsname{-0.0102}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1.lo\endcsname{-0.030}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V1.lo.4\endcsname{-0.0302}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2.4\endcsname{-0.0155}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2.hi.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2.lo\endcsname{-0.025}
\expandafter\def\csname nv@d.mr.cr.ref.pc.rnd.V2.lo.4\endcsname{-0.0249}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT.4\endcsname{+0.0023}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.IT.lo.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC.hi.4\endcsname{0.0045}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.LOC.lo.4\endcsname{-0.0043}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1.4\endcsname{-0.0083}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1.hi.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V1.lo.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2.4\endcsname{-0.0082}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2.hi.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.ref.pc.stdp.V2.lo.4\endcsname{-0.0137}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT\endcsname{-0.009}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT.hi.4\endcsname{0.0062}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.IT.lo.4\endcsname{-0.0245}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC\endcsname{-0.019}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC.4\endcsname{-0.0195}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC.hi.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.LOC.lo.4\endcsname{-0.0363}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1\endcsname{+0.040}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1.4\endcsname{+0.0404}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1.hi\endcsname{0.058}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1.hi.4\endcsname{0.0581}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1.lo\endcsname{0.022}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V1.lo.4\endcsname{0.0218}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2\endcsname{+0.023}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2.4\endcsname{+0.0233}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2.hi\endcsname{0.038}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2.hi.4\endcsname{0.0383}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.bp.V2.lo.4\endcsname{0.0078}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT\endcsname{-0.008}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT.hi.4\endcsname{0.0048}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.IT.lo.4\endcsname{-0.0210}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC.4\endcsname{-0.0134}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC.hi.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.LOC.lo.4\endcsname{-0.0259}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1\endcsname{+0.063}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1.4\endcsname{+0.0630}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1.hi\endcsname{0.082}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1.hi.4\endcsname{0.0825}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1.lo\endcsname{0.043}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V1.lo.4\endcsname{0.0433}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2\endcsname{+0.038}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2.4\endcsname{+0.0384}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2.hi\endcsname{0.055}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2.hi.4\endcsname{0.0549}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2.lo\endcsname{0.022}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.fa.V2.lo.4\endcsname{0.0225}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.IT.lo.4\endcsname{-0.0180}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC.4\endcsname{-0.0121}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC.hi.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.LOC.lo.4\endcsname{-0.0213}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1\endcsname{+0.020}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1.4\endcsname{+0.0202}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1.hi\endcsname{0.030}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1.hi.4\endcsname{0.0302}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V1.lo.4\endcsname{0.0102}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2.4\endcsname{+0.0155}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2.hi\endcsname{0.025}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2.hi.4\endcsname{0.0249}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.pc.V2.lo.4\endcsname{0.0065}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT.hi.4\endcsname{0.0038}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.IT.lo.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC.4\endcsname{-0.0122}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC.hi.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.LOC.lo.4\endcsname{-0.0217}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1\endcsname{+0.012}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1.4\endcsname{+0.0119}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1.hi\endcsname{0.023}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1.hi.4\endcsname{0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V1.lo.4\endcsname{0.0004}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2\endcsname{+0.007}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2.4\endcsname{+0.0073}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2.hi.4\endcsname{0.0174}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.rnd.stdp.V2.lo.4\endcsname{-0.0028}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT.4\endcsname{-0.0040}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT.hi.4\endcsname{0.0085}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.IT.lo.4\endcsname{-0.0157}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC.4\endcsname{-0.0072}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC.hi.4\endcsname{0.0047}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.LOC.lo.4\endcsname{-0.0203}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1\endcsname{+0.028}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1.4\endcsname{+0.0285}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1.hi\endcsname{0.040}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1.hi.4\endcsname{0.0400}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1.lo\endcsname{0.016}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V1.lo.4\endcsname{0.0161}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2\endcsname{+0.016}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2.4\endcsname{+0.0159}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2.hi\endcsname{0.026}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2.hi.4\endcsname{0.0259}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.bp.V2.lo.4\endcsname{0.0053}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT.hi.4\endcsname{0.0090}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.IT.lo.4\endcsname{-0.0133}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC.hi\endcsname{0.007}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC.hi.4\endcsname{0.0073}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.LOC.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1\endcsname{+0.051}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1.4\endcsname{+0.0511}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1.hi\endcsname{0.065}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1.hi.4\endcsname{0.0654}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1.lo\endcsname{0.038}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V1.lo.4\endcsname{0.0375}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2\endcsname{+0.031}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2.4\endcsname{+0.0310}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2.hi\endcsname{0.043}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2.hi.4\endcsname{0.0428}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2.lo\endcsname{0.020}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.fa.V2.lo.4\endcsname{0.0198}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT.hi.4\endcsname{0.0026}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC.hi.4\endcsname{0.0043}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.LOC.lo.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1.4\endcsname{+0.0083}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1.hi\endcsname{0.014}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1.hi.4\endcsname{0.0145}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V1.lo.4\endcsname{0.0020}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2.4\endcsname{+0.0082}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2.hi.4\endcsname{0.0137}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.pc.V2.lo.4\endcsname{0.0030}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT.hi.4\endcsname{0.0145}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.IT.lo.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC\endcsname{+0.012}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC.4\endcsname{+0.0122}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC.hi.4\endcsname{0.0217}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC.lo\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.LOC.lo.4\endcsname{0.0035}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1\endcsname{-0.012}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1.4\endcsname{-0.0119}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1.hi.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V1.lo.4\endcsname{-0.0226}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2\endcsname{-0.007}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2.hi\endcsname{0.003}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2.hi.4\endcsname{0.0028}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.mr.cr.ref.stdp.rnd.V2.lo.4\endcsname{-0.0174}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT.4\endcsname{+0.0017}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT.hi.4\endcsname{0.0068}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.IT.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC.4\endcsname{+0.0042}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC.hi.4\endcsname{0.0095}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.LOC.lo.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1\endcsname{+0.013}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1.4\endcsname{+0.0134}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1.hi\endcsname{0.018}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1.hi.4\endcsname{0.0178}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V1.lo.4\endcsname{0.0090}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2.4\endcsname{+0.0084}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2.hi.4\endcsname{0.0120}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.bp.fa.V2.lo.4\endcsname{0.0052}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT.hi.4\endcsname{0.0065}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.IT.lo.4\endcsname{-0.0031}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC.4\endcsname{+0.0036}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC.hi.4\endcsname{0.0092}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.LOC.lo.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1.4\endcsname{+0.0100}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1.hi.4\endcsname{0.0142}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V1.lo.4\endcsname{0.0061}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2.4\endcsname{+0.0062}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2.hi.4\endcsname{0.0095}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2.lo\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.bp.pc.V2.lo.4\endcsname{0.0033}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT.4\endcsname{+0.0035}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT.hi.4\endcsname{0.0120}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.IT.lo.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC.4\endcsname{+0.0096}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC.hi\endcsname{0.018}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC.hi.4\endcsname{0.0181}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.LOC.lo.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1\endcsname{-0.032}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1.4\endcsname{-0.0319}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1.hi\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1.hi.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1.lo\endcsname{-0.044}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V1.lo.4\endcsname{-0.0440}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2.4\endcsname{-0.0176}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2.hi.4\endcsname{-0.0086}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2.lo\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.all.bn.bp.rnd.V2.lo.4\endcsname{-0.0269}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT.hi.4\endcsname{0.0049}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.IT.lo.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC.4\endcsname{+0.0038}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC.hi.4\endcsname{0.0094}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.LOC.lo.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1.hi.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V1.lo.4\endcsname{-0.0081}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2.hi.4\endcsname{0.0000}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.bp.stdp.V2.lo.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.IT.lo.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC.4\endcsname{-0.0042}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC.hi.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.LOC.lo.4\endcsname{-0.0095}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1.4\endcsname{-0.0134}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1.hi.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V1.lo.4\endcsname{-0.0178}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2.4\endcsname{-0.0084}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2.hi.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.fa.bp.V2.lo.4\endcsname{-0.0120}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT.hi.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.IT.lo.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC.hi.4\endcsname{0.0020}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.LOC.lo.4\endcsname{-0.0028}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1.hi.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V1.lo.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2.4\endcsname{-0.0022}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2.hi.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.fa.pc.V2.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT.hi.4\endcsname{0.0091}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.IT.lo.4\endcsname{-0.0051}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC.4\endcsname{+0.0054}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC.hi.4\endcsname{0.0121}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.LOC.lo.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1\endcsname{-0.045}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1.4\endcsname{-0.0453}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1.hi\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1.hi.4\endcsname{-0.0325}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V1.lo.4\endcsname{-0.0581}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2.4\endcsname{-0.0260}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2.hi.4\endcsname{-0.0162}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.all.bn.fa.rnd.V2.lo.4\endcsname{-0.0362}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT.hi.4\endcsname{0.0020}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.IT.lo.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC.hi.4\endcsname{0.0031}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.LOC.lo.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1.4\endcsname{-0.0179}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1.hi\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1.hi.4\endcsname{-0.0131}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V1.lo.4\endcsname{-0.0229}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2.4\endcsname{-0.0110}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2.hi.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.bn.fa.stdp.V2.lo.4\endcsname{-0.0144}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT.hi.4\endcsname{0.0031}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.IT.lo.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC.hi.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.LOC.lo.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1.hi.4\endcsname{-0.0061}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V1.lo.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2.hi.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.pc.bp.V2.lo.4\endcsname{-0.0095}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT.hi.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.IT.lo.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC.hi.4\endcsname{0.0028}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.LOC.lo.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1.4\endcsname{+0.0033}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1.hi.4\endcsname{0.0053}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V1.lo.4\endcsname{0.0012}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2.4\endcsname{+0.0022}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.pc.fa.V2.lo.4\endcsname{0.0006}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT.4\endcsname{+0.0019}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT.hi.4\endcsname{0.0088}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.IT.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC.4\endcsname{+0.0059}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC.hi.4\endcsname{0.0118}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.LOC.lo.4\endcsname{0.0003}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1\endcsname{-0.042}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1.4\endcsname{-0.0419}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1.hi\endcsname{-0.030}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1.hi.4\endcsname{-0.0300}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1.lo\endcsname{-0.054}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V1.lo.4\endcsname{-0.0538}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2\endcsname{-0.024}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2.4\endcsname{-0.0239}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2.hi.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2.lo\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.all.bn.pc.rnd.V2.lo.4\endcsname{-0.0332}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT.hi.4\endcsname{0.0018}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.IT.lo.4\endcsname{-0.0046}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC.hi.4\endcsname{0.0029}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.LOC.lo.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1.hi\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1.hi.4\endcsname{-0.0107}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V1.lo.4\endcsname{-0.0186}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2.4\endcsname{-0.0088}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2.hi.4\endcsname{-0.0061}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.pc.stdp.V2.lo.4\endcsname{-0.0117}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT.hi.4\endcsname{0.0045}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.IT.lo.4\endcsname{-0.0120}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC.4\endcsname{-0.0096}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC.hi.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.LOC.lo.4\endcsname{-0.0181}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1\endcsname{+0.032}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1.4\endcsname{+0.0319}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1.hi\endcsname{0.044}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1.hi.4\endcsname{0.0440}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1.lo\endcsname{0.020}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V1.lo.4\endcsname{0.0202}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2\endcsname{+0.018}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2.4\endcsname{+0.0176}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2.hi\endcsname{0.027}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2.hi.4\endcsname{0.0269}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.bn.rnd.bp.V2.lo.4\endcsname{0.0086}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT.hi.4\endcsname{0.0051}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.IT.lo.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC.hi.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.LOC.lo.4\endcsname{-0.0121}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1\endcsname{+0.045}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1.4\endcsname{+0.0453}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1.hi\endcsname{0.058}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1.hi.4\endcsname{0.0581}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1.lo\endcsname{0.033}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V1.lo.4\endcsname{0.0325}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2\endcsname{+0.026}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2.4\endcsname{+0.0260}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2.hi.4\endcsname{0.0362}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2.lo\endcsname{0.016}
\expandafter\def\csname nv@d.ps.all.bn.rnd.fa.V2.lo.4\endcsname{0.0162}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.IT.lo.4\endcsname{-0.0088}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC.hi.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.LOC.lo.4\endcsname{-0.0118}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1\endcsname{+0.042}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1.4\endcsname{+0.0419}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1.hi\endcsname{0.054}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1.hi.4\endcsname{0.0538}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1.lo\endcsname{0.030}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V1.lo.4\endcsname{0.0300}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2\endcsname{+0.024}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2.4\endcsname{+0.0239}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2.hi\endcsname{0.033}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2.hi.4\endcsname{0.0332}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2.lo\endcsname{0.015}
\expandafter\def\csname nv@d.ps.all.bn.rnd.pc.V2.lo.4\endcsname{0.0151}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT.hi.4\endcsname{0.0031}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.IT.lo.4\endcsname{-0.0102}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC.hi.4\endcsname{-0.0000}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.LOC.lo.4\endcsname{-0.0117}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1\endcsname{+0.027}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1.4\endcsname{+0.0274}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1.hi\endcsname{0.038}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1.hi.4\endcsname{0.0384}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1.lo\endcsname{0.016}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V1.lo.4\endcsname{0.0163}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2.4\endcsname{+0.0151}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2.hi\endcsname{0.024}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2.hi.4\endcsname{0.0241}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.bn.rnd.stdp.V2.lo.4\endcsname{0.0063}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT.hi.4\endcsname{0.0045}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.IT.lo.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC.hi.4\endcsname{0.0013}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.LOC.lo.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1.4\endcsname{+0.0045}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1.hi.4\endcsname{0.0081}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V1.lo.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2.4\endcsname{+0.0026}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2.hi.4\endcsname{0.0052}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.bp.V2.lo.4\endcsname{-0.0000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT.4\endcsname{+0.0014}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT.hi.4\endcsname{0.0049}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.IT.lo.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC.hi.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.LOC.lo.4\endcsname{-0.0031}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1\endcsname{+0.018}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1.4\endcsname{+0.0179}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1.hi\endcsname{0.023}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1.hi.4\endcsname{0.0229}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V1.lo.4\endcsname{0.0131}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2.4\endcsname{+0.0110}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2.hi.4\endcsname{0.0144}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.bn.stdp.fa.V2.lo.4\endcsname{0.0077}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT.4\endcsname{+0.0013}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT.hi.4\endcsname{0.0046}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.IT.lo.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC.hi.4\endcsname{0.0027}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.LOC.lo.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1.4\endcsname{+0.0145}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1.hi\endcsname{0.019}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1.hi.4\endcsname{0.0186}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1.lo\endcsname{0.011}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V1.lo.4\endcsname{0.0107}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2.4\endcsname{+0.0088}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2.hi.4\endcsname{0.0117}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.bn.stdp.pc.V2.lo.4\endcsname{0.0061}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT.4\endcsname{+0.0032}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT.hi.4\endcsname{0.0102}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.IT.lo.4\endcsname{-0.0031}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC.4\endcsname{+0.0058}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC.hi.4\endcsname{0.0117}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.LOC.lo.4\endcsname{0.0000}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1.4\endcsname{-0.0274}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1.hi.4\endcsname{-0.0163}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1.lo\endcsname{-0.038}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V1.lo.4\endcsname{-0.0384}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2.hi.4\endcsname{-0.0063}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.ps.all.bn.stdp.rnd.V2.lo.4\endcsname{-0.0241}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT.4\endcsname{+0.0023}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.IT.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC.4\endcsname{+0.0036}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC.hi.4\endcsname{0.0093}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.LOC.lo.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1.4\endcsname{+0.0147}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1.hi\endcsname{0.020}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1.hi.4\endcsname{0.0199}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V1.lo.4\endcsname{0.0098}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2.4\endcsname{+0.0095}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2.hi.4\endcsname{0.0135}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.ref.bp.fa.V2.lo.4\endcsname{0.0058}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT.hi.4\endcsname{0.0064}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.IT.lo.4\endcsname{-0.0056}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC.4\endcsname{+0.0030}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC.hi.4\endcsname{0.0107}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.LOC.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1.4\endcsname{-0.0162}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1.hi.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V1.lo.4\endcsname{-0.0258}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2.4\endcsname{-0.0063}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2.hi.4\endcsname{0.0019}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.ref.bp.pc.V2.lo.4\endcsname{-0.0137}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT.4\endcsname{+0.0041}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT.hi.4\endcsname{0.0128}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.IT.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC.4\endcsname{+0.0090}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC.hi\endcsname{0.018}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC.hi.4\endcsname{0.0180}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.LOC.lo.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1\endcsname{-0.030}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1.4\endcsname{-0.0304}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1.hi\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1.hi.4\endcsname{-0.0184}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1.lo\endcsname{-0.042}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V1.lo.4\endcsname{-0.0424}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2.4\endcsname{-0.0166}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2.hi.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.all.ref.bp.rnd.V2.lo.4\endcsname{-0.0260}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT.4\endcsname{+0.0017}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT.hi.4\endcsname{0.0083}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.IT.lo.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC.4\endcsname{+0.0032}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.LOC.lo.4\endcsname{-0.0031}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1\endcsname{-0.022}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1.4\endcsname{-0.0218}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1.hi.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1.lo\endcsname{-0.029}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V1.lo.4\endcsname{-0.0293}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2.4\endcsname{-0.0114}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2.hi.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.ref.bp.stdp.V2.lo.4\endcsname{-0.0177}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC.hi.4\endcsname{0.0015}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.LOC.lo.4\endcsname{-0.0093}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1.4\endcsname{-0.0147}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1.hi.4\endcsname{-0.0098}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V1.lo.4\endcsname{-0.0199}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2.4\endcsname{-0.0095}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2.hi.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.all.ref.fa.bp.V2.lo.4\endcsname{-0.0135}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT.hi.4\endcsname{0.0033}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.IT.lo.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.LOC.lo.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1\endcsname{-0.031}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1.4\endcsname{-0.0309}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1.hi\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1.hi.4\endcsname{-0.0214}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1.lo\endcsname{-0.041}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V1.lo.4\endcsname{-0.0407}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2.4\endcsname{-0.0158}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2.hi.4\endcsname{-0.0082}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.all.ref.fa.pc.V2.lo.4\endcsname{-0.0234}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT.hi.4\endcsname{0.0091}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.IT.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC.4\endcsname{+0.0054}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC.hi.4\endcsname{0.0121}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.LOC.lo.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1\endcsname{-0.045}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1.4\endcsname{-0.0451}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1.hi\endcsname{-0.032}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1.hi.4\endcsname{-0.0324}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V1.lo.4\endcsname{-0.0579}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2.4\endcsname{-0.0261}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2.hi.4\endcsname{-0.0163}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.all.ref.fa.rnd.V2.lo.4\endcsname{-0.0362}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.IT.lo.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC.hi.4\endcsname{0.0041}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.LOC.lo.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1\endcsname{-0.037}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1.4\endcsname{-0.0365}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1.hi\endcsname{-0.028}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1.hi.4\endcsname{-0.0277}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1.lo\endcsname{-0.046}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V1.lo.4\endcsname{-0.0458}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2.4\endcsname{-0.0209}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2.hi.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2.lo\endcsname{-0.028}
\expandafter\def\csname nv@d.ps.all.ref.fa.stdp.V2.lo.4\endcsname{-0.0282}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT.hi.4\endcsname{0.0056}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.IT.lo.4\endcsname{-0.0064}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.LOC.lo.4\endcsname{-0.0107}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1\endcsname{+0.016}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1.4\endcsname{+0.0162}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1.hi.4\endcsname{0.0258}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V1.lo.4\endcsname{0.0066}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2.4\endcsname{+0.0063}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2.hi.4\endcsname{0.0137}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.bp.V2.lo.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT.hi.4\endcsname{0.0066}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.IT.lo.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC.4\endcsname{+0.0006}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC.hi.4\endcsname{0.0058}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.LOC.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1\endcsname{+0.031}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1.4\endcsname{+0.0309}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1.hi\endcsname{0.041}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1.hi.4\endcsname{0.0407}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1.lo\endcsname{0.021}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V1.lo.4\endcsname{0.0214}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2\endcsname{+0.016}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2.4\endcsname{+0.0158}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2.hi\endcsname{0.023}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2.hi.4\endcsname{0.0234}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.ref.pc.fa.V2.lo.4\endcsname{0.0082}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT.hi.4\endcsname{0.0092}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.IT.lo.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC.4\endcsname{+0.0060}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC.hi.4\endcsname{0.0109}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.LOC.lo.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1.hi.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V1.lo.4\endcsname{-0.0208}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2.hi.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.ref.pc.rnd.V2.lo.4\endcsname{-0.0159}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT.4\endcsname{+0.0012}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT.hi.4\endcsname{0.0040}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.IT.lo.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC.hi.4\endcsname{0.0027}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.LOC.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1.4\endcsname{-0.0056}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1.hi.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V1.lo.4\endcsname{-0.0096}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2.4\endcsname{-0.0051}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2.hi.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.pc.stdp.V2.lo.4\endcsname{-0.0085}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.IT.lo.4\endcsname{-0.0128}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC.hi.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.LOC.lo.4\endcsname{-0.0180}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1\endcsname{+0.030}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1.4\endcsname{+0.0304}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1.hi\endcsname{0.042}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1.hi.4\endcsname{0.0424}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1.lo\endcsname{0.018}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V1.lo.4\endcsname{0.0184}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2.4\endcsname{+0.0166}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2.hi.4\endcsname{0.0260}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.all.ref.rnd.bp.V2.lo.4\endcsname{0.0074}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.IT.lo.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC.hi.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.LOC.lo.4\endcsname{-0.0121}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1\endcsname{+0.045}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1.4\endcsname{+0.0451}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1.hi\endcsname{0.058}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1.hi.4\endcsname{0.0579}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1.lo\endcsname{0.032}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V1.lo.4\endcsname{0.0324}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2\endcsname{+0.026}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2.4\endcsname{+0.0261}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2.hi.4\endcsname{0.0362}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2.lo\endcsname{0.016}
\expandafter\def\csname nv@d.ps.all.ref.rnd.fa.V2.lo.4\endcsname{0.0163}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT.hi.4\endcsname{0.0016}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.IT.lo.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC.hi.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.LOC.lo.4\endcsname{-0.0109}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1.4\endcsname{+0.0142}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1.hi.4\endcsname{0.0208}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V1.lo.4\endcsname{0.0077}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2.4\endcsname{+0.0103}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2.hi\endcsname{0.016}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2.hi.4\endcsname{0.0159}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.rnd.pc.V2.lo.4\endcsname{0.0048}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT.4\endcsname{-0.0025}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT.hi.4\endcsname{0.0021}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.IT.lo.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC.hi.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.LOC.lo.4\endcsname{-0.0110}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1.4\endcsname{+0.0086}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1.hi\endcsname{0.016}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1.hi.4\endcsname{0.0158}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V1.lo.4\endcsname{0.0008}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2.hi.4\endcsname{0.0114}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.rnd.stdp.V2.lo.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT.hi.4\endcsname{0.0052}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.IT.lo.4\endcsname{-0.0083}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC.hi.4\endcsname{0.0031}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.LOC.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1\endcsname{+0.022}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1.4\endcsname{+0.0218}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1.hi\endcsname{0.029}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1.hi.4\endcsname{0.0293}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1.lo\endcsname{0.014}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V1.lo.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2.4\endcsname{+0.0114}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2.hi\endcsname{0.018}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2.hi.4\endcsname{0.0177}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.bp.V2.lo.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT.4\endcsname{+0.0006}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT.hi.4\endcsname{0.0066}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.IT.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC.hi.4\endcsname{0.0047}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.LOC.lo.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1\endcsname{+0.037}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1.4\endcsname{+0.0365}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1.hi\endcsname{0.046}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1.hi.4\endcsname{0.0458}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1.lo\endcsname{0.028}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V1.lo.4\endcsname{0.0277}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2\endcsname{+0.021}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2.4\endcsname{+0.0209}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2.hi\endcsname{0.028}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2.hi.4\endcsname{0.0282}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2.lo\endcsname{0.014}
\expandafter\def\csname nv@d.ps.all.ref.stdp.fa.V2.lo.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT.hi.4\endcsname{0.0015}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.IT.lo.4\endcsname{-0.0040}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.LOC.lo.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1.4\endcsname{+0.0056}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1.hi.4\endcsname{0.0096}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V1.lo.4\endcsname{0.0015}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2.4\endcsname{+0.0051}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2.hi.4\endcsname{0.0085}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.pc.V2.lo.4\endcsname{0.0020}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT.4\endcsname{+0.0025}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT.hi.4\endcsname{0.0076}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.IT.lo.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC.4\endcsname{+0.0058}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC.hi.4\endcsname{0.0110}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.LOC.lo.4\endcsname{0.0006}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1.4\endcsname{-0.0086}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1.hi.4\endcsname{-0.0008}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V1.lo.4\endcsname{-0.0158}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2.hi.4\endcsname{0.0011}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.all.ref.stdp.rnd.V2.lo.4\endcsname{-0.0114}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.IT.lo.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC.4\endcsname{+0.0044}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC.hi.4\endcsname{0.0102}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.LOC.lo.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1.4\endcsname{+0.0138}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1.hi\endcsname{0.019}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1.hi.4\endcsname{0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V1.lo.4\endcsname{0.0092}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2.4\endcsname{+0.0087}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2.hi.4\endcsname{0.0125}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.bp.fa.V2.lo.4\endcsname{0.0053}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT.4\endcsname{+0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT.hi.4\endcsname{0.0072}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.IT.lo.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC.hi.4\endcsname{0.0097}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.LOC.lo.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1.4\endcsname{+0.0104}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1.hi.4\endcsname{0.0149}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V1.lo.4\endcsname{0.0065}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2.4\endcsname{+0.0066}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.pc.V2.lo.4\endcsname{0.0035}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT.4\endcsname{+0.0054}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT.hi.4\endcsname{0.0144}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.IT.lo.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC.4\endcsname{+0.0110}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC.hi.4\endcsname{0.0206}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.LOC.lo.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1\endcsname{-0.031}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1.4\endcsname{-0.0308}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1.hi.4\endcsname{-0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1.lo\endcsname{-0.043}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V1.lo.4\endcsname{-0.0428}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2.4\endcsname{-0.0165}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2.hi.4\endcsname{-0.0072}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.cr.bn.bp.rnd.V2.lo.4\endcsname{-0.0261}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT.4\endcsname{+0.0006}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT.hi.4\endcsname{0.0056}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.IT.lo.4\endcsname{-0.0043}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC.hi.4\endcsname{0.0097}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.LOC.lo.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1.4\endcsname{-0.0042}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1.hi.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V1.lo.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2.hi.4\endcsname{0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.bp.stdp.V2.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT.hi.4\endcsname{0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC.hi.4\endcsname{0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.LOC.lo.4\endcsname{-0.0102}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1.4\endcsname{-0.0138}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1.hi.4\endcsname{-0.0092}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V1.lo.4\endcsname{-0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2.hi.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.cr.bn.fa.bp.V2.lo.4\endcsname{-0.0125}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.IT.lo.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC.hi.4\endcsname{0.0018}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.LOC.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1.hi.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V1.lo.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2.hi.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.pc.V2.lo.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT.4\endcsname{+0.0039}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT.hi.4\endcsname{0.0118}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.IT.lo.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC.4\endcsname{+0.0066}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC.hi.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.LOC.lo.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1\endcsname{-0.045}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1.4\endcsname{-0.0446}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1.hi\endcsname{-0.031}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1.hi.4\endcsname{-0.0313}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V1.lo.4\endcsname{-0.0580}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2\endcsname{-0.025}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2.4\endcsname{-0.0252}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2.hi.4\endcsname{-0.0150}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.cr.bn.fa.rnd.V2.lo.4\endcsname{-0.0361}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT.hi.4\endcsname{0.0029}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.IT.lo.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.LOC.lo.4\endcsname{-0.0042}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1.4\endcsname{-0.0179}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1.hi\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1.hi.4\endcsname{-0.0130}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V1.lo.4\endcsname{-0.0229}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2.4\endcsname{-0.0110}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2.hi.4\endcsname{-0.0077}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.bn.fa.stdp.V2.lo.4\endcsname{-0.0146}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT.hi.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.IT.lo.4\endcsname{-0.0072}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC.hi.4\endcsname{0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.LOC.lo.4\endcsname{-0.0097}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1.hi.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V1.lo.4\endcsname{-0.0149}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2.hi.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.bn.pc.bp.V2.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT.hi.4\endcsname{0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.IT.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC.4\endcsname{+0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.LOC.lo.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1.4\endcsname{+0.0033}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1.hi.4\endcsname{0.0054}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V1.lo.4\endcsname{0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2.4\endcsname{+0.0021}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2.hi.4\endcsname{0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.cr.bn.pc.fa.V2.lo.4\endcsname{0.0005}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT.hi.4\endcsname{0.0115}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.IT.lo.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC.4\endcsname{+0.0073}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC.hi.4\endcsname{0.0137}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.LOC.lo.4\endcsname{0.0013}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1\endcsname{-0.041}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1.4\endcsname{-0.0413}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1.hi\endcsname{-0.029}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1.hi.4\endcsname{-0.0292}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1.lo\endcsname{-0.053}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V1.lo.4\endcsname{-0.0533}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2.4\endcsname{-0.0231}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2.hi.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2.lo\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.cr.bn.pc.rnd.V2.lo.4\endcsname{-0.0327}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT.4\endcsname{-0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT.hi.4\endcsname{0.0022}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.IT.lo.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC.4\endcsname{+0.0000}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.LOC.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1.4\endcsname{-0.0146}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1.hi\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1.hi.4\endcsname{-0.0105}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V1.lo.4\endcsname{-0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2.4\endcsname{-0.0089}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2.hi.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.bn.pc.stdp.V2.lo.4\endcsname{-0.0119}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT.hi.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.IT.lo.4\endcsname{-0.0144}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC.4\endcsname{-0.0110}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC.hi.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.LOC.lo.4\endcsname{-0.0206}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1\endcsname{+0.031}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1.4\endcsname{+0.0308}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1.hi\endcsname{0.043}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1.hi.4\endcsname{0.0428}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V1.lo.4\endcsname{0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2.4\endcsname{+0.0165}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2.hi.4\endcsname{0.0261}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.bp.V2.lo.4\endcsname{0.0072}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT.hi.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.IT.lo.4\endcsname{-0.0118}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC.hi.4\endcsname{0.0002}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.LOC.lo.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1\endcsname{+0.045}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1.4\endcsname{+0.0446}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1.hi\endcsname{0.058}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1.hi.4\endcsname{0.0580}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1.lo\endcsname{0.031}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V1.lo.4\endcsname{0.0313}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2\endcsname{+0.025}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2.4\endcsname{+0.0252}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2.hi.4\endcsname{0.0361}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2.lo\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.fa.V2.lo.4\endcsname{0.0150}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT.hi.4\endcsname{0.0041}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.IT.lo.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC.hi.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.LOC.lo.4\endcsname{-0.0137}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1\endcsname{+0.041}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1.4\endcsname{+0.0413}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1.hi\endcsname{0.053}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1.hi.4\endcsname{0.0533}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1.lo\endcsname{0.029}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V1.lo.4\endcsname{0.0292}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2\endcsname{+0.023}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2.4\endcsname{+0.0231}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2.hi\endcsname{0.033}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2.hi.4\endcsname{0.0327}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2.lo\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.pc.V2.lo.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT.hi.4\endcsname{0.0028}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.IT.lo.4\endcsname{-0.0123}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC.hi.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.LOC.lo.4\endcsname{-0.0138}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1\endcsname{+0.027}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1.4\endcsname{+0.0267}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1.hi\endcsname{0.038}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1.hi.4\endcsname{0.0381}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1.lo\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V1.lo.4\endcsname{0.0154}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2.4\endcsname{+0.0142}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2.hi\endcsname{0.024}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2.hi.4\endcsname{0.0238}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.rnd.stdp.V2.lo.4\endcsname{0.0051}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT.hi.4\endcsname{0.0043}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.IT.lo.4\endcsname{-0.0056}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC.hi.4\endcsname{0.0017}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.LOC.lo.4\endcsname{-0.0097}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1.4\endcsname{+0.0042}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1.hi.4\endcsname{0.0079}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V1.lo.4\endcsname{0.0004}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2.4\endcsname{+0.0023}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.bp.V2.lo.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT.4\endcsname{+0.0009}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT.hi.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.IT.lo.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC.4\endcsname{+0.0007}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC.hi.4\endcsname{0.0042}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.LOC.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1\endcsname{+0.018}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1.4\endcsname{+0.0179}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1.hi\endcsname{0.023}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1.hi.4\endcsname{0.0229}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V1.lo.4\endcsname{0.0130}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2.4\endcsname{+0.0110}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2.hi.4\endcsname{0.0146}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.fa.V2.lo.4\endcsname{0.0077}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT.4\endcsname{+0.0011}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT.hi.4\endcsname{0.0045}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.IT.lo.4\endcsname{-0.0022}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC.4\endcsname{-0.0000}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.LOC.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1.4\endcsname{+0.0146}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1.hi\endcsname{0.019}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1.hi.4\endcsname{0.0186}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1.lo\endcsname{0.011}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V1.lo.4\endcsname{0.0105}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2.4\endcsname{+0.0089}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2.hi.4\endcsname{0.0119}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.pc.V2.lo.4\endcsname{0.0062}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT.4\endcsname{+0.0048}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT.hi.4\endcsname{0.0123}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.IT.lo.4\endcsname{-0.0028}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC.4\endcsname{+0.0073}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC.hi.4\endcsname{0.0138}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.LOC.lo.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1.4\endcsname{-0.0267}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1.hi.4\endcsname{-0.0154}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1.lo\endcsname{-0.038}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V1.lo.4\endcsname{-0.0381}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2.hi.4\endcsname{-0.0051}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.ps.cr.bn.stdp.rnd.V2.lo.4\endcsname{-0.0238}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT.4\endcsname{+0.0021}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT.hi.4\endcsname{0.0084}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.IT.lo.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC.4\endcsname{+0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC.hi.4\endcsname{0.0100}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.LOC.lo.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1.4\endcsname{+0.0152}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1.hi.4\endcsname{0.0206}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V1.lo.4\endcsname{0.0102}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2.4\endcsname{+0.0098}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2.hi.4\endcsname{0.0142}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.bp.fa.V2.lo.4\endcsname{0.0060}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT.hi.4\endcsname{0.0079}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.IT.lo.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC.4\endcsname{+0.0041}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC.hi.4\endcsname{0.0127}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.LOC.lo.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1.4\endcsname{-0.0148}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1.hi.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1.lo\endcsname{-0.025}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V1.lo.4\endcsname{-0.0245}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2.hi.4\endcsname{0.0031}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.cr.ref.bp.pc.V2.lo.4\endcsname{-0.0132}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT.4\endcsname{+0.0060}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT.hi.4\endcsname{0.0153}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.IT.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC.4\endcsname{+0.0105}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC.hi\endcsname{0.020}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC.hi.4\endcsname{0.0202}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.LOC.lo.4\endcsname{0.0017}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1\endcsname{-0.029}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1.4\endcsname{-0.0292}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1.hi.4\endcsname{-0.0164}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1.lo\endcsname{-0.041}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V1.lo.4\endcsname{-0.0412}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2.4\endcsname{-0.0155}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2.hi.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2.lo\endcsname{-0.025}
\expandafter\def\csname nv@d.ps.cr.ref.bp.rnd.V2.lo.4\endcsname{-0.0252}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT.4\endcsname{+0.0030}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT.hi.4\endcsname{0.0101}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.IT.lo.4\endcsname{-0.0046}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC.4\endcsname{+0.0040}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC.hi.4\endcsname{0.0115}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.LOC.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1.4\endcsname{-0.0205}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1.hi\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1.hi.4\endcsname{-0.0123}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1.lo\endcsname{-0.028}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V1.lo.4\endcsname{-0.0283}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2.hi.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2.lo\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.cr.ref.bp.stdp.V2.lo.4\endcsname{-0.0168}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT.hi.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.IT.lo.4\endcsname{-0.0084}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC.hi.4\endcsname{0.0018}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.LOC.lo.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1.4\endcsname{-0.0152}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1.hi.4\endcsname{-0.0102}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V1.lo.4\endcsname{-0.0206}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2.4\endcsname{-0.0098}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2.hi.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.ref.fa.bp.V2.lo.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT.hi.4\endcsname{0.0055}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.IT.lo.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC.4\endcsname{+0.0002}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC.hi.4\endcsname{0.0059}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.LOC.lo.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1\endcsname{-0.030}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1.4\endcsname{-0.0300}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1.hi\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1.hi.4\endcsname{-0.0197}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1.lo\endcsname{-0.040}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V1.lo.4\endcsname{-0.0398}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2.4\endcsname{-0.0150}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2.hi.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.cr.ref.fa.pc.V2.lo.4\endcsname{-0.0229}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT.4\endcsname{+0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT.hi.4\endcsname{0.0117}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.IT.lo.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC.4\endcsname{+0.0066}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC.hi.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.LOC.lo.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1\endcsname{-0.044}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1.4\endcsname{-0.0445}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1.hi\endcsname{-0.031}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1.hi.4\endcsname{-0.0313}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V1.lo.4\endcsname{-0.0578}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2\endcsname{-0.025}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2.4\endcsname{-0.0253}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2.hi.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.cr.ref.fa.rnd.V2.lo.4\endcsname{-0.0360}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT.4\endcsname{+0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT.hi.4\endcsname{0.0069}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.IT.lo.4\endcsname{-0.0062}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC.hi.4\endcsname{0.0053}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.LOC.lo.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1.4\endcsname{-0.0358}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1.hi\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1.hi.4\endcsname{-0.0267}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1.lo\endcsname{-0.045}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V1.lo.4\endcsname{-0.0451}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2.hi\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2.hi.4\endcsname{-0.0131}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2.lo\endcsname{-0.028}
\expandafter\def\csname nv@d.ps.cr.ref.fa.stdp.V2.lo.4\endcsname{-0.0277}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT.hi.4\endcsname{0.0054}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.IT.lo.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC.hi.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.LOC.lo.4\endcsname{-0.0127}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1.4\endcsname{+0.0148}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1.hi\endcsname{0.025}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1.hi.4\endcsname{0.0245}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V1.lo.4\endcsname{0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2.hi.4\endcsname{0.0132}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.pc.bp.V2.lo.4\endcsname{-0.0031}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT.4\endcsname{+0.0004}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT.hi.4\endcsname{0.0062}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.IT.lo.4\endcsname{-0.0055}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC.hi.4\endcsname{0.0059}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.LOC.lo.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1\endcsname{+0.030}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1.4\endcsname{+0.0300}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1.hi\endcsname{0.040}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1.hi.4\endcsname{0.0398}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1.lo\endcsname{0.020}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V1.lo.4\endcsname{0.0197}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2.4\endcsname{+0.0150}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2.hi\endcsname{0.023}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2.hi.4\endcsname{0.0229}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.cr.ref.pc.fa.V2.lo.4\endcsname{0.0068}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT.4\endcsname{+0.0044}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT.hi.4\endcsname{0.0108}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.IT.lo.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC.4\endcsname{+0.0065}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC.hi.4\endcsname{0.0117}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.LOC.lo.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1.4\endcsname{-0.0144}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1.hi.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1.lo\endcsname{-0.022}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V1.lo.4\endcsname{-0.0215}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2.hi.4\endcsname{-0.0046}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.cr.ref.pc.rnd.V2.lo.4\endcsname{-0.0163}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT.4\endcsname{+0.0013}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT.hi.4\endcsname{0.0044}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.IT.lo.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC.hi.4\endcsname{0.0026}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.LOC.lo.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1.hi.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V1.lo.4\endcsname{-0.0099}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2.hi.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.ref.pc.stdp.V2.lo.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.IT.lo.4\endcsname{-0.0153}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC.4\endcsname{-0.0105}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC.hi.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC.lo\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.LOC.lo.4\endcsname{-0.0202}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1\endcsname{+0.029}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1.4\endcsname{+0.0292}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1.hi\endcsname{0.041}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1.hi.4\endcsname{0.0412}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1.lo\endcsname{0.016}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V1.lo.4\endcsname{0.0164}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2.4\endcsname{+0.0155}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2.hi\endcsname{0.025}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2.hi.4\endcsname{0.0252}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.bp.V2.lo.4\endcsname{0.0058}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT.hi.4\endcsname{0.0038}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.IT.lo.4\endcsname{-0.0117}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC.4\endcsname{-0.0066}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC.hi.4\endcsname{0.0002}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.LOC.lo.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1\endcsname{+0.044}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1.4\endcsname{+0.0445}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1.hi\endcsname{0.058}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1.hi.4\endcsname{0.0578}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1.lo\endcsname{0.031}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V1.lo.4\endcsname{0.0313}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2\endcsname{+0.025}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2.4\endcsname{+0.0253}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2.hi.4\endcsname{0.0360}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2.lo\endcsname{0.015}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.fa.V2.lo.4\endcsname{0.0151}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT.hi.4\endcsname{0.0015}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.IT.lo.4\endcsname{-0.0108}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC.hi.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.LOC.lo.4\endcsname{-0.0117}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1.4\endcsname{+0.0144}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1.hi\endcsname{0.022}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1.hi.4\endcsname{0.0215}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V1.lo.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2.4\endcsname{+0.0103}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2.hi\endcsname{0.016}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2.hi.4\endcsname{0.0163}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.pc.V2.lo.4\endcsname{0.0046}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT.hi.4\endcsname{0.0021}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.IT.lo.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC.4\endcsname{-0.0065}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC.hi.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.LOC.lo.4\endcsname{-0.0122}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1.4\endcsname{+0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1.hi\endcsname{0.016}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1.hi.4\endcsname{0.0162}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V1.lo.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2.4\endcsname{+0.0051}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2.hi.4\endcsname{0.0116}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.rnd.stdp.V2.lo.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT.hi.4\endcsname{0.0046}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.IT.lo.4\endcsname{-0.0101}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC.4\endcsname{-0.0040}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.LOC.lo.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1\endcsname{+0.021}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1.4\endcsname{+0.0205}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1.hi\endcsname{0.028}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1.hi.4\endcsname{0.0283}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1.lo\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V1.lo.4\endcsname{0.0123}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2.4\endcsname{+0.0104}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2.hi.4\endcsname{0.0168}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.bp.V2.lo.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT.hi.4\endcsname{0.0062}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.IT.lo.4\endcsname{-0.0069}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC.hi.4\endcsname{0.0049}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.LOC.lo.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1\endcsname{+0.036}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1.4\endcsname{+0.0358}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1.hi\endcsname{0.045}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1.hi.4\endcsname{0.0451}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1.lo\endcsname{0.027}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V1.lo.4\endcsname{0.0267}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2\endcsname{+0.020}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2.4\endcsname{+0.0202}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2.hi\endcsname{0.028}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2.hi.4\endcsname{0.0277}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2.lo\endcsname{0.013}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.fa.V2.lo.4\endcsname{0.0131}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT.hi.4\endcsname{0.0017}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.IT.lo.4\endcsname{-0.0044}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC.hi.4\endcsname{0.0026}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.LOC.lo.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1.4\endcsname{+0.0058}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1.hi.4\endcsname{0.0099}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V1.lo.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2.hi.4\endcsname{0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.pc.V2.lo.4\endcsname{0.0020}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT.4\endcsname{+0.0030}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT.hi.4\endcsname{0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.IT.lo.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC.4\endcsname{+0.0065}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC.hi.4\endcsname{0.0122}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.LOC.lo.4\endcsname{0.0012}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1.hi.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V1.lo.4\endcsname{-0.0162}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2.4\endcsname{-0.0051}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2.hi.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.cr.ref.stdp.rnd.V2.lo.4\endcsname{-0.0116}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT.4\endcsname{+0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT.hi.4\endcsname{0.0079}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.IT.lo.4\endcsname{-0.0025}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC.4\endcsname{+0.0050}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC.hi.4\endcsname{0.0102}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.LOC.lo.4\endcsname{0.0001}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1.4\endcsname{+0.0144}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1.hi\endcsname{0.019}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1.hi.4\endcsname{0.0193}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V1.lo.4\endcsname{0.0097}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2.4\endcsname{+0.0089}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2.hi.4\endcsname{0.0128}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.bn.bp.fa.V2.lo.4\endcsname{0.0054}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT.4\endcsname{+0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT.hi.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.IT.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC.4\endcsname{+0.0047}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC.hi.4\endcsname{0.0099}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.LOC.lo.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1.4\endcsname{+0.0111}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1.hi.4\endcsname{0.0153}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V1.lo.4\endcsname{0.0068}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2.4\endcsname{+0.0068}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2.hi.4\endcsname{0.0103}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.bp.pc.V2.lo.4\endcsname{0.0038}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT\endcsname{+0.006}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT.4\endcsname{+0.0061}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT.hi.4\endcsname{0.0144}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.IT.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC\endcsname{+0.012}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC.4\endcsname{+0.0125}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC.hi.4\endcsname{0.0206}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.LOC.lo.4\endcsname{0.0050}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1.4\endcsname{-0.0327}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1.hi\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1.hi.4\endcsname{-0.0211}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1.lo\endcsname{-0.044}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V1.lo.4\endcsname{-0.0437}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2.4\endcsname{-0.0178}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2.hi.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.crb.bn.bp.rnd.V2.lo.4\endcsname{-0.0262}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT.4\endcsname{+0.0012}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT.hi.4\endcsname{0.0058}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.IT.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC.4\endcsname{+0.0043}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC.hi.4\endcsname{0.0096}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.LOC.lo.4\endcsname{-0.0007}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1.hi.4\endcsname{0.0004}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V1.lo.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2.hi.4\endcsname{0.0009}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.bp.stdp.V2.lo.4\endcsname{-0.0046}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT.hi.4\endcsname{0.0025}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.IT.lo.4\endcsname{-0.0079}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC.hi.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.LOC.lo.4\endcsname{-0.0102}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1.4\endcsname{-0.0144}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1.hi.4\endcsname{-0.0097}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V1.lo.4\endcsname{-0.0193}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2.4\endcsname{-0.0089}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2.hi.4\endcsname{-0.0054}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.crb.bn.fa.bp.V2.lo.4\endcsname{-0.0128}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT.hi.4\endcsname{0.0034}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.IT.lo.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC.hi.4\endcsname{0.0021}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.LOC.lo.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1.4\endcsname{-0.0033}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1.hi.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V1.lo.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2.hi\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2.hi.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.fa.pc.V2.lo.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT.4\endcsname{+0.0034}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT.hi.4\endcsname{0.0104}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.IT.lo.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC.4\endcsname{+0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC.hi.4\endcsname{0.0142}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.LOC.lo.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1\endcsname{-0.047}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1.4\endcsname{-0.0471}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1.hi\endcsname{-0.034}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1.hi.4\endcsname{-0.0336}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V1.lo.4\endcsname{-0.0591}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2.4\endcsname{-0.0267}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2.hi\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2.hi.4\endcsname{-0.0172}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.crb.bn.fa.rnd.V2.lo.4\endcsname{-0.0361}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT.hi.4\endcsname{0.0020}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.IT.lo.4\endcsname{-0.0053}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC.4\endcsname{-0.0006}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC.hi.4\endcsname{0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.LOC.lo.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1.4\endcsname{-0.0179}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1.hi\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1.hi.4\endcsname{-0.0128}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1.lo\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V1.lo.4\endcsname{-0.0229}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2.4\endcsname{-0.0108}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2.hi.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.bn.fa.stdp.V2.lo.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.IT.lo.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC.hi.4\endcsname{0.0001}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.LOC.lo.4\endcsname{-0.0099}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1.4\endcsname{-0.0111}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1.hi.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V1.lo.4\endcsname{-0.0153}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2.hi.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.pc.bp.V2.lo.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT.hi.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.IT.lo.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC.hi.4\endcsname{0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.LOC.lo.4\endcsname{-0.0021}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1.4\endcsname{+0.0033}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1.hi.4\endcsname{0.0053}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V1.lo.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2.4\endcsname{+0.0021}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2.lo\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.bn.pc.fa.V2.lo.4\endcsname{0.0005}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT.4\endcsname{+0.0037}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT.hi.4\endcsname{0.0103}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.IT.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC.4\endcsname{+0.0078}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC.hi.4\endcsname{0.0135}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC.lo\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.LOC.lo.4\endcsname{0.0026}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1\endcsname{-0.044}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1.4\endcsname{-0.0438}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1.hi\endcsname{-0.032}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1.hi.4\endcsname{-0.0319}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1.lo\endcsname{-0.055}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V1.lo.4\endcsname{-0.0547}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2\endcsname{-0.025}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2.4\endcsname{-0.0246}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2.hi\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2.hi.4\endcsname{-0.0162}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2.lo\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.crb.bn.pc.rnd.V2.lo.4\endcsname{-0.0332}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT.hi.4\endcsname{0.0018}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.IT.lo.4\endcsname{-0.0043}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC.hi.4\endcsname{0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.LOC.lo.4\endcsname{-0.0032}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1.4\endcsname{-0.0145}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1.hi.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V1.lo.4\endcsname{-0.0185}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2.hi.4\endcsname{-0.0061}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2.lo\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.crb.bn.pc.stdp.V2.lo.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT.4\endcsname{-0.0061}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.IT.lo.4\endcsname{-0.0144}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC.4\endcsname{-0.0125}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC.hi.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.LOC.lo.4\endcsname{-0.0206}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1\endcsname{+0.033}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1.4\endcsname{+0.0327}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1.hi\endcsname{0.044}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1.hi.4\endcsname{0.0437}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1.lo\endcsname{0.021}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V1.lo.4\endcsname{0.0211}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2\endcsname{+0.018}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2.4\endcsname{+0.0178}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2.hi.4\endcsname{0.0262}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.bp.V2.lo.4\endcsname{0.0091}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT.hi.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.IT.lo.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC.hi.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.LOC.lo.4\endcsname{-0.0142}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1\endcsname{+0.047}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1.4\endcsname{+0.0471}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1.hi\endcsname{0.059}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1.hi.4\endcsname{0.0591}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1.lo\endcsname{0.034}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V1.lo.4\endcsname{0.0336}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2\endcsname{+0.027}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2.4\endcsname{+0.0267}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2.hi.4\endcsname{0.0361}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2.lo\endcsname{0.017}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.fa.V2.lo.4\endcsname{0.0172}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT.4\endcsname{-0.0037}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.IT.lo.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC.hi\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC.hi.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.LOC.lo.4\endcsname{-0.0135}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1\endcsname{+0.044}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1.4\endcsname{+0.0438}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1.hi\endcsname{0.055}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1.hi.4\endcsname{0.0547}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1.lo\endcsname{0.032}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V1.lo.4\endcsname{0.0319}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2\endcsname{+0.025}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2.4\endcsname{+0.0246}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2.hi\endcsname{0.033}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2.hi.4\endcsname{0.0332}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2.lo\endcsname{0.016}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.pc.V2.lo.4\endcsname{0.0162}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT.4\endcsname{-0.0049}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT.hi.4\endcsname{0.0016}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.IT.lo.4\endcsname{-0.0114}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC.4\endcsname{-0.0081}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC.hi.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.LOC.lo.4\endcsname{-0.0139}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1\endcsname{+0.029}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1.4\endcsname{+0.0293}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1.hi\endcsname{0.040}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1.hi.4\endcsname{0.0397}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V1.lo.4\endcsname{0.0187}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2\endcsname{+0.016}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2.4\endcsname{+0.0159}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2.hi\endcsname{0.024}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2.hi.4\endcsname{0.0239}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.crb.bn.rnd.stdp.V2.lo.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT.4\endcsname{-0.0012}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT.hi.4\endcsname{0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.IT.lo.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC.4\endcsname{-0.0043}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC.hi.4\endcsname{0.0007}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.LOC.lo.4\endcsname{-0.0096}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1.4\endcsname{+0.0035}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1.hi.4\endcsname{0.0073}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V1.lo.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2.4\endcsname{+0.0019}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2.hi.4\endcsname{0.0046}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.bp.V2.lo.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT.4\endcsname{+0.0016}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT.hi.4\endcsname{0.0053}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.IT.lo.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC.4\endcsname{+0.0006}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC.hi.4\endcsname{0.0038}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.LOC.lo.4\endcsname{-0.0027}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1\endcsname{+0.018}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1.4\endcsname{+0.0179}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1.hi\endcsname{0.023}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1.hi.4\endcsname{0.0229}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V1.lo.4\endcsname{0.0128}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2\endcsname{+0.011}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2.4\endcsname{+0.0108}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2.hi.4\endcsname{0.0142}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.fa.V2.lo.4\endcsname{0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT.4\endcsname{+0.0012}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT.hi.4\endcsname{0.0043}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.IT.lo.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC.4\endcsname{+0.0003}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC.hi.4\endcsname{0.0032}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.LOC.lo.4\endcsname{-0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1\endcsname{+0.015}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1.4\endcsname{+0.0145}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1.hi\endcsname{0.019}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1.hi.4\endcsname{0.0185}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V1.lo.4\endcsname{0.0104}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2.4\endcsname{+0.0087}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2.hi.4\endcsname{0.0115}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.pc.V2.lo.4\endcsname{0.0061}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT.4\endcsname{+0.0049}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT.hi.4\endcsname{0.0114}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.IT.lo.4\endcsname{-0.0016}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC.4\endcsname{+0.0081}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC.hi.4\endcsname{0.0139}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.LOC.lo.4\endcsname{0.0024}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1\endcsname{-0.029}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1.4\endcsname{-0.0293}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1.hi.4\endcsname{-0.0187}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1.lo\endcsname{-0.040}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V1.lo.4\endcsname{-0.0397}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2.4\endcsname{-0.0159}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2.hi.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.ps.crb.bn.stdp.rnd.V2.lo.4\endcsname{-0.0239}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT.4\endcsname{+0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT.hi.4\endcsname{0.0086}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.IT.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC.4\endcsname{+0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC.hi.4\endcsname{0.0104}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.LOC.lo.4\endcsname{-0.0003}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1\endcsname{+0.016}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1.4\endcsname{+0.0156}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1.hi.4\endcsname{0.0210}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V1.lo.4\endcsname{0.0103}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2\endcsname{+0.010}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2.4\endcsname{+0.0097}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2.hi.4\endcsname{0.0140}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.crb.ref.bp.fa.V2.lo.4\endcsname{0.0059}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT.4\endcsname{+0.0015}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT.hi.4\endcsname{0.0074}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.IT.lo.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC.4\endcsname{+0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC.hi.4\endcsname{0.0115}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.LOC.lo.4\endcsname{-0.0029}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1.4\endcsname{-0.0175}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1.hi.4\endcsname{-0.0078}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V1.lo.4\endcsname{-0.0264}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2.4\endcsname{-0.0076}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2.hi.4\endcsname{0.0002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.ref.bp.pc.V2.lo.4\endcsname{-0.0150}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT.4\endcsname{+0.0068}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT.hi.4\endcsname{0.0151}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.IT.lo.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC\endcsname{+0.012}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC.4\endcsname{+0.0123}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC.hi.4\endcsname{0.0209}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC.lo\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.LOC.lo.4\endcsname{0.0045}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1\endcsname{-0.031}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1.4\endcsname{-0.0313}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1.hi\endcsname{-0.020}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1.hi.4\endcsname{-0.0196}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1.lo\endcsname{-0.042}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V1.lo.4\endcsname{-0.0422}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2.4\endcsname{-0.0170}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2.hi.4\endcsname{-0.0083}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@d.ps.crb.ref.bp.rnd.V2.lo.4\endcsname{-0.0256}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT.4\endcsname{+0.0020}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT.hi.4\endcsname{0.0090}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.IT.lo.4\endcsname{-0.0046}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC.4\endcsname{+0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC.hi.4\endcsname{0.0105}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.LOC.lo.4\endcsname{-0.0019}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1\endcsname{-0.022}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1.4\endcsname{-0.0222}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1.hi\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1.hi.4\endcsname{-0.0143}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1.lo\endcsname{-0.030}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V1.lo.4\endcsname{-0.0298}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2.4\endcsname{-0.0121}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2.hi.4\endcsname{-0.0058}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2.lo\endcsname{-0.018}
\expandafter\def\csname nv@d.ps.crb.ref.bp.stdp.V2.lo.4\endcsname{-0.0182}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.IT.lo.4\endcsname{-0.0086}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC.hi.4\endcsname{0.0003}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.LOC.lo.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1.4\endcsname{-0.0156}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1.hi.4\endcsname{-0.0103}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V1.lo.4\endcsname{-0.0210}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2.4\endcsname{-0.0097}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2.hi.4\endcsname{-0.0059}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.ref.fa.bp.V2.lo.4\endcsname{-0.0140}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT.4\endcsname{-0.0018}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT.hi.4\endcsname{0.0030}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.IT.lo.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC.hi.4\endcsname{0.0041}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.LOC.lo.4\endcsname{-0.0060}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1.4\endcsname{-0.0331}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1.hi\endcsname{-0.023}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1.hi.4\endcsname{-0.0233}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1.lo\endcsname{-0.042}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V1.lo.4\endcsname{-0.0422}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2.4\endcsname{-0.0173}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2.hi\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2.hi.4\endcsname{-0.0100}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@d.ps.crb.ref.fa.pc.V2.lo.4\endcsname{-0.0245}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT\endcsname{+0.003}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT.4\endcsname{+0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT.hi.4\endcsname{0.0104}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.IT.lo.4\endcsname{-0.0038}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC\endcsname{+0.007}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC.4\endcsname{+0.0075}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC.hi.4\endcsname{0.0141}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.LOC.lo.4\endcsname{0.0014}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1\endcsname{-0.047}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1.4\endcsname{-0.0469}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1.hi\endcsname{-0.033}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1.hi.4\endcsname{-0.0334}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V1.lo.4\endcsname{-0.0590}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2\endcsname{-0.027}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2.4\endcsname{-0.0267}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2.hi\endcsname{-0.017}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2.hi.4\endcsname{-0.0172}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2.lo\endcsname{-0.036}
\expandafter\def\csname nv@d.ps.crb.ref.fa.rnd.V2.lo.4\endcsname{-0.0360}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT.4\endcsname{-0.0013}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT.hi.4\endcsname{0.0042}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.IT.lo.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC.4\endcsname{-0.0009}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC.hi.4\endcsname{0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.LOC.lo.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1\endcsname{-0.038}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1.4\endcsname{-0.0379}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1.hi\endcsname{-0.029}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1.hi.4\endcsname{-0.0286}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1.lo\endcsname{-0.046}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V1.lo.4\endcsname{-0.0465}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2\endcsname{-0.022}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2.4\endcsname{-0.0217}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2.hi\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2.hi.4\endcsname{-0.0147}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2.lo\endcsname{-0.028}
\expandafter\def\csname nv@d.ps.crb.ref.fa.stdp.V2.lo.4\endcsname{-0.0285}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT.hi.4\endcsname{0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.IT.lo.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC.hi.4\endcsname{0.0029}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.LOC.lo.4\endcsname{-0.0115}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1\endcsname{+0.017}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1.4\endcsname{+0.0175}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1.hi.4\endcsname{0.0264}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V1.lo.4\endcsname{0.0078}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2.4\endcsname{+0.0076}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2.hi.4\endcsname{0.0150}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.pc.bp.V2.lo.4\endcsname{-0.0002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT.4\endcsname{+0.0018}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT.hi.4\endcsname{0.0068}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.IT.lo.4\endcsname{-0.0030}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC.4\endcsname{+0.0010}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC.hi.4\endcsname{0.0060}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.LOC.lo.4\endcsname{-0.0041}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1\endcsname{+0.033}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1.4\endcsname{+0.0331}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1.hi\endcsname{0.042}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1.hi.4\endcsname{0.0422}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1.lo\endcsname{0.023}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V1.lo.4\endcsname{0.0233}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2.4\endcsname{+0.0173}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2.hi\endcsname{0.024}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2.hi.4\endcsname{0.0245}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2.lo\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.ref.pc.fa.V2.lo.4\endcsname{0.0100}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT.4\endcsname{+0.0052}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT.hi.4\endcsname{0.0112}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.IT.lo.4\endcsname{-0.0004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC.4\endcsname{+0.0085}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC.hi.4\endcsname{0.0135}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.LOC.lo.4\endcsname{0.0036}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1.4\endcsname{-0.0139}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1.hi\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1.hi.4\endcsname{-0.0073}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V1.lo.4\endcsname{-0.0207}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2.4\endcsname{-0.0094}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2.hi.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.ref.pc.rnd.V2.lo.4\endcsname{-0.0153}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT.4\endcsname{+0.0005}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT.hi.4\endcsname{0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.IT.lo.4\endcsname{-0.0023}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC.4\endcsname{+0.0001}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC.hi.4\endcsname{0.0026}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.LOC.lo.4\endcsname{-0.0025}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1.4\endcsname{-0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1.hi.4\endcsname{-0.0008}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V1.lo.4\endcsname{-0.0087}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2.hi.4\endcsname{-0.0015}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2.lo\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.pc.stdp.V2.lo.4\endcsname{-0.0074}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT.4\endcsname{-0.0068}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT.hi.4\endcsname{0.0019}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT.lo\endcsname{-0.015}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.IT.lo.4\endcsname{-0.0151}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC\endcsname{-0.012}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC.4\endcsname{-0.0123}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC.hi\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC.hi.4\endcsname{-0.0045}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.LOC.lo.4\endcsname{-0.0209}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1\endcsname{+0.031}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1.4\endcsname{+0.0313}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1.hi\endcsname{0.042}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1.hi.4\endcsname{0.0422}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1.lo\endcsname{0.020}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V1.lo.4\endcsname{0.0196}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2\endcsname{+0.017}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2.4\endcsname{+0.0170}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2.hi\endcsname{0.026}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2.hi.4\endcsname{0.0256}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.bp.V2.lo.4\endcsname{0.0083}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT.hi.4\endcsname{0.0038}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.IT.lo.4\endcsname{-0.0104}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC\endcsname{-0.007}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC.4\endcsname{-0.0075}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC.hi.4\endcsname{-0.0014}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC.lo\endcsname{-0.014}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.LOC.lo.4\endcsname{-0.0141}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1\endcsname{+0.047}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1.4\endcsname{+0.0469}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1.hi\endcsname{0.059}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1.hi.4\endcsname{0.0590}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1.lo\endcsname{0.033}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V1.lo.4\endcsname{0.0334}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2\endcsname{+0.027}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2.4\endcsname{+0.0267}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2.hi.4\endcsname{0.0360}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2.lo\endcsname{0.017}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.fa.V2.lo.4\endcsname{0.0172}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT.4\endcsname{-0.0052}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT.hi.4\endcsname{0.0004}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.IT.lo.4\endcsname{-0.0112}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC.4\endcsname{-0.0085}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC.hi.4\endcsname{-0.0036}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.LOC.lo.4\endcsname{-0.0135}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1\endcsname{+0.014}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1.4\endcsname{+0.0139}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1.hi\endcsname{0.021}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1.hi.4\endcsname{0.0207}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1.lo\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V1.lo.4\endcsname{0.0073}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2.4\endcsname{+0.0094}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2.hi\endcsname{0.015}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2.hi.4\endcsname{0.0153}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.pc.V2.lo.4\endcsname{0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT.4\endcsname{-0.0047}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT.hi\endcsname{0.000}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT.hi.4\endcsname{0.0001}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.IT.lo.4\endcsname{-0.0099}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC\endcsname{-0.008}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC.4\endcsname{-0.0084}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC.hi\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC.hi.4\endcsname{-0.0035}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC.lo\endcsname{-0.013}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.LOC.lo.4\endcsname{-0.0134}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1\endcsname{+0.009}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1.4\endcsname{+0.0091}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1.hi\endcsname{0.016}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1.hi.4\endcsname{0.0161}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V1.lo.4\endcsname{0.0017}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2.4\endcsname{+0.0050}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2.hi.4\endcsname{0.0109}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@d.ps.crb.ref.rnd.stdp.V2.lo.4\endcsname{-0.0010}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT.4\endcsname{-0.0020}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT.hi.4\endcsname{0.0046}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.IT.lo.4\endcsname{-0.0090}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC.4\endcsname{-0.0039}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC.hi.4\endcsname{0.0019}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.LOC.lo.4\endcsname{-0.0105}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1\endcsname{+0.022}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1.4\endcsname{+0.0222}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1.hi\endcsname{0.030}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1.hi.4\endcsname{0.0298}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1.lo\endcsname{0.014}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V1.lo.4\endcsname{0.0143}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2\endcsname{+0.012}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2.4\endcsname{+0.0121}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2.hi\endcsname{0.018}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2.hi.4\endcsname{0.0182}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.bp.V2.lo.4\endcsname{0.0058}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT.4\endcsname{+0.0013}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT.hi.4\endcsname{0.0073}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.IT.lo.4\endcsname{-0.0042}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC.4\endcsname{+0.0009}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC.hi.4\endcsname{0.0052}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.LOC.lo.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1\endcsname{+0.038}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1.4\endcsname{+0.0379}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1.hi\endcsname{0.046}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1.hi.4\endcsname{0.0465}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1.lo\endcsname{0.029}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V1.lo.4\endcsname{0.0286}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2\endcsname{+0.022}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2.4\endcsname{+0.0217}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2.hi\endcsname{0.028}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2.hi.4\endcsname{0.0285}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2.lo\endcsname{0.015}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.fa.V2.lo.4\endcsname{0.0147}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT.4\endcsname{-0.0005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT.hi.4\endcsname{0.0023}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.IT.lo.4\endcsname{-0.0034}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC.hi.4\endcsname{0.0025}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.LOC.lo.4\endcsname{-0.0026}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1.4\endcsname{+0.0048}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1.hi\endcsname{0.009}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1.hi.4\endcsname{0.0087}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1.lo\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V1.lo.4\endcsname{0.0008}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2\endcsname{+0.004}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2.4\endcsname{+0.0045}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2.hi\endcsname{0.007}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2.hi.4\endcsname{0.0074}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2.lo\endcsname{0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.pc.V2.lo.4\endcsname{0.0015}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT\endcsname{+0.005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT.4\endcsname{+0.0047}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT.hi.4\endcsname{0.0099}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT.lo\endcsname{-0.000}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.IT.lo.4\endcsname{-0.0001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC\endcsname{+0.008}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC.4\endcsname{+0.0084}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC.hi.4\endcsname{0.0134}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC.lo\endcsname{0.004}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.LOC.lo.4\endcsname{0.0035}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1\endcsname{-0.009}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1.4\endcsname{-0.0091}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1.hi\endcsname{-0.002}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1.hi.4\endcsname{-0.0017}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1.lo\endcsname{-0.016}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V1.lo.4\endcsname{-0.0161}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2\endcsname{-0.005}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2.4\endcsname{-0.0050}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2.hi.4\endcsname{0.0010}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2.lo\endcsname{-0.011}
\expandafter\def\csname nv@d.ps.crb.ref.stdp.rnd.V2.lo.4\endcsname{-0.0109}
\expandafter\def\csname nv@err.bp.V1\endcsname{0.033}
\expandafter\def\csname nv@err.bp.V2\endcsname{0.018}
\expandafter\def\csname nv@err.bp.V2.hi\endcsname{.022}
\expandafter\def\csname nv@err.gap.V1\endcsname{+0.042}
\expandafter\def\csname nv@err.gap.sweep\endcsname{+0.044}
\expandafter\def\csname nv@err.nsig\endcsname{26}
\expandafter\def\csname nv@err.pmax\endcsname{0.0144}
\expandafter\def\csname nv@err.rnd.V1\endcsname{0.075}
\expandafter\def\csname nv@err.seedsd.max\endcsname{0.011}
\expandafter\def\csname nv@err.seedsd.min\endcsname{0.003}
\expandafter\def\csname nv@fdr.bp.fa.V1.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.bp.fa.V1.bh_p_fam7\endcsname{0.0014}
\expandafter\def\csname nv@fdr.bp.fa.V1.d\endcsname{+0.0138}
\expandafter\def\csname nv@fdr.bp.fa.V1.hi\endcsname{0.0186}
\expandafter\def\csname nv@fdr.bp.fa.V1.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.bp.fa.V1.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.bp.fa.V1.lo\endcsname{0.0092}
\expandafter\def\csname nv@fdr.bp.fa.V1.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.bp.fa.V2.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.bp.fa.V2.d\endcsname{+0.0087}
\expandafter\def\csname nv@fdr.bp.fa.V2.hi\endcsname{0.0125}
\expandafter\def\csname nv@fdr.bp.fa.V2.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.bp.fa.V2.lo\endcsname{0.0053}
\expandafter\def\csname nv@fdr.bp.fa.V2.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.fa.pc.V1.bh_p_fam11\endcsname{0.0037}
\expandafter\def\csname nv@fdr.fa.pc.V1.bh_p_fam7\endcsname{0.0035}
\expandafter\def\csname nv@fdr.fa.pc.V1.d\endcsname{-0.0033}
\expandafter\def\csname nv@fdr.fa.pc.V1.hi\endcsname{-0.0011}
\expandafter\def\csname nv@fdr.fa.pc.V1.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.fa.pc.V1.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.fa.pc.V1.lo\endcsname{-0.0054}
\expandafter\def\csname nv@fdr.fa.pc.V1.p_boot\endcsname{0.0030}
\expandafter\def\csname nv@fdr.fa.pc.V2.bh_p_fam11\endcsname{0.0099}
\expandafter\def\csname nv@fdr.fa.pc.V2.d\endcsname{-0.0021}
\expandafter\def\csname nv@fdr.fa.pc.V2.hi\endcsname{-0.0005}
\expandafter\def\csname nv@fdr.fa.pc.V2.holm_p_fam11\endcsname{0.0180}
\expandafter\def\csname nv@fdr.fa.pc.V2.lo\endcsname{-0.0037}
\expandafter\def\csname nv@fdr.fa.pc.V2.p_boot\endcsname{0.0090}
\expandafter\def\csname nv@fdr.fa.stdp.V1.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.fa.stdp.V1.bh_p_fam7\endcsname{0.0014}
\expandafter\def\csname nv@fdr.fa.stdp.V1.d\endcsname{-0.0179}
\expandafter\def\csname nv@fdr.fa.stdp.V1.hi\endcsname{-0.0130}
\expandafter\def\csname nv@fdr.fa.stdp.V1.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.fa.stdp.V1.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.fa.stdp.V1.lo\endcsname{-0.0229}
\expandafter\def\csname nv@fdr.fa.stdp.V1.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.fa.stdp.V2.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.fa.stdp.V2.d\endcsname{-0.0110}
\expandafter\def\csname nv@fdr.fa.stdp.V2.hi\endcsname{-0.0077}
\expandafter\def\csname nv@fdr.fa.stdp.V2.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.fa.stdp.V2.lo\endcsname{-0.0146}
\expandafter\def\csname nv@fdr.fa.stdp.V2.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.bh_p_fam11\endcsname{0.0190}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.bh_p_fam7\endcsname{0.0190}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.d\endcsname{-0.0110}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.hi\endcsname{-0.0023}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.holm_p_fam11\endcsname{0.0190}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.holm_p_fam7\endcsname{0.0190}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.lo\endcsname{-0.0206}
\expandafter\def\csname nv@fdr.rnd.bp.LOC.p_boot\endcsname{0.0190}
\expandafter\def\csname nv@fdr.rnd.bp.V1.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.bp.V1.bh_p_fam7\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.bp.V1.d\endcsname{+0.0308}
\expandafter\def\csname nv@fdr.rnd.bp.V1.hi\endcsname{0.0428}
\expandafter\def\csname nv@fdr.rnd.bp.V1.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.rnd.bp.V1.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.rnd.bp.V1.lo\endcsname{0.0186}
\expandafter\def\csname nv@fdr.rnd.bp.V1.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.rnd.bp.V2.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.bp.V2.bh_p_fam7\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.bp.V2.d\endcsname{+0.0165}
\expandafter\def\csname nv@fdr.rnd.bp.V2.hi\endcsname{0.0261}
\expandafter\def\csname nv@fdr.rnd.bp.V2.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.rnd.bp.V2.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.rnd.bp.V2.lo\endcsname{0.0072}
\expandafter\def\csname nv@fdr.rnd.bp.V2.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.rnd.fa.V1.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.fa.V1.bh_p_fam7\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.fa.V1.d\endcsname{+0.0446}
\expandafter\def\csname nv@fdr.rnd.fa.V1.hi\endcsname{0.0580}
\expandafter\def\csname nv@fdr.rnd.fa.V1.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.rnd.fa.V1.holm_p_fam7\endcsname{0.0070}
\expandafter\def\csname nv@fdr.rnd.fa.V1.lo\endcsname{0.0313}
\expandafter\def\csname nv@fdr.rnd.fa.V1.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@fdr.rnd.fa.V2.bh_p_fam11\endcsname{0.0014}
\expandafter\def\csname nv@fdr.rnd.fa.V2.d\endcsname{+0.0252}
\expandafter\def\csname nv@fdr.rnd.fa.V2.hi\endcsname{0.0361}
\expandafter\def\csname nv@fdr.rnd.fa.V2.holm_p_fam11\endcsname{0.0110}
\expandafter\def\csname nv@fdr.rnd.fa.V2.lo\endcsname{0.0150}
\expandafter\def\csname nv@fdr.rnd.fa.V2.p_boot\endcsname{0.0010}
\expandafter\def\csname nv@gabor.bp.mean\endcsname{1.99}
\expandafter\def\csname nv@gabor.bp.std\endcsname{0.52}
\expandafter\def\csname nv@gabor.fa.mean\endcsname{1.82}
\expandafter\def\csname nv@gabor.fa.std\endcsname{0.36}
\expandafter\def\csname nv@gabor.pc.mean\endcsname{1.73}
\expandafter\def\csname nv@gabor.pc.std\endcsname{0.45}
\expandafter\def\csname nv@gabor.rnd.mean\endcsname{1.73}
\expandafter\def\csname nv@gabor.rnd.std\endcsname{0.45}
\expandafter\def\csname nv@gabor.stdp.mean\endcsname{1.79}
\expandafter\def\csname nv@gabor.stdp.std\endcsname{0.47}
\expandafter\def\csname nv@init.ratio\endcsname{2.4}
\expandafter\def\csname nv@lag.one.max\endcsname{1.030}
\expandafter\def\csname nv@lag.one.min\endcsname{0.998}
\expandafter\def\csname nv@lag.one.n\endcsname{5}
\expandafter\def\csname nv@lag.rho.max\endcsname{-0.10}
\expandafter\def\csname nv@lag.rho.min\endcsname{-0.30}
\expandafter\def\csname nv@lb.all.IT\endcsname{0.035}
\expandafter\def\csname nv@lb.all.IT.hi\endcsname{0.042}
\expandafter\def\csname nv@lb.all.IT.lo\endcsname{0.028}
\expandafter\def\csname nv@lb.all.LOC\endcsname{0.034}
\expandafter\def\csname nv@lb.all.LOC.hi\endcsname{0.042}
\expandafter\def\csname nv@lb.all.LOC.lo\endcsname{0.027}
\expandafter\def\csname nv@lb.all.V1\endcsname{0.057}
\expandafter\def\csname nv@lb.all.V1.hi\endcsname{0.069}
\expandafter\def\csname nv@lb.all.V1.lo\endcsname{0.045}
\expandafter\def\csname nv@lb.all.V2\endcsname{0.033}
\expandafter\def\csname nv@lb.all.V2.hi\endcsname{0.041}
\expandafter\def\csname nv@lb.all.V2.lo\endcsname{0.025}
\expandafter\def\csname nv@lb.cr.IT\endcsname{0.021}
\expandafter\def\csname nv@lb.cr.IT.hi\endcsname{0.028}
\expandafter\def\csname nv@lb.cr.IT.lo\endcsname{0.014}
\expandafter\def\csname nv@lb.cr.LOC\endcsname{0.018}
\expandafter\def\csname nv@lb.cr.LOC.hi\endcsname{0.027}
\expandafter\def\csname nv@lb.cr.LOC.lo\endcsname{0.011}
\expandafter\def\csname nv@lb.cr.V1\endcsname{0.051}
\expandafter\def\csname nv@lb.cr.V1.hi\endcsname{0.064}
\expandafter\def\csname nv@lb.cr.V1.lo\endcsname{0.039}
\expandafter\def\csname nv@lb.cr.V2\endcsname{0.024}
\expandafter\def\csname nv@lb.cr.V2.hi\endcsname{0.032}
\expandafter\def\csname nv@lb.cr.V2.lo\endcsname{0.016}
\expandafter\def\csname nv@lb.crb.IT\endcsname{0.021}
\expandafter\def\csname nv@lb.crb.IT.hi\endcsname{0.028}
\expandafter\def\csname nv@lb.crb.IT.lo\endcsname{0.014}
\expandafter\def\csname nv@lb.crb.LOC\endcsname{0.019}
\expandafter\def\csname nv@lb.crb.LOC.hi\endcsname{0.027}
\expandafter\def\csname nv@lb.crb.LOC.lo\endcsname{0.011}
\expandafter\def\csname nv@lb.crb.V1\endcsname{0.054}
\expandafter\def\csname nv@lb.crb.V1.hi\endcsname{0.066}
\expandafter\def\csname nv@lb.crb.V1.lo\endcsname{0.041}
\expandafter\def\csname nv@lb.crb.V2\endcsname{0.026}
\expandafter\def\csname nv@lb.crb.V2.hi\endcsname{0.034}
\expandafter\def\csname nv@lb.crb.V2.lo\endcsname{0.018}
\expandafter\def\csname nv@lbchg.IT\endcsname{39}
\expandafter\def\csname nv@lbchg.LOC\endcsname{46}
\expandafter\def\csname nv@lbchg.V1\endcsname{10}
\expandafter\def\csname nv@lbchg.V2\endcsname{28}
\expandafter\def\csname nv@lbnull.cr.IT.mean\endcsname{0.000}
\expandafter\def\csname nv@lbnull.cr.IT.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.cr.IT.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.cr.LOC.mean\endcsname{-0.000}
\expandafter\def\csname nv@lbnull.cr.LOC.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.cr.LOC.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.cr.V1.mean\endcsname{0.000}
\expandafter\def\csname nv@lbnull.cr.V1.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.cr.V1.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.cr.V2.mean\endcsname{-0.000}
\expandafter\def\csname nv@lbnull.cr.V2.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.cr.V2.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.crb.IT.mean\endcsname{0.000}
\expandafter\def\csname nv@lbnull.crb.IT.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.crb.IT.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.crb.LOC.mean\endcsname{-0.000}
\expandafter\def\csname nv@lbnull.crb.LOC.q\endcsname{0.003}
\expandafter\def\csname nv@lbnull.crb.LOC.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.crb.V1.mean\endcsname{0.000}
\expandafter\def\csname nv@lbnull.crb.V1.q\endcsname{0.005}
\expandafter\def\csname nv@lbnull.crb.V1.sd\endcsname{0.002}
\expandafter\def\csname nv@lbnull.crb.V2.mean\endcsname{-0.000}
\expandafter\def\csname nv@lbnull.crb.V2.q\endcsname{0.004}
\expandafter\def\csname nv@lbnull.crb.V2.sd\endcsname{0.002}
\expandafter\def\csname nv@lum.s1.V1.all\endcsname{0.052}
\expandafter\def\csname nv@lum.s1.V1.chg\endcsname{-1}
\expandafter\def\csname nv@lum.s1.V1.cr\endcsname{0.054}
\expandafter\def\csname nv@lum.s1.V1.crb\endcsname{0.054}
\expandafter\def\csname nv@lum.s1.V2.all\endcsname{0.033}
\expandafter\def\csname nv@lum.s1.V2.chg\endcsname{-2}
\expandafter\def\csname nv@lum.s1.V2.cr\endcsname{0.034}
\expandafter\def\csname nv@lum.s1.V2.crb\endcsname{0.033}
\expandafter\def\csname nv@lum.s2.V1.all\endcsname{0.094}
\expandafter\def\csname nv@lum.s2.V1.chg\endcsname{-10}
\expandafter\def\csname nv@lum.s2.V1.cr\endcsname{0.096}
\expandafter\def\csname nv@lum.s2.V1.crb\endcsname{0.086}
\expandafter\def\csname nv@lum.s2.V2.all\endcsname{0.061}
\expandafter\def\csname nv@lum.s2.V2.chg\endcsname{-16}
\expandafter\def\csname nv@lum.s2.V2.cr\endcsname{0.061}
\expandafter\def\csname nv@lum.s2.V2.crb\endcsname{0.051}
\expandafter\def\csname nv@lum.s3.V1.all\endcsname{0.011}
\expandafter\def\csname nv@lum.s3.V1.chg\endcsname{-2}
\expandafter\def\csname nv@lum.s3.V1.cr\endcsname{0.011}
\expandafter\def\csname nv@lum.s3.V1.crb\endcsname{0.011}
\expandafter\def\csname nv@lum.s3.V2.all\endcsname{0.002}
\expandafter\def\csname nv@lum.s3.V2.chg\endcsname{-12}
\expandafter\def\csname nv@lum.s3.V2.cr\endcsname{0.002}
\expandafter\def\csname nv@lum.s3.V2.crb\endcsname{0.002}
\expandafter\def\csname nv@lumv1.mr.all\endcsname{0.074}
\expandafter\def\csname nv@lumv1.mr.cr\endcsname{0.076}
\expandafter\def\csname nv@lumv1.ps.all\endcsname{0.052}
\expandafter\def\csname nv@lumv1.ps.cr\endcsname{0.054}
\expandafter\def\csname nv@ml.all.bn.bp.IT\endcsname{-0.026}
\expandafter\def\csname nv@ml.all.bn.bp.IT.hi\endcsname{-0.018}
\expandafter\def\csname nv@ml.all.bn.bp.IT.lo\endcsname{-0.034}
\expandafter\def\csname nv@ml.all.bn.bp.LOC\endcsname{-0.026}
\expandafter\def\csname nv@ml.all.bn.bp.LOC.hi\endcsname{-0.017}
\expandafter\def\csname nv@ml.all.bn.bp.LOC.lo\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.bn.bp.V1\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.bn.bp.V1.hi\endcsname{-0.023}
\expandafter\def\csname nv@ml.all.bn.bp.V1.lo\endcsname{-0.050}
\expandafter\def\csname nv@ml.all.bn.bp.V2\endcsname{-0.021}
\expandafter\def\csname nv@ml.all.bn.bp.V2.hi\endcsname{-0.011}
\expandafter\def\csname nv@ml.all.bn.bp.V2.lo\endcsname{-0.032}
\expandafter\def\csname nv@ml.all.bn.fa.IT\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.bn.fa.IT.hi\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.bn.fa.IT.lo\endcsname{-0.037}
\expandafter\def\csname nv@ml.all.bn.fa.LOC\endcsname{-0.031}
\expandafter\def\csname nv@ml.all.bn.fa.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.bn.fa.LOC.lo\endcsname{-0.040}
\expandafter\def\csname nv@ml.all.bn.fa.V1\endcsname{-0.050}
\expandafter\def\csname nv@ml.all.bn.fa.V1.hi\endcsname{-0.035}
\expandafter\def\csname nv@ml.all.bn.fa.V1.lo\endcsname{-0.065}
\expandafter\def\csname nv@ml.all.bn.fa.V2\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.bn.fa.V2.hi\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.bn.fa.V2.lo\endcsname{-0.041}
\expandafter\def\csname nv@ml.all.bn.pc.IT\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.bn.pc.IT.hi\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.bn.pc.IT.lo\endcsname{-0.037}
\expandafter\def\csname nv@ml.all.bn.pc.LOC\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.bn.pc.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.bn.pc.LOC.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.bn.pc.V1\endcsname{-0.046}
\expandafter\def\csname nv@ml.all.bn.pc.V1.hi\endcsname{-0.032}
\expandafter\def\csname nv@ml.all.bn.pc.V1.lo\endcsname{-0.062}
\expandafter\def\csname nv@ml.all.bn.pc.V2\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.bn.pc.V2.hi\endcsname{-0.017}
\expandafter\def\csname nv@ml.all.bn.pc.V2.lo\endcsname{-0.038}
\expandafter\def\csname nv@ml.all.bn.rnd.IT\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.bn.rnd.IT.hi\endcsname{-0.021}
\expandafter\def\csname nv@ml.all.bn.rnd.IT.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.bn.rnd.LOC\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.bn.rnd.LOC.hi\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.bn.rnd.LOC.lo\endcsname{-0.045}
\expandafter\def\csname nv@ml.all.bn.rnd.V1\endcsname{-0.004}
\expandafter\def\csname nv@ml.all.bn.rnd.V1.hi\endcsname{0.010}
\expandafter\def\csname nv@ml.all.bn.rnd.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.bn.rnd.V2\endcsname{-0.004}
\expandafter\def\csname nv@ml.all.bn.rnd.V2.hi\endcsname{0.007}
\expandafter\def\csname nv@ml.all.bn.rnd.V2.lo\endcsname{-0.016}
\expandafter\def\csname nv@ml.all.bn.stdp.IT\endcsname{-0.027}
\expandafter\def\csname nv@ml.all.bn.stdp.IT.hi\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.bn.stdp.IT.lo\endcsname{-0.035}
\expandafter\def\csname nv@ml.all.bn.stdp.LOC\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.bn.stdp.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.bn.stdp.LOC.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.bn.stdp.V1\endcsname{-0.032}
\expandafter\def\csname nv@ml.all.bn.stdp.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.bn.stdp.V1.lo\endcsname{-0.046}
\expandafter\def\csname nv@ml.all.bn.stdp.V2\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.bn.stdp.V2.hi\endcsname{-0.008}
\expandafter\def\csname nv@ml.all.bn.stdp.V2.lo\endcsname{-0.029}
\expandafter\def\csname nv@ml.all.ref.bp.IT\endcsname{-0.026}
\expandafter\def\csname nv@ml.all.ref.bp.IT.hi\endcsname{-0.018}
\expandafter\def\csname nv@ml.all.ref.bp.IT.lo\endcsname{-0.034}
\expandafter\def\csname nv@ml.all.ref.bp.LOC\endcsname{-0.027}
\expandafter\def\csname nv@ml.all.ref.bp.LOC.hi\endcsname{-0.017}
\expandafter\def\csname nv@ml.all.ref.bp.LOC.lo\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.ref.bp.V1\endcsname{-0.035}
\expandafter\def\csname nv@ml.all.ref.bp.V1.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.ref.bp.V1.lo\endcsname{-0.049}
\expandafter\def\csname nv@ml.all.ref.bp.V2\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.ref.bp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@ml.all.ref.bp.V2.lo\endcsname{-0.031}
\expandafter\def\csname nv@ml.all.ref.fa.IT\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.ref.fa.IT.hi\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.ref.fa.IT.lo\endcsname{-0.037}
\expandafter\def\csname nv@ml.all.ref.fa.LOC\endcsname{-0.031}
\expandafter\def\csname nv@ml.all.ref.fa.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.ref.fa.LOC.lo\endcsname{-0.040}
\expandafter\def\csname nv@ml.all.ref.fa.V1\endcsname{-0.050}
\expandafter\def\csname nv@ml.all.ref.fa.V1.hi\endcsname{-0.035}
\expandafter\def\csname nv@ml.all.ref.fa.V1.lo\endcsname{-0.065}
\expandafter\def\csname nv@ml.all.ref.fa.V2\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.ref.fa.V2.hi\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.ref.fa.V2.lo\endcsname{-0.041}
\expandafter\def\csname nv@ml.all.ref.pc.IT\endcsname{-0.026}
\expandafter\def\csname nv@ml.all.ref.pc.IT.hi\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.ref.pc.IT.lo\endcsname{-0.035}
\expandafter\def\csname nv@ml.all.ref.pc.LOC\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.ref.pc.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.ref.pc.LOC.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.ref.pc.V1\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.ref.pc.V1.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.all.ref.pc.V1.lo\endcsname{-0.031}
\expandafter\def\csname nv@ml.all.ref.pc.V2\endcsname{-0.014}
\expandafter\def\csname nv@ml.all.ref.pc.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@ml.all.ref.pc.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.all.ref.rnd.IT\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.ref.rnd.IT.hi\endcsname{-0.021}
\expandafter\def\csname nv@ml.all.ref.rnd.IT.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.ref.rnd.LOC\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.ref.rnd.LOC.hi\endcsname{-0.028}
\expandafter\def\csname nv@ml.all.ref.rnd.LOC.lo\endcsname{-0.045}
\expandafter\def\csname nv@ml.all.ref.rnd.V1\endcsname{-0.004}
\expandafter\def\csname nv@ml.all.ref.rnd.V1.hi\endcsname{0.010}
\expandafter\def\csname nv@ml.all.ref.rnd.V1.lo\endcsname{-0.019}
\expandafter\def\csname nv@ml.all.ref.rnd.V2\endcsname{-0.004}
\expandafter\def\csname nv@ml.all.ref.rnd.V2.hi\endcsname{0.007}
\expandafter\def\csname nv@ml.all.ref.rnd.V2.lo\endcsname{-0.016}
\expandafter\def\csname nv@ml.all.ref.stdp.IT\endcsname{-0.027}
\expandafter\def\csname nv@ml.all.ref.stdp.IT.hi\endcsname{-0.020}
\expandafter\def\csname nv@ml.all.ref.stdp.IT.lo\endcsname{-0.036}
\expandafter\def\csname nv@ml.all.ref.stdp.LOC\endcsname{-0.030}
\expandafter\def\csname nv@ml.all.ref.stdp.LOC.hi\endcsname{-0.022}
\expandafter\def\csname nv@ml.all.ref.stdp.LOC.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.all.ref.stdp.V1\endcsname{-0.013}
\expandafter\def\csname nv@ml.all.ref.stdp.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@ml.all.ref.stdp.V1.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.all.ref.stdp.V2\endcsname{-0.009}
\expandafter\def\csname nv@ml.all.ref.stdp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@ml.all.ref.stdp.V2.lo\endcsname{-0.019}
\expandafter\def\csname nv@ml.cr.bn.bp.IT\endcsname{-0.012}
\expandafter\def\csname nv@ml.cr.bn.bp.IT.hi\endcsname{-0.003}
\expandafter\def\csname nv@ml.cr.bn.bp.IT.lo\endcsname{-0.020}
\expandafter\def\csname nv@ml.cr.bn.bp.LOC\endcsname{-0.010}
\expandafter\def\csname nv@ml.cr.bn.bp.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@ml.cr.bn.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.bn.bp.V1\endcsname{-0.029}
\expandafter\def\csname nv@ml.cr.bn.bp.V1.hi\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.bn.bp.V1.lo\endcsname{-0.043}
\expandafter\def\csname nv@ml.cr.bn.bp.V2\endcsname{-0.011}
\expandafter\def\csname nv@ml.cr.bn.bp.V2.hi\endcsname{-0.000}
\expandafter\def\csname nv@ml.cr.bn.bp.V2.hi.4\endcsname{-0.0000}
\expandafter\def\csname nv@ml.cr.bn.bp.V2.lo\endcsname{-0.023}
\expandafter\def\csname nv@ml.cr.bn.fa.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.cr.bn.fa.IT.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.bn.fa.IT.lo\endcsname{-0.023}
\expandafter\def\csname nv@ml.cr.bn.fa.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.cr.bn.fa.LOC.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.cr.bn.fa.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.cr.bn.fa.V1\endcsname{-0.043}
\expandafter\def\csname nv@ml.cr.bn.fa.V1.hi\endcsname{-0.028}
\expandafter\def\csname nv@ml.cr.bn.fa.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@ml.cr.bn.fa.V2\endcsname{-0.020}
\expandafter\def\csname nv@ml.cr.bn.fa.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@ml.cr.bn.fa.V2.lo\endcsname{-0.032}
\expandafter\def\csname nv@ml.cr.bn.pc.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.cr.bn.pc.IT.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.bn.pc.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.cr.bn.pc.LOC\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.bn.pc.LOC.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.bn.pc.LOC.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.cr.bn.pc.V1\endcsname{-0.040}
\expandafter\def\csname nv@ml.cr.bn.pc.V1.hi\endcsname{-0.024}
\expandafter\def\csname nv@ml.cr.bn.pc.V1.lo\endcsname{-0.055}
\expandafter\def\csname nv@ml.cr.bn.pc.V2\endcsname{-0.018}
\expandafter\def\csname nv@ml.cr.bn.pc.V2.hi\endcsname{-0.007}
\expandafter\def\csname nv@ml.cr.bn.pc.V2.lo\endcsname{-0.030}
\expandafter\def\csname nv@ml.cr.bn.rnd.IT\endcsname{-0.017}
\expandafter\def\csname nv@ml.cr.bn.rnd.IT.hi\endcsname{-0.008}
\expandafter\def\csname nv@ml.cr.bn.rnd.IT.lo\endcsname{-0.027}
\expandafter\def\csname nv@ml.cr.bn.rnd.LOC\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.bn.rnd.LOC.hi\endcsname{-0.012}
\expandafter\def\csname nv@ml.cr.bn.rnd.LOC.lo\endcsname{-0.032}
\expandafter\def\csname nv@ml.cr.bn.rnd.V1\endcsname{+0.002}
\expandafter\def\csname nv@ml.cr.bn.rnd.V1.hi\endcsname{0.017}
\expandafter\def\csname nv@ml.cr.bn.rnd.V1.lo\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.bn.rnd.V2\endcsname{+0.005}
\expandafter\def\csname nv@ml.cr.bn.rnd.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@ml.cr.bn.rnd.V2.lo\endcsname{-0.007}
\expandafter\def\csname nv@ml.cr.bn.stdp.IT\endcsname{-0.012}
\expandafter\def\csname nv@ml.cr.bn.stdp.IT.hi\endcsname{-0.004}
\expandafter\def\csname nv@ml.cr.bn.stdp.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.bn.stdp.LOC\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.bn.stdp.LOC.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.bn.stdp.LOC.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.cr.bn.stdp.V1\endcsname{-0.025}
\expandafter\def\csname nv@ml.cr.bn.stdp.V1.hi\endcsname{-0.010}
\expandafter\def\csname nv@ml.cr.bn.stdp.V1.lo\endcsname{-0.039}
\expandafter\def\csname nv@ml.cr.bn.stdp.V2\endcsname{-0.009}
\expandafter\def\csname nv@ml.cr.bn.stdp.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@ml.cr.bn.stdp.V2.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.ref.bp.IT\endcsname{-0.011}
\expandafter\def\csname nv@ml.cr.ref.bp.IT.hi\endcsname{-0.002}
\expandafter\def\csname nv@ml.cr.ref.bp.IT.lo\endcsname{-0.020}
\expandafter\def\csname nv@ml.cr.ref.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@ml.cr.ref.bp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@ml.cr.ref.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.ref.bp.V1\endcsname{-0.027}
\expandafter\def\csname nv@ml.cr.ref.bp.V1.hi\endcsname{-0.012}
\expandafter\def\csname nv@ml.cr.ref.bp.V1.lo\endcsname{-0.042}
\expandafter\def\csname nv@ml.cr.ref.bp.V2\endcsname{-0.010}
\expandafter\def\csname nv@ml.cr.ref.bp.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@ml.cr.ref.bp.V2.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.cr.ref.fa.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.cr.ref.fa.IT.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.ref.fa.IT.lo\endcsname{-0.023}
\expandafter\def\csname nv@ml.cr.ref.fa.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.cr.ref.fa.LOC.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.cr.ref.fa.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.cr.ref.fa.V1\endcsname{-0.043}
\expandafter\def\csname nv@ml.cr.ref.fa.V1.hi\endcsname{-0.027}
\expandafter\def\csname nv@ml.cr.ref.fa.V1.lo\endcsname{-0.059}
\expandafter\def\csname nv@ml.cr.ref.fa.V2\endcsname{-0.020}
\expandafter\def\csname nv@ml.cr.ref.fa.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@ml.cr.ref.fa.V2.lo\endcsname{-0.032}
\expandafter\def\csname nv@ml.cr.ref.pc.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.cr.ref.pc.IT.hi\endcsname{-0.004}
\expandafter\def\csname nv@ml.cr.ref.pc.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.cr.ref.pc.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.cr.ref.pc.LOC.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.cr.ref.pc.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.cr.ref.pc.V1\endcsname{-0.013}
\expandafter\def\csname nv@ml.cr.ref.pc.V1.hi\endcsname{0.002}
\expandafter\def\csname nv@ml.cr.ref.pc.V1.lo\endcsname{-0.026}
\expandafter\def\csname nv@ml.cr.ref.pc.V2\endcsname{-0.005}
\expandafter\def\csname nv@ml.cr.ref.pc.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@ml.cr.ref.pc.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@ml.cr.ref.rnd.IT\endcsname{-0.017}
\expandafter\def\csname nv@ml.cr.ref.rnd.IT.hi\endcsname{-0.008}
\expandafter\def\csname nv@ml.cr.ref.rnd.IT.lo\endcsname{-0.027}
\expandafter\def\csname nv@ml.cr.ref.rnd.LOC\endcsname{-0.021}
\expandafter\def\csname nv@ml.cr.ref.rnd.LOC.hi\endcsname{-0.012}
\expandafter\def\csname nv@ml.cr.ref.rnd.LOC.lo\endcsname{-0.032}
\expandafter\def\csname nv@ml.cr.ref.rnd.V1\endcsname{+0.002}
\expandafter\def\csname nv@ml.cr.ref.rnd.V1.hi\endcsname{0.017}
\expandafter\def\csname nv@ml.cr.ref.rnd.V1.lo\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.ref.rnd.V2\endcsname{+0.005}
\expandafter\def\csname nv@ml.cr.ref.rnd.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@ml.cr.ref.rnd.V2.lo\endcsname{-0.007}
\expandafter\def\csname nv@ml.cr.ref.stdp.IT\endcsname{-0.014}
\expandafter\def\csname nv@ml.cr.ref.stdp.IT.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.cr.ref.stdp.IT.lo\endcsname{-0.023}
\expandafter\def\csname nv@ml.cr.ref.stdp.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.cr.ref.stdp.LOC.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.cr.ref.stdp.LOC.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.cr.ref.stdp.V1\endcsname{-0.007}
\expandafter\def\csname nv@ml.cr.ref.stdp.V1.hi\endcsname{0.007}
\expandafter\def\csname nv@ml.cr.ref.stdp.V1.lo\endcsname{-0.020}
\expandafter\def\csname nv@ml.cr.ref.stdp.V2\endcsname{+0.000}
\expandafter\def\csname nv@ml.cr.ref.stdp.V2.hi\endcsname{0.010}
\expandafter\def\csname nv@ml.cr.ref.stdp.V2.lo\endcsname{-0.010}
\expandafter\def\csname nv@ml.crb.bn.bp.IT\endcsname{-0.012}
\expandafter\def\csname nv@ml.crb.bn.bp.IT.hi\endcsname{-0.004}
\expandafter\def\csname nv@ml.crb.bn.bp.IT.lo\endcsname{-0.020}
\expandafter\def\csname nv@ml.crb.bn.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@ml.crb.bn.bp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@ml.crb.bn.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.crb.bn.bp.V1\endcsname{-0.033}
\expandafter\def\csname nv@ml.crb.bn.bp.V1.hi\endcsname{-0.019}
\expandafter\def\csname nv@ml.crb.bn.bp.V1.lo\endcsname{-0.046}
\expandafter\def\csname nv@ml.crb.bn.bp.V2\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.bn.bp.V2.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.crb.bn.bp.V2.lo\endcsname{-0.026}
\expandafter\def\csname nv@ml.crb.bn.fa.IT\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.bn.fa.IT.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.crb.bn.fa.IT.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.bn.fa.LOC\endcsname{-0.016}
\expandafter\def\csname nv@ml.crb.bn.fa.LOC.hi\endcsname{-0.008}
\expandafter\def\csname nv@ml.crb.bn.fa.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@ml.crb.bn.fa.V1\endcsname{-0.048}
\expandafter\def\csname nv@ml.crb.bn.fa.V1.hi\endcsname{-0.032}
\expandafter\def\csname nv@ml.crb.bn.fa.V1.lo\endcsname{-0.062}
\expandafter\def\csname nv@ml.crb.bn.fa.V2\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.bn.fa.V2.hi\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.bn.fa.V2.lo\endcsname{-0.035}
\expandafter\def\csname nv@ml.crb.bn.pc.IT\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.bn.pc.IT.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.crb.bn.pc.IT.lo\endcsname{-0.023}
\expandafter\def\csname nv@ml.crb.bn.pc.LOC\endcsname{-0.016}
\expandafter\def\csname nv@ml.crb.bn.pc.LOC.hi\endcsname{-0.007}
\expandafter\def\csname nv@ml.crb.bn.pc.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@ml.crb.bn.pc.V1\endcsname{-0.044}
\expandafter\def\csname nv@ml.crb.bn.pc.V1.hi\endcsname{-0.029}
\expandafter\def\csname nv@ml.crb.bn.pc.V1.lo\endcsname{-0.058}
\expandafter\def\csname nv@ml.crb.bn.pc.V2\endcsname{-0.022}
\expandafter\def\csname nv@ml.crb.bn.pc.V2.hi\endcsname{-0.011}
\expandafter\def\csname nv@ml.crb.bn.pc.V2.lo\endcsname{-0.033}
\expandafter\def\csname nv@ml.crb.bn.rnd.IT\endcsname{-0.018}
\expandafter\def\csname nv@ml.crb.bn.rnd.IT.hi\endcsname{-0.009}
\expandafter\def\csname nv@ml.crb.bn.rnd.IT.lo\endcsname{-0.028}
\expandafter\def\csname nv@ml.crb.bn.rnd.LOC\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.bn.rnd.LOC.hi\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.bn.rnd.LOC.lo\endcsname{-0.034}
\expandafter\def\csname nv@ml.crb.bn.rnd.V1\endcsname{-0.001}
\expandafter\def\csname nv@ml.crb.bn.rnd.V1.hi\endcsname{0.015}
\expandafter\def\csname nv@ml.crb.bn.rnd.V1.lo\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.bn.rnd.V2\endcsname{+0.002}
\expandafter\def\csname nv@ml.crb.bn.rnd.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@ml.crb.bn.rnd.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@ml.crb.bn.stdp.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.crb.bn.stdp.IT.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.crb.bn.stdp.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.crb.bn.stdp.LOC\endcsname{-0.016}
\expandafter\def\csname nv@ml.crb.bn.stdp.LOC.hi\endcsname{-0.007}
\expandafter\def\csname nv@ml.crb.bn.stdp.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.crb.bn.stdp.V1\endcsname{-0.030}
\expandafter\def\csname nv@ml.crb.bn.stdp.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.bn.stdp.V1.lo\endcsname{-0.043}
\expandafter\def\csname nv@ml.crb.bn.stdp.V2\endcsname{-0.013}
\expandafter\def\csname nv@ml.crb.bn.stdp.V2.hi\endcsname{-0.003}
\expandafter\def\csname nv@ml.crb.bn.stdp.V2.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.ref.bp.IT\endcsname{-0.012}
\expandafter\def\csname nv@ml.crb.ref.bp.IT.hi\endcsname{-0.003}
\expandafter\def\csname nv@ml.crb.ref.bp.IT.lo\endcsname{-0.020}
\expandafter\def\csname nv@ml.crb.ref.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@ml.crb.ref.bp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@ml.crb.ref.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@ml.crb.ref.bp.V1\endcsname{-0.032}
\expandafter\def\csname nv@ml.crb.ref.bp.V1.hi\endcsname{-0.018}
\expandafter\def\csname nv@ml.crb.ref.bp.V1.lo\endcsname{-0.044}
\expandafter\def\csname nv@ml.crb.ref.bp.V2\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.ref.bp.V2.hi\endcsname{-0.004}
\expandafter\def\csname nv@ml.crb.ref.bp.V2.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.crb.ref.fa.IT\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.ref.fa.IT.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.crb.ref.fa.IT.lo\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.ref.fa.LOC\endcsname{-0.016}
\expandafter\def\csname nv@ml.crb.ref.fa.LOC.hi\endcsname{-0.008}
\expandafter\def\csname nv@ml.crb.ref.fa.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@ml.crb.ref.fa.V1\endcsname{-0.048}
\expandafter\def\csname nv@ml.crb.ref.fa.V1.hi\endcsname{-0.032}
\expandafter\def\csname nv@ml.crb.ref.fa.V1.lo\endcsname{-0.062}
\expandafter\def\csname nv@ml.crb.ref.fa.V2\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.ref.fa.V2.hi\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.ref.fa.V2.lo\endcsname{-0.035}
\expandafter\def\csname nv@ml.crb.ref.pc.IT\endcsname{-0.013}
\expandafter\def\csname nv@ml.crb.ref.pc.IT.hi\endcsname{-0.005}
\expandafter\def\csname nv@ml.crb.ref.pc.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.crb.ref.pc.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.ref.pc.LOC.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.crb.ref.pc.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.crb.ref.pc.V1\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.ref.pc.V1.hi\endcsname{0.000}
\expandafter\def\csname nv@ml.crb.ref.pc.V1.lo\endcsname{-0.028}
\expandafter\def\csname nv@ml.crb.ref.pc.V2\endcsname{-0.007}
\expandafter\def\csname nv@ml.crb.ref.pc.V2.hi\endcsname{0.004}
\expandafter\def\csname nv@ml.crb.ref.pc.V2.lo\endcsname{-0.017}
\expandafter\def\csname nv@ml.crb.ref.rnd.IT\endcsname{-0.018}
\expandafter\def\csname nv@ml.crb.ref.rnd.IT.hi\endcsname{-0.009}
\expandafter\def\csname nv@ml.crb.ref.rnd.IT.lo\endcsname{-0.028}
\expandafter\def\csname nv@ml.crb.ref.rnd.LOC\endcsname{-0.024}
\expandafter\def\csname nv@ml.crb.ref.rnd.LOC.hi\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.ref.rnd.LOC.lo\endcsname{-0.034}
\expandafter\def\csname nv@ml.crb.ref.rnd.V1\endcsname{-0.001}
\expandafter\def\csname nv@ml.crb.ref.rnd.V1.hi\endcsname{0.015}
\expandafter\def\csname nv@ml.crb.ref.rnd.V1.lo\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.ref.rnd.V2\endcsname{+0.002}
\expandafter\def\csname nv@ml.crb.ref.rnd.V2.hi\endcsname{0.014}
\expandafter\def\csname nv@ml.crb.ref.rnd.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@ml.crb.ref.stdp.IT\endcsname{-0.014}
\expandafter\def\csname nv@ml.crb.ref.stdp.IT.hi\endcsname{-0.006}
\expandafter\def\csname nv@ml.crb.ref.stdp.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.crb.ref.stdp.LOC\endcsname{-0.015}
\expandafter\def\csname nv@ml.crb.ref.stdp.LOC.hi\endcsname{-0.007}
\expandafter\def\csname nv@ml.crb.ref.stdp.LOC.lo\endcsname{-0.025}
\expandafter\def\csname nv@ml.crb.ref.stdp.V1\endcsname{-0.010}
\expandafter\def\csname nv@ml.crb.ref.stdp.V1.hi\endcsname{0.004}
\expandafter\def\csname nv@ml.crb.ref.stdp.V1.lo\endcsname{-0.022}
\expandafter\def\csname nv@ml.crb.ref.stdp.V2\endcsname{-0.003}
\expandafter\def\csname nv@ml.crb.ref.stdp.V2.hi\endcsname{0.008}
\expandafter\def\csname nv@ml.crb.ref.stdp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@nboot\endcsname{1000}
\expandafter\def\csname nv@nperm\endcsname{1000}
\expandafter\def\csname nv@nprimary\endcsname{7}
\expandafter\def\csname nv@nprimary.old\endcsname{11}
\expandafter\def\csname nv@pairs.cr\endcsname{210{,}205}
\expandafter\def\csname nv@pairs.cr.pct\endcsname{81.2}
\expandafter\def\csname nv@pairs.excl.pct\endcsname{18.8}
\expandafter\def\csname nv@pairs.total\endcsname{258{,}840}
\expandafter\def\csname nv@part.bp.d\endcsname{-0.008}
\expandafter\def\csname nv@part.bp.par\endcsname{0.026}
\expandafter\def\csname nv@part.bp.std\endcsname{0.034}
\expandafter\def\csname nv@part.d.max\endcsname{-0.004}
\expandafter\def\csname nv@part.d.min\endcsname{-0.008}
\expandafter\def\csname nv@part.fa.V2.p\endcsname{0.755}
\expandafter\def\csname nv@part.fa.V2.par\endcsname{0.001}
\expandafter\def\csname nv@part.fa.d\endcsname{-0.007}
\expandafter\def\csname nv@part.fa.par\endcsname{0.005}
\expandafter\def\csname nv@part.fa.std\endcsname{0.012}
\expandafter\def\csname nv@part.rnd.d\endcsname{-0.004}
\expandafter\def\csname nv@part.rnd.par\endcsname{0.074}
\expandafter\def\csname nv@part.rnd.std\endcsname{0.078}
\expandafter\def\csname nv@permseed\endcsname{20261005}
\expandafter\def\csname nv@pr.d.V1.max\endcsname{-0.002}
\expandafter\def\csname nv@pr.d.V1.min\endcsname{-0.005}
\expandafter\def\csname nv@pr.delta.bp.IT\endcsname{-0.0003}
\expandafter\def\csname nv@pr.delta.bp.IT.hi\endcsname{0.0004}
\expandafter\def\csname nv@pr.delta.bp.IT.lo\endcsname{-0.0010}
\expandafter\def\csname nv@pr.delta.bp.LOC\endcsname{-0.0002}
\expandafter\def\csname nv@pr.delta.bp.LOC.hi\endcsname{0.0005}
\expandafter\def\csname nv@pr.delta.bp.LOC.lo\endcsname{-0.0009}
\expandafter\def\csname nv@pr.delta.bp.V1\endcsname{-0.0052}
\expandafter\def\csname nv@pr.delta.bp.V1.hi\endcsname{-0.0027}
\expandafter\def\csname nv@pr.delta.bp.V1.lo\endcsname{-0.0080}
\expandafter\def\csname nv@pr.delta.bp.V2\endcsname{-0.0022}
\expandafter\def\csname nv@pr.delta.bp.V2.hi\endcsname{-0.0002}
\expandafter\def\csname nv@pr.delta.bp.V2.lo\endcsname{-0.0045}
\expandafter\def\csname nv@pr.delta.fa.IT\endcsname{-0.0005}
\expandafter\def\csname nv@pr.delta.fa.IT.hi\endcsname{0.0011}
\expandafter\def\csname nv@pr.delta.fa.IT.lo\endcsname{-0.0023}
\expandafter\def\csname nv@pr.delta.fa.LOC\endcsname{-0.0004}
\expandafter\def\csname nv@pr.delta.fa.LOC.hi\endcsname{0.0007}
\expandafter\def\csname nv@pr.delta.fa.LOC.lo\endcsname{-0.0015}
\expandafter\def\csname nv@pr.delta.fa.V1\endcsname{-0.0045}
\expandafter\def\csname nv@pr.delta.fa.V1.hi\endcsname{-0.0024}
\expandafter\def\csname nv@pr.delta.fa.V1.lo\endcsname{-0.0069}
\expandafter\def\csname nv@pr.delta.fa.V2\endcsname{-0.0020}
\expandafter\def\csname nv@pr.delta.fa.V2.hi\endcsname{-0.0003}
\expandafter\def\csname nv@pr.delta.fa.V2.lo\endcsname{-0.0040}
\expandafter\def\csname nv@pr.delta.pc.IT\endcsname{-0.0005}
\expandafter\def\csname nv@pr.delta.pc.IT.hi\endcsname{0.0010}
\expandafter\def\csname nv@pr.delta.pc.IT.lo\endcsname{-0.0022}
\expandafter\def\csname nv@pr.delta.pc.LOC\endcsname{-0.0004}
\expandafter\def\csname nv@pr.delta.pc.LOC.hi\endcsname{0.0008}
\expandafter\def\csname nv@pr.delta.pc.LOC.lo\endcsname{-0.0016}
\expandafter\def\csname nv@pr.delta.pc.V1\endcsname{-0.0046}
\expandafter\def\csname nv@pr.delta.pc.V1.hi\endcsname{-0.0026}
\expandafter\def\csname nv@pr.delta.pc.V1.lo\endcsname{-0.0071}
\expandafter\def\csname nv@pr.delta.pc.V2\endcsname{-0.0021}
\expandafter\def\csname nv@pr.delta.pc.V2.hi\endcsname{-0.0005}
\expandafter\def\csname nv@pr.delta.pc.V2.lo\endcsname{-0.0041}
\expandafter\def\csname nv@pr.delta.rnd.IT\endcsname{-0.0008}
\expandafter\def\csname nv@pr.delta.rnd.IT.hi\endcsname{0.0011}
\expandafter\def\csname nv@pr.delta.rnd.IT.lo\endcsname{-0.0029}
\expandafter\def\csname nv@pr.delta.rnd.LOC\endcsname{-0.0002}
\expandafter\def\csname nv@pr.delta.rnd.LOC.hi\endcsname{0.0002}
\expandafter\def\csname nv@pr.delta.rnd.LOC.lo\endcsname{-0.0007}
\expandafter\def\csname nv@pr.delta.rnd.V1\endcsname{-0.0025}
\expandafter\def\csname nv@pr.delta.rnd.V1.hi\endcsname{-0.0011}
\expandafter\def\csname nv@pr.delta.rnd.V1.lo\endcsname{-0.0042}
\expandafter\def\csname nv@pr.delta.rnd.V2\endcsname{-0.0011}
\expandafter\def\csname nv@pr.delta.rnd.V2.hi\endcsname{-0.0000}
\expandafter\def\csname nv@pr.delta.rnd.V2.lo\endcsname{-0.0024}
\expandafter\def\csname nv@pr.delta.stdp.IT\endcsname{-0.0005}
\expandafter\def\csname nv@pr.delta.stdp.IT.hi\endcsname{0.0008}
\expandafter\def\csname nv@pr.delta.stdp.IT.lo\endcsname{-0.0018}
\expandafter\def\csname nv@pr.delta.stdp.LOC\endcsname{-0.0004}
\expandafter\def\csname nv@pr.delta.stdp.LOC.hi\endcsname{0.0009}
\expandafter\def\csname nv@pr.delta.stdp.LOC.lo\endcsname{-0.0017}
\expandafter\def\csname nv@pr.delta.stdp.V1\endcsname{-0.0045}
\expandafter\def\csname nv@pr.delta.stdp.V1.hi\endcsname{-0.0024}
\expandafter\def\csname nv@pr.delta.stdp.V1.lo\endcsname{-0.0069}
\expandafter\def\csname nv@pr.delta.stdp.V2\endcsname{-0.0020}
\expandafter\def\csname nv@pr.delta.stdp.V2.hi\endcsname{-0.0002}
\expandafter\def\csname nv@pr.delta.stdp.V2.lo\endcsname{-0.0041}
\expandafter\def\csname nv@pr.partial.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@pr.partial.bp.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@pr.partial.bp.IT.lo\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@pr.partial.bp.LOC.hi\endcsname{0.015}
\expandafter\def\csname nv@pr.partial.bp.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@pr.partial.bp.V1\endcsname{0.017}
\expandafter\def\csname nv@pr.partial.bp.V1.hi\endcsname{0.027}
\expandafter\def\csname nv@pr.partial.bp.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@pr.partial.bp.V2\endcsname{0.010}
\expandafter\def\csname nv@pr.partial.bp.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@pr.partial.bp.V2.lo\endcsname{0.003}
\expandafter\def\csname nv@pr.partial.fa.IT\endcsname{0.007}
\expandafter\def\csname nv@pr.partial.fa.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@pr.partial.fa.IT.lo\endcsname{0.001}
\expandafter\def\csname nv@pr.partial.fa.LOC\endcsname{0.003}
\expandafter\def\csname nv@pr.partial.fa.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@pr.partial.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@pr.partial.fa.V1\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.fa.V1.hi\endcsname{0.013}
\expandafter\def\csname nv@pr.partial.fa.V1.lo\endcsname{-0.004}
\expandafter\def\csname nv@pr.partial.fa.V2\endcsname{0.002}
\expandafter\def\csname nv@pr.partial.fa.V2.hi\endcsname{0.008}
\expandafter\def\csname nv@pr.partial.fa.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@pr.partial.pc.IT\endcsname{0.007}
\expandafter\def\csname nv@pr.partial.pc.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@pr.partial.pc.IT.lo\endcsname{0.001}
\expandafter\def\csname nv@pr.partial.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.pc.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@pr.partial.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@pr.partial.pc.V1\endcsname{0.007}
\expandafter\def\csname nv@pr.partial.pc.V1.hi\endcsname{0.017}
\expandafter\def\csname nv@pr.partial.pc.V1.lo\endcsname{-0.001}
\expandafter\def\csname nv@pr.partial.pc.V2\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.pc.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@pr.partial.pc.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@pr.partial.rnd.IT\endcsname{0.003}
\expandafter\def\csname nv@pr.partial.rnd.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@pr.partial.rnd.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@pr.partial.rnd.LOC\endcsname{-0.003}
\expandafter\def\csname nv@pr.partial.rnd.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.rnd.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@pr.partial.rnd.V1\endcsname{0.051}
\expandafter\def\csname nv@pr.partial.rnd.V1.hi\endcsname{0.066}
\expandafter\def\csname nv@pr.partial.rnd.V1.lo\endcsname{0.037}
\expandafter\def\csname nv@pr.partial.rnd.V2\endcsname{0.028}
\expandafter\def\csname nv@pr.partial.rnd.V2.hi\endcsname{0.038}
\expandafter\def\csname nv@pr.partial.rnd.V2.lo\endcsname{0.018}
\expandafter\def\csname nv@pr.partial.stdp.IT\endcsname{0.008}
\expandafter\def\csname nv@pr.partial.stdp.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@pr.partial.stdp.IT.lo\endcsname{0.003}
\expandafter\def\csname nv@pr.partial.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@pr.partial.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@pr.partial.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@pr.partial.stdp.V1\endcsname{0.022}
\expandafter\def\csname nv@pr.partial.stdp.V1.hi\endcsname{0.032}
\expandafter\def\csname nv@pr.partial.stdp.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@pr.partial.stdp.V2\endcsname{0.013}
\expandafter\def\csname nv@pr.partial.stdp.V2.hi\endcsname{0.020}
\expandafter\def\csname nv@pr.partial.stdp.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@pr.std.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@pr.std.bp.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@pr.std.bp.IT.lo\endcsname{0.004}
\expandafter\def\csname nv@pr.std.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@pr.std.bp.LOC.hi\endcsname{0.015}
\expandafter\def\csname nv@pr.std.bp.LOC.lo\endcsname{0.001}
\expandafter\def\csname nv@pr.std.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@pr.std.bp.V1.hi\endcsname{0.033}
\expandafter\def\csname nv@pr.std.bp.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@pr.std.bp.V2\endcsname{0.012}
\expandafter\def\csname nv@pr.std.bp.V2.hi\endcsname{0.020}
\expandafter\def\csname nv@pr.std.bp.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@pr.std.fa.IT\endcsname{0.008}
\expandafter\def\csname nv@pr.std.fa.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@pr.std.fa.IT.lo\endcsname{0.001}
\expandafter\def\csname nv@pr.std.fa.LOC\endcsname{0.004}
\expandafter\def\csname nv@pr.std.fa.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@pr.std.fa.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@pr.std.fa.V1\endcsname{0.009}
\expandafter\def\csname nv@pr.std.fa.V1.hi\endcsname{0.018}
\expandafter\def\csname nv@pr.std.fa.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@pr.std.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@pr.std.fa.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@pr.std.fa.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@pr.std.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@pr.std.pc.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@pr.std.pc.IT.lo\endcsname{0.002}
\expandafter\def\csname nv@pr.std.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@pr.std.pc.LOC.hi\endcsname{0.011}
\expandafter\def\csname nv@pr.std.pc.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@pr.std.pc.V1\endcsname{0.012}
\expandafter\def\csname nv@pr.std.pc.V1.hi\endcsname{0.022}
\expandafter\def\csname nv@pr.std.pc.V1.lo\endcsname{0.003}
\expandafter\def\csname nv@pr.std.pc.V2\endcsname{0.006}
\expandafter\def\csname nv@pr.std.pc.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@pr.std.pc.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@pr.std.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@pr.std.rnd.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@pr.std.rnd.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@pr.std.rnd.LOC\endcsname{-0.003}
\expandafter\def\csname nv@pr.std.rnd.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@pr.std.rnd.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@pr.std.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@pr.std.rnd.V1.hi\endcsname{0.069}
\expandafter\def\csname nv@pr.std.rnd.V1.lo\endcsname{0.039}
\expandafter\def\csname nv@pr.std.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@pr.std.rnd.V2.hi\endcsname{0.040}
\expandafter\def\csname nv@pr.std.rnd.V2.lo\endcsname{0.019}
\expandafter\def\csname nv@pr.std.stdp.IT\endcsname{0.009}
\expandafter\def\csname nv@pr.std.stdp.IT.hi\endcsname{0.014}
\expandafter\def\csname nv@pr.std.stdp.IT.lo\endcsname{0.003}
\expandafter\def\csname nv@pr.std.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@pr.std.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@pr.std.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@pr.std.stdp.V1\endcsname{0.027}
\expandafter\def\csname nv@pr.std.stdp.V1.hi\endcsname{0.037}
\expandafter\def\csname nv@pr.std.stdp.V1.lo\endcsname{0.017}
\expandafter\def\csname nv@pr.std.stdp.V2\endcsname{0.015}
\expandafter\def\csname nv@pr.std.stdp.V2.hi\endcsname{0.023}
\expandafter\def\csname nv@pr.std.stdp.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@prd.rnd.bp.IT\endcsname{-0.006}
\expandafter\def\csname nv@prd.rnd.bp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@prd.rnd.bp.IT.lo\endcsname{-0.015}
\expandafter\def\csname nv@prd.rnd.bp.LOC\endcsname{-0.011}
\expandafter\def\csname nv@prd.rnd.bp.LOC.hi\endcsname{-0.002}
\expandafter\def\csname nv@prd.rnd.bp.LOC.lo\endcsname{-0.021}
\expandafter\def\csname nv@prd.rnd.bp.V1\endcsname{+0.034}
\expandafter\def\csname nv@prd.rnd.bp.V1.hi\endcsname{0.046}
\expandafter\def\csname nv@prd.rnd.bp.V1.lo\endcsname{0.021}
\expandafter\def\csname nv@prd.rnd.bp.V2\endcsname{+0.018}
\expandafter\def\csname nv@prd.rnd.bp.V2.hi\endcsname{0.027}
\expandafter\def\csname nv@prd.rnd.bp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@pval.dev\endcsname{0.00005}
\expandafter\def\csname nv@range.mr.IT.max\endcsname{0.015}
\expandafter\def\csname nv@range.mr.IT.min\endcsname{0.006}
\expandafter\def\csname nv@range.mr.LOC.max\endcsname{0.013}
\expandafter\def\csname nv@range.mr.LOC.min\endcsname{-0.007}
\expandafter\def\csname nv@range.mr.V1.max\endcsname{0.077}
\expandafter\def\csname nv@range.mr.V1.min\endcsname{0.014}
\expandafter\def\csname nv@range.mr.V2.max\endcsname{0.043}
\expandafter\def\csname nv@range.mr.V2.min\endcsname{0.005}
\expandafter\def\csname nv@range.ps.IT.max\endcsname{0.009}
\expandafter\def\csname nv@range.ps.IT.min\endcsname{0.004}
\expandafter\def\csname nv@range.ps.LOC.max\endcsname{0.008}
\expandafter\def\csname nv@range.ps.LOC.min\endcsname{-0.003}
\expandafter\def\csname nv@range.ps.V1.max\endcsname{0.053}
\expandafter\def\csname nv@range.ps.V1.min\endcsname{0.009}
\expandafter\def\csname nv@range.ps.V2.max\endcsname{0.029}
\expandafter\def\csname nv@range.ps.V2.min\endcsname{0.004}
\expandafter\def\csname nv@repair.max\endcsname{0.0013}
\expandafter\def\csname nv@res.bp.32\endcsname{0.046}
\expandafter\def\csname nv@res.gap.224\endcsname{+0.0304}
\expandafter\def\csname nv@res.gap.224.3\endcsname{+0.030}
\expandafter\def\csname nv@res.gap.224.hi\endcsname{+0.0423}
\expandafter\def\csname nv@res.gap.224.hi.3\endcsname{0.042}
\expandafter\def\csname nv@res.gap.224.lo\endcsname{+0.0181}
\expandafter\def\csname nv@res.gap.224.lo.3\endcsname{0.018}
\expandafter\def\csname nv@res.gap.32\endcsname{-0.0007}
\expandafter\def\csname nv@res.gap.32.3\endcsname{-0.001}
\expandafter\def\csname nv@res.gap.32.hi\endcsname{+0.0090}
\expandafter\def\csname nv@res.gap.32.hi.3\endcsname{0.009}
\expandafter\def\csname nv@res.gap.32.lo\endcsname{-0.0109}
\expandafter\def\csname nv@res.gap.32.lo.3\endcsname{-0.011}
\expandafter\def\csname nv@res.rnd.32\endcsname{0.045}
\expandafter\def\csname nv@rho.mr.all.bn.bp.IT\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.all.bn.bp.IT.4\endcsname{0.0127}
\expandafter\def\csname nv@rho.mr.all.bn.bp.IT.hi\endcsname{.021}
\expandafter\def\csname nv@rho.mr.all.bn.bp.IT.lo\endcsname{.005}
\expandafter\def\csname nv@rho.mr.all.bn.bp.LOC\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.all.bn.bp.LOC.4\endcsname{0.0126}
\expandafter\def\csname nv@rho.mr.all.bn.bp.LOC.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.all.bn.bp.LOC.lo\endcsname{.002}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V1\endcsname{0.031}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V1.4\endcsname{0.0314}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V1.hi\endcsname{.047}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V1.lo\endcsname{.018}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V2\endcsname{0.017}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V2.4\endcsname{0.0169}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V2.hi\endcsname{.029}
\expandafter\def\csname nv@rho.mr.all.bn.bp.V2.lo\endcsname{.006}
\expandafter\def\csname nv@rho.mr.all.bn.fa.IT\endcsname{0.011}
\expandafter\def\csname nv@rho.mr.all.bn.fa.IT.4\endcsname{0.0115}
\expandafter\def\csname nv@rho.mr.all.bn.fa.IT.hi\endcsname{.021}
\expandafter\def\csname nv@rho.mr.all.bn.fa.IT.lo\endcsname{.002}
\expandafter\def\csname nv@rho.mr.all.bn.fa.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.bn.fa.LOC.4\endcsname{0.0056}
\expandafter\def\csname nv@rho.mr.all.bn.fa.LOC.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.all.bn.fa.LOC.lo\endcsname{-.005}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V1\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V1.4\endcsname{0.0115}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V1.hi\endcsname{.026}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V1.lo\endcsname{-.000}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V2.4\endcsname{0.0040}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V2.hi\endcsname{.015}
\expandafter\def\csname nv@rho.mr.all.bn.fa.V2.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.all.bn.pc.IT\endcsname{0.011}
\expandafter\def\csname nv@rho.mr.all.bn.pc.IT.4\endcsname{0.0109}
\expandafter\def\csname nv@rho.mr.all.bn.pc.IT.hi\endcsname{.020}
\expandafter\def\csname nv@rho.mr.all.bn.pc.IT.lo\endcsname{.002}
\expandafter\def\csname nv@rho.mr.all.bn.pc.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.bn.pc.LOC.4\endcsname{0.0062}
\expandafter\def\csname nv@rho.mr.all.bn.pc.LOC.hi\endcsname{.016}
\expandafter\def\csname nv@rho.mr.all.bn.pc.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V1\endcsname{0.016}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V1.4\endcsname{0.0163}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V1.hi\endcsname{.031}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V1.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V2\endcsname{0.007}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V2.4\endcsname{0.0075}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V2.hi\endcsname{.019}
\expandafter\def\csname nv@rho.mr.all.bn.pc.V2.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.IT.4\endcsname{0.0078}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.IT.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.IT.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.LOC\endcsname{-0.005}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.LOC.4\endcsname{-0.0051}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.LOC.hi\endcsname{.005}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.LOC.lo\endcsname{-.016}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V1\endcsname{0.075}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V1.4\endcsname{0.0755}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V1.hi\endcsname{.098}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V1.lo\endcsname{.055}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V2\endcsname{0.043}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V2.4\endcsname{0.0433}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V2.hi\endcsname{.060}
\expandafter\def\csname nv@rho.mr.all.bn.rnd.V2.lo\endcsname{.028}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.IT\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.IT.4\endcsname{0.0131}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.IT.hi\endcsname{.021}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.LOC.4\endcsname{0.0057}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.LOC.hi\endcsname{.015}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V1\endcsname{0.037}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V1.4\endcsname{0.0372}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V1.hi\endcsname{.053}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V1.lo\endcsname{.023}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V2\endcsname{0.021}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V2.4\endcsname{0.0207}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V2.hi\endcsname{.033}
\expandafter\def\csname nv@rho.mr.all.bn.stdp.V2.lo\endcsname{.010}
\expandafter\def\csname nv@rho.mr.all.ref.bp.IT\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.all.ref.bp.IT.4\endcsname{0.0133}
\expandafter\def\csname nv@rho.mr.all.ref.bp.IT.hi\endcsname{.022}
\expandafter\def\csname nv@rho.mr.all.ref.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.all.ref.bp.LOC\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.all.ref.bp.LOC.4\endcsname{0.0116}
\expandafter\def\csname nv@rho.mr.all.ref.bp.LOC.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.all.ref.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V1\endcsname{0.033}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V1.4\endcsname{0.0335}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V1.hi\endcsname{.049}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V1.lo\endcsname{.020}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V2\endcsname{0.018}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V2.4\endcsname{0.0185}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V2.hi\endcsname{.031}
\expandafter\def\csname nv@rho.mr.all.ref.bp.V2.lo\endcsname{.007}
\expandafter\def\csname nv@rho.mr.all.ref.fa.IT\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.all.ref.fa.IT.4\endcsname{0.0116}
\expandafter\def\csname nv@rho.mr.all.ref.fa.IT.hi\endcsname{.020}
\expandafter\def\csname nv@rho.mr.all.ref.fa.IT.lo\endcsname{.002}
\expandafter\def\csname nv@rho.mr.all.ref.fa.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.ref.fa.LOC.4\endcsname{0.0056}
\expandafter\def\csname nv@rho.mr.all.ref.fa.LOC.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.all.ref.fa.LOC.lo\endcsname{-.005}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V1\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V1.4\endcsname{0.0117}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V1.hi\endcsname{.026}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V1.lo\endcsname{.000}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V2.4\endcsname{0.0039}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V2.hi\endcsname{.015}
\expandafter\def\csname nv@rho.mr.all.ref.fa.V2.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.all.ref.pc.IT\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.all.ref.pc.IT.4\endcsname{0.0136}
\expandafter\def\csname nv@rho.mr.all.ref.pc.IT.hi\endcsname{.022}
\expandafter\def\csname nv@rho.mr.all.ref.pc.IT.lo\endcsname{.006}
\expandafter\def\csname nv@rho.mr.all.ref.pc.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.ref.pc.LOC.4\endcsname{0.0060}
\expandafter\def\csname nv@rho.mr.all.ref.pc.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.mr.all.ref.pc.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V1\endcsname{0.056}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V1.4\endcsname{0.0561}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V1.hi\endcsname{.074}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V1.lo\endcsname{.040}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V2\endcsname{0.028}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V2.4\endcsname{0.0279}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V2.hi\endcsname{.040}
\expandafter\def\csname nv@rho.mr.all.ref.pc.V2.lo\endcsname{.017}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.IT.4\endcsname{0.0078}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.IT.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.IT.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.LOC\endcsname{-0.005}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.LOC.4\endcsname{-0.0051}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.LOC.hi\endcsname{.005}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.LOC.lo\endcsname{-.016}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V1\endcsname{0.075}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V1.4\endcsname{0.0755}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V1.hi\endcsname{.098}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V1.lo\endcsname{.055}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V2\endcsname{0.043}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V2.4\endcsname{0.0433}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V2.hi\endcsname{.060}
\expandafter\def\csname nv@rho.mr.all.ref.rnd.V2.lo\endcsname{.028}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.IT\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.IT.4\endcsname{0.0119}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.IT.hi\endcsname{.019}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.LOC.4\endcsname{0.0058}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V1\endcsname{0.064}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V1.4\endcsname{0.0641}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V1.hi\endcsname{.082}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V1.lo\endcsname{.048}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V2\endcsname{0.036}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V2.4\endcsname{0.0358}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V2.hi\endcsname{.048}
\expandafter\def\csname nv@rho.mr.all.ref.stdp.V2.lo\endcsname{.024}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.IT\endcsname{0.015}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.IT.4\endcsname{0.0149}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.IT.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.IT.lo\endcsname{.006}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.LOC\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.LOC.4\endcsname{0.0133}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.LOC.hi\endcsname{.027}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V1\endcsname{0.034}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V1.4\endcsname{0.0341}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V1.hi\endcsname{.050}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V1.lo\endcsname{.020}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V2\endcsname{0.019}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V2.4\endcsname{0.0186}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V2.hi\endcsname{.031}
\expandafter\def\csname nv@rho.mr.cr.bn.bp.V2.lo\endcsname{.007}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.IT\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.IT.4\endcsname{0.0140}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.IT.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.LOC.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.LOC.hi\endcsname{.019}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.LOC.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V1\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V1.4\endcsname{0.0135}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V1.hi\endcsname{.028}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V1.lo\endcsname{.000}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V2\endcsname{0.005}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V2.4\endcsname{0.0052}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V2.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.cr.bn.fa.V2.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.IT\endcsname{0.013}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.IT.4\endcsname{0.0130}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.IT.hi\endcsname{.023}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.LOC\endcsname{0.007}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.LOC.4\endcsname{0.0070}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.LOC.hi\endcsname{.018}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V1\endcsname{0.018}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V1.4\endcsname{0.0183}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V1.hi\endcsname{.034}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V1.lo\endcsname{.006}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V2\endcsname{0.009}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V2.4\endcsname{0.0085}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V2.hi\endcsname{.020}
\expandafter\def\csname nv@rho.mr.cr.bn.pc.V2.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.IT\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.IT.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.IT.hi\endcsname{.016}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.IT.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.LOC\endcsname{-0.007}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.LOC.4\endcsname{-0.0071}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.LOC.lo\endcsname{-.018}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V1\endcsname{0.077}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V1.4\endcsname{0.0767}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V1.hi\endcsname{.099}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V1.lo\endcsname{.055}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V2\endcsname{0.043}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V2.4\endcsname{0.0435}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V2.hi\endcsname{.061}
\expandafter\def\csname nv@rho.mr.cr.bn.rnd.V2.lo\endcsname{.027}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.IT\endcsname{0.015}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.IT.4\endcsname{0.0147}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.IT.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.IT.lo\endcsname{.005}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.LOC\endcsname{0.007}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.LOC.4\endcsname{0.0065}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.LOC.hi\endcsname{.017}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V1\endcsname{0.039}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V1.4\endcsname{0.0393}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V1.hi\endcsname{.056}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V1.lo\endcsname{.025}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V2\endcsname{0.022}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V2.4\endcsname{0.0220}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V2.hi\endcsname{.035}
\expandafter\def\csname nv@rho.mr.cr.bn.stdp.V2.lo\endcsname{.010}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.IT\endcsname{0.015}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.IT.4\endcsname{0.0154}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.IT.hi\endcsname{.025}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.IT.lo\endcsname{.005}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.LOC\endcsname{0.012}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.LOC.4\endcsname{0.0124}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.LOC.hi\endcsname{.026}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.LOC.lo\endcsname{-.000}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V1\endcsname{0.036}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V1.4\endcsname{0.0363}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V1.hi\endcsname{.052}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V1.lo\endcsname{.022}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V2\endcsname{0.020}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V2.4\endcsname{0.0202}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V2.hi\endcsname{.033}
\expandafter\def\csname nv@rho.mr.cr.ref.bp.V2.lo\endcsname{.008}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.IT\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.IT.4\endcsname{0.0141}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.IT.hi\endcsname{.024}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.LOC\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.LOC.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.LOC.hi\endcsname{.019}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.LOC.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V1\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V1.4\endcsname{0.0137}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V1.hi\endcsname{.028}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V1.lo\endcsname{.000}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V2\endcsname{0.005}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V2.4\endcsname{0.0051}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V2.hi\endcsname{.016}
\expandafter\def\csname nv@rho.mr.cr.ref.fa.V2.lo\endcsname{-.006}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.IT\endcsname{0.014}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.IT.4\endcsname{0.0137}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.IT.hi\endcsname{.023}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.IT.lo\endcsname{.005}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.LOC\endcsname{0.005}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.LOC.4\endcsname{0.0050}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.LOC.hi\endcsname{.013}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V1\endcsname{0.056}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V1.4\endcsname{0.0565}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V1.hi\endcsname{.074}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V1.lo\endcsname{.040}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V2\endcsname{0.028}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V2.4\endcsname{0.0280}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V2.hi\endcsname{.042}
\expandafter\def\csname nv@rho.mr.cr.ref.pc.V2.lo\endcsname{.016}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.IT\endcsname{0.006}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.IT.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.IT.hi\endcsname{.016}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.IT.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.LOC\endcsname{-0.007}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.LOC.4\endcsname{-0.0071}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.LOC.lo\endcsname{-.018}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V1\endcsname{0.077}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V1.4\endcsname{0.0767}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V1.hi\endcsname{.099}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V1.lo\endcsname{.055}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V2\endcsname{0.043}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V2.4\endcsname{0.0435}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V2.hi\endcsname{.061}
\expandafter\def\csname nv@rho.mr.cr.ref.rnd.V2.lo\endcsname{.027}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.IT\endcsname{0.011}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.IT.4\endcsname{0.0114}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.IT.hi\endcsname{.020}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.LOC\endcsname{0.005}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.LOC.4\endcsname{0.0051}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V1\endcsname{0.065}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V1.4\endcsname{0.0648}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V1.hi\endcsname{.083}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V1.lo\endcsname{.048}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V2\endcsname{0.036}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V2.4\endcsname{0.0361}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V2.hi\endcsname{.050}
\expandafter\def\csname nv@rho.mr.cr.ref.stdp.V2.lo\endcsname{.024}
\expandafter\def\csname nv@rho.ps.all.bn.bp.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.all.bn.bp.IT.4\endcsname{0.0083}
\expandafter\def\csname nv@rho.ps.all.bn.bp.IT.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.all.bn.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.bn.bp.LOC\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.bn.bp.LOC.4\endcsname{0.0075}
\expandafter\def\csname nv@rho.ps.all.bn.bp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.all.bn.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V1\endcsname{0.021}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V1.4\endcsname{0.0207}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V1.hi\endcsname{.031}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V1.lo\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V2\endcsname{0.011}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V2.4\endcsname{0.0113}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V2.hi\endcsname{.019}
\expandafter\def\csname nv@rho.ps.all.bn.bp.V2.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.bn.fa.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.bn.fa.IT.4\endcsname{0.0066}
\expandafter\def\csname nv@rho.ps.all.bn.fa.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.bn.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.all.bn.fa.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.all.bn.fa.LOC.4\endcsname{0.0033}
\expandafter\def\csname nv@rho.ps.all.bn.fa.LOC.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.bn.fa.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V1\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V1.4\endcsname{0.0073}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V1.hi\endcsname{.016}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V1.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V2\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V2.4\endcsname{0.0028}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V2.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.bn.fa.V2.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.ps.all.bn.pc.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.bn.pc.IT.4\endcsname{0.0068}
\expandafter\def\csname nv@rho.ps.all.bn.pc.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.bn.pc.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.all.bn.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.all.bn.pc.LOC.4\endcsname{0.0039}
\expandafter\def\csname nv@rho.ps.all.bn.pc.LOC.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.bn.pc.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V1\endcsname{0.011}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V1.4\endcsname{0.0106}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V1.hi\endcsname{.021}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V1.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V2\endcsname{0.005}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V2.4\endcsname{0.0050}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V2.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.bn.pc.V2.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.IT\endcsname{0.005}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.IT.4\endcsname{0.0048}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.IT.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.IT.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.LOC\endcsname{-0.002}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.LOC.4\endcsname{-0.0021}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.LOC.lo\endcsname{-.008}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V1.4\endcsname{0.0526}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V1.hi\endcsname{.068}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V2.4\endcsname{0.0289}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V2.hi\endcsname{.039}
\expandafter\def\csname nv@rho.ps.all.bn.rnd.V2.lo\endcsname{.019}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.IT.4\endcsname{0.0080}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.IT.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.LOC.4\endcsname{0.0037}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.LOC.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V1\endcsname{0.025}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V1.4\endcsname{0.0252}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V1.hi\endcsname{.036}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V1.lo\endcsname{.016}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V2\endcsname{0.014}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V2.4\endcsname{0.0138}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V2.hi\endcsname{.022}
\expandafter\def\csname nv@rho.ps.all.bn.stdp.V2.lo\endcsname{.007}
\expandafter\def\csname nv@rho.ps.all.ref.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.all.ref.bp.IT.4\endcsname{0.0090}
\expandafter\def\csname nv@rho.ps.all.ref.bp.IT.hi\endcsname{.015}
\expandafter\def\csname nv@rho.ps.all.ref.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.ref.bp.LOC\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.ref.bp.LOC.4\endcsname{0.0070}
\expandafter\def\csname nv@rho.ps.all.ref.bp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.all.ref.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V1.4\endcsname{0.0222}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V1.hi\endcsname{.033}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V1.lo\endcsname{.013}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V2\endcsname{0.012}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V2.4\endcsname{0.0123}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V2.hi\endcsname{.021}
\expandafter\def\csname nv@rho.ps.all.ref.bp.V2.lo\endcsname{.005}
\expandafter\def\csname nv@rho.ps.all.ref.fa.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.ref.fa.IT.4\endcsname{0.0067}
\expandafter\def\csname nv@rho.ps.all.ref.fa.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.ref.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.all.ref.fa.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.all.ref.fa.LOC.4\endcsname{0.0033}
\expandafter\def\csname nv@rho.ps.all.ref.fa.LOC.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.ref.fa.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V1\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V1.4\endcsname{0.0075}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V1.hi\endcsname{.016}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V1.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V2\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V2.4\endcsname{0.0028}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V2.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.ref.fa.V2.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.ps.all.ref.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.all.ref.pc.IT.4\endcsname{0.0085}
\expandafter\def\csname nv@rho.ps.all.ref.pc.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.all.ref.pc.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.ref.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.all.ref.pc.LOC.4\endcsname{0.0040}
\expandafter\def\csname nv@rho.ps.all.ref.pc.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.all.ref.pc.LOC.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V1\endcsname{0.038}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V1.4\endcsname{0.0384}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V1.hi\endcsname{.051}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V1.lo\endcsname{.027}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V2\endcsname{0.019}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V2.4\endcsname{0.0186}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V2.hi\endcsname{.026}
\expandafter\def\csname nv@rho.ps.all.ref.pc.V2.lo\endcsname{.011}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.IT\endcsname{0.005}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.IT.4\endcsname{0.0048}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.IT.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.IT.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.LOC\endcsname{-0.002}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.LOC.4\endcsname{-0.0021}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.LOC.lo\endcsname{-.008}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V1.4\endcsname{0.0526}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V1.hi\endcsname{.068}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V2.4\endcsname{0.0289}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V2.hi\endcsname{.039}
\expandafter\def\csname nv@rho.ps.all.ref.rnd.V2.lo\endcsname{.019}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.IT.4\endcsname{0.0073}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.LOC.4\endcsname{0.0038}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.LOC.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V1\endcsname{0.044}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V1.4\endcsname{0.0440}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V1.hi\endcsname{.056}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V1.lo\endcsname{.033}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V2\endcsname{0.024}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V2.4\endcsname{0.0237}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V2.hi\endcsname{.032}
\expandafter\def\csname nv@rho.ps.all.ref.stdp.V2.lo\endcsname{.016}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.IT.4\endcsname{0.0094}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.IT.hi\endcsname{.015}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.LOC.4\endcsname{0.0080}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.LOC.hi\endcsname{.015}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V1.4\endcsname{0.0224}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V1.hi\endcsname{.033}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V1.lo\endcsname{.013}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V2\endcsname{0.012}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V2.4\endcsname{0.0123}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V2.hi\endcsname{.020}
\expandafter\def\csname nv@rho.ps.cr.bn.bp.V2.lo\endcsname{.005}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.IT.4\endcsname{0.0078}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.LOC.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.LOC.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V1\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V1.4\endcsname{0.0086}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V1.hi\endcsname{.018}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V1.lo\endcsname{.000}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V2.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V2.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.bn.fa.V2.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.IT.4\endcsname{0.0077}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.IT.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.IT.lo\endcsname{.002}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.LOC.4\endcsname{0.0043}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.LOC.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V1\endcsname{0.012}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V1.4\endcsname{0.0119}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V1.hi\endcsname{.022}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V1.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V2\endcsname{0.006}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V2.4\endcsname{0.0057}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V2.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.cr.bn.pc.V2.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.IT.4\endcsname{0.0040}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.IT.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.IT.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.LOC\endcsname{-0.003}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.LOC.4\endcsname{-0.0030}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.LOC.lo\endcsname{-.010}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V1.4\endcsname{0.0532}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V1.hi\endcsname{.069}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V2.4\endcsname{0.0288}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V2.hi\endcsname{.040}
\expandafter\def\csname nv@rho.ps.cr.bn.rnd.V2.lo\endcsname{.019}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.IT\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.IT.4\endcsname{0.0087}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.LOC.4\endcsname{0.0043}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.LOC.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V1\endcsname{0.027}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V1.4\endcsname{0.0265}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V1.hi\endcsname{.037}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V1.lo\endcsname{.017}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V2\endcsname{0.015}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V2.4\endcsname{0.0146}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V2.hi\endcsname{.023}
\expandafter\def\csname nv@rho.ps.cr.bn.stdp.V2.lo\endcsname{.007}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.IT\endcsname{0.010}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.IT.4\endcsname{0.0100}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.IT.hi\endcsname{.016}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.LOC.4\endcsname{0.0075}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.LOC.hi\endcsname{.015}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.LOC.lo\endcsname{.000}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V1\endcsname{0.024}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V1.4\endcsname{0.0240}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V1.hi\endcsname{.035}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V1.lo\endcsname{.015}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V2\endcsname{0.013}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V2.4\endcsname{0.0133}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V2.hi\endcsname{.022}
\expandafter\def\csname nv@rho.ps.cr.ref.bp.V2.lo\endcsname{.005}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.IT.4\endcsname{0.0079}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.LOC.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.LOC.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V1\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V1.4\endcsname{0.0087}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V1.hi\endcsname{.018}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V1.lo\endcsname{.000}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V2\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V2.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V2.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.ref.fa.V2.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.IT.4\endcsname{0.0083}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.LOC.4\endcsname{0.0035}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.LOC.hi\endcsname{.008}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V1\endcsname{0.039}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V1.4\endcsname{0.0387}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V1.hi\endcsname{.051}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V1.lo\endcsname{.027}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V2\endcsname{0.019}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V2.4\endcsname{0.0185}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V2.hi\endcsname{.027}
\expandafter\def\csname nv@rho.ps.cr.ref.pc.V2.lo\endcsname{.011}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.IT.4\endcsname{0.0040}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.IT.hi\endcsname{.010}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.IT.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.LOC\endcsname{-0.003}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.LOC.4\endcsname{-0.0030}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.LOC.hi\endcsname{.004}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.LOC.lo\endcsname{-.010}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V1.4\endcsname{0.0532}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V1.hi\endcsname{.069}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V2\endcsname{0.029}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V2.4\endcsname{0.0288}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V2.hi\endcsname{.040}
\expandafter\def\csname nv@rho.ps.cr.ref.rnd.V2.lo\endcsname{.019}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.IT.4\endcsname{0.0070}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.IT.lo\endcsname{.002}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.LOC.4\endcsname{0.0035}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V1\endcsname{0.045}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V1.4\endcsname{0.0445}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V1.hi\endcsname{.057}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V1.lo\endcsname{.033}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V2\endcsname{0.024}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V2.4\endcsname{0.0238}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V2.hi\endcsname{.032}
\expandafter\def\csname nv@rho.ps.cr.ref.stdp.V2.lo\endcsname{.016}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.IT\endcsname{0.009}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.IT.4\endcsname{0.0090}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.IT.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.LOC\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.LOC.4\endcsname{0.0076}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V1\endcsname{0.021}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V1.4\endcsname{0.0207}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V1.hi\endcsname{.031}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V1.lo\endcsname{.012}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V2\endcsname{0.010}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V2.4\endcsname{0.0104}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V2.hi\endcsname{.018}
\expandafter\def\csname nv@rho.ps.crb.bn.bp.V2.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.IT\endcsname{0.006}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.IT.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.LOC.4\endcsname{0.0026}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.LOC.lo\endcsname{-.004}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V1\endcsname{0.006}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V1.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V1.hi\endcsname{.016}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V1.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V2\endcsname{0.002}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V2.4\endcsname{0.0015}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V2.hi\endcsname{.008}
\expandafter\def\csname nv@rho.ps.crb.bn.fa.V2.lo\endcsname{-.005}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.IT\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.IT.4\endcsname{0.0066}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.LOC.4\endcsname{0.0029}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.LOC.hi\endcsname{.008}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V1\endcsname{0.010}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V1.4\endcsname{0.0096}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V1.hi\endcsname{.020}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V1.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V2\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V2.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V2.hi\endcsname{.011}
\expandafter\def\csname nv@rho.ps.crb.bn.pc.V2.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.IT\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.IT.4\endcsname{0.0029}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.IT.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.IT.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.LOC\endcsname{-0.005}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.LOC.4\endcsname{-0.0049}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.LOC.hi\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.LOC.lo\endcsname{-.011}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V1.4\endcsname{0.0534}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V1.hi\endcsname{.069}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V2\endcsname{0.028}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V2.4\endcsname{0.0282}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V2.hi\endcsname{.039}
\expandafter\def\csname nv@rho.ps.crb.bn.rnd.V2.lo\endcsname{.018}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.IT.4\endcsname{0.0079}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.IT.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.LOC.4\endcsname{0.0032}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.LOC.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V1\endcsname{0.024}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V1.4\endcsname{0.0242}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V1.hi\endcsname{.035}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V1.lo\endcsname{.014}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V2\endcsname{0.012}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V2.4\endcsname{0.0123}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V2.hi\endcsname{.020}
\expandafter\def\csname nv@rho.ps.crb.bn.stdp.V2.lo\endcsname{.005}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.IT\endcsname{0.010}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.IT.4\endcsname{0.0097}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.IT.hi\endcsname{.015}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.IT.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.LOC\endcsname{0.007}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.LOC.4\endcsname{0.0074}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.LOC.hi\endcsname{.014}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.LOC.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V1\endcsname{0.022}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V1.4\endcsname{0.0221}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V1.hi\endcsname{.033}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V1.lo\endcsname{.013}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V2\endcsname{0.011}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V2.4\endcsname{0.0112}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V2.hi\endcsname{.019}
\expandafter\def\csname nv@rho.ps.crb.ref.bp.V2.lo\endcsname{.004}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.IT\endcsname{0.006}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.IT.4\endcsname{0.0063}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.IT.lo\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.LOC.4\endcsname{0.0026}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.LOC.lo\endcsname{-.003}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V1\endcsname{0.006}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V1.4\endcsname{0.0065}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V1.hi\endcsname{.017}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V1.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V2\endcsname{0.002}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V2.4\endcsname{0.0015}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V2.hi\endcsname{.008}
\expandafter\def\csname nv@rho.ps.crb.ref.fa.V2.lo\endcsname{-.005}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.IT.4\endcsname{0.0082}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.IT.hi\endcsname{.013}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.LOC\endcsname{0.004}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.LOC.4\endcsname{0.0036}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.LOC.hi\endcsname{.008}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.LOC.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V1\endcsname{0.040}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V1.4\endcsname{0.0396}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V1.hi\endcsname{.052}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V1.lo\endcsname{.028}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V2\endcsname{0.019}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V2.4\endcsname{0.0188}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V2.hi\endcsname{.027}
\expandafter\def\csname nv@rho.ps.crb.ref.pc.V2.lo\endcsname{.011}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.IT\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.IT.4\endcsname{0.0029}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.IT.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.IT.lo\endcsname{-.002}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.LOC\endcsname{-0.005}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.LOC.4\endcsname{-0.0049}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.LOC.hi\endcsname{.001}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.LOC.lo\endcsname{-.011}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V1\endcsname{0.053}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V1.4\endcsname{0.0534}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V1.hi\endcsname{.069}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V1.lo\endcsname{.039}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V2\endcsname{0.028}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V2.4\endcsname{0.0282}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V2.hi\endcsname{.039}
\expandafter\def\csname nv@rho.ps.crb.ref.rnd.V2.lo\endcsname{.018}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.IT\endcsname{0.008}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.IT.4\endcsname{0.0077}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.IT.hi\endcsname{.012}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.IT.lo\endcsname{.003}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.LOC\endcsname{0.003}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.LOC.4\endcsname{0.0035}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.LOC.hi\endcsname{.009}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.LOC.lo\endcsname{-.001}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V1\endcsname{0.044}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V1.4\endcsname{0.0443}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V1.hi\endcsname{.057}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V1.lo\endcsname{.033}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V2\endcsname{0.023}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V2.4\endcsname{0.0233}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V2.hi\endcsname{.032}
\expandafter\def\csname nv@rho.ps.crb.ref.stdp.V2.lo\endcsname{.015}
\expandafter\def\csname nv@rp.IT.p\endcsname{0.226}
\expandafter\def\csname nv@rp.IT.rho\endcsname{0.097}
\expandafter\def\csname nv@rp.LOC.p\endcsname{0.160}
\expandafter\def\csname nv@rp.LOC.rho\endcsname{0.171}
\expandafter\def\csname nv@rp.V1.p\endcsname{0.336}
\expandafter\def\csname nv@rp.V1.rho\endcsname{0.055}
\expandafter\def\csname nv@rp.V2.p\endcsname{0.323}
\expandafter\def\csname nv@rp.V2.rho\endcsname{0.065}
\expandafter\def\csname nv@rp.nperm\endcsname{3{,}628{,}800}
\expandafter\def\csname nv@seed.bp.IT.max\endcsname{0.0105}
\expandafter\def\csname nv@seed.bp.IT.min\endcsname{0.0086}
\expandafter\def\csname nv@seed.bp.IT.sd\endcsname{0.0007}
\expandafter\def\csname nv@seed.bp.LOC.max\endcsname{0.0088}
\expandafter\def\csname nv@seed.bp.LOC.min\endcsname{0.0076}
\expandafter\def\csname nv@seed.bp.LOC.sd\endcsname{0.0005}
\expandafter\def\csname nv@seed.bp.V1.max\endcsname{0.0297}
\expandafter\def\csname nv@seed.bp.V1.min\endcsname{0.0182}
\expandafter\def\csname nv@seed.bp.V1.sd\endcsname{0.0045}
\expandafter\def\csname nv@seed.bp.V2.max\endcsname{0.0164}
\expandafter\def\csname nv@seed.bp.V2.min\endcsname{0.0097}
\expandafter\def\csname nv@seed.bp.V2.sd\endcsname{0.0025}
\expandafter\def\csname nv@seed.fa.IT.max\endcsname{0.0086}
\expandafter\def\csname nv@seed.fa.IT.min\endcsname{0.0072}
\expandafter\def\csname nv@seed.fa.IT.sd\endcsname{0.0005}
\expandafter\def\csname nv@seed.fa.LOC.max\endcsname{0.0043}
\expandafter\def\csname nv@seed.fa.LOC.min\endcsname{0.0030}
\expandafter\def\csname nv@seed.fa.LOC.sd\endcsname{0.0006}
\expandafter\def\csname nv@seed.fa.V1.max\endcsname{0.0150}
\expandafter\def\csname nv@seed.fa.V1.min\endcsname{0.0026}
\expandafter\def\csname nv@seed.fa.V1.sd\endcsname{0.0045}
\expandafter\def\csname nv@seed.fa.V2.max\endcsname{0.0058}
\expandafter\def\csname nv@seed.fa.V2.min\endcsname{0.0022}
\expandafter\def\csname nv@seed.fa.V2.sd\endcsname{0.0014}
\expandafter\def\csname nv@seed.pc.IT.max\endcsname{0.0087}
\expandafter\def\csname nv@seed.pc.IT.min\endcsname{0.0068}
\expandafter\def\csname nv@seed.pc.IT.sd\endcsname{0.0007}
\expandafter\def\csname nv@seed.pc.LOC.max\endcsname{0.0058}
\expandafter\def\csname nv@seed.pc.LOC.min\endcsname{0.0025}
\expandafter\def\csname nv@seed.pc.LOC.sd\endcsname{0.0014}
\expandafter\def\csname nv@seed.pc.V1.max\endcsname{0.0175}
\expandafter\def\csname nv@seed.pc.V1.min\endcsname{0.0090}
\expandafter\def\csname nv@seed.pc.V1.sd\endcsname{0.0032}
\expandafter\def\csname nv@seed.pc.V2.max\endcsname{0.0080}
\expandafter\def\csname nv@seed.pc.V2.min\endcsname{0.0042}
\expandafter\def\csname nv@seed.pc.V2.sd\endcsname{0.0014}
\expandafter\def\csname nv@seed.rnd.IT.max\endcsname{0.0073}
\expandafter\def\csname nv@seed.rnd.IT.min\endcsname{0.0020}
\expandafter\def\csname nv@seed.rnd.IT.sd\endcsname{0.0020}
\expandafter\def\csname nv@seed.rnd.LOC.max\endcsname{-0.0007}
\expandafter\def\csname nv@seed.rnd.LOC.min\endcsname{-0.0052}
\expandafter\def\csname nv@seed.rnd.LOC.sd\endcsname{0.0019}
\expandafter\def\csname nv@seed.rnd.V1.max\endcsname{0.0594}
\expandafter\def\csname nv@seed.rnd.V1.min\endcsname{0.0446}
\expandafter\def\csname nv@seed.rnd.V1.sd\endcsname{0.0059}
\expandafter\def\csname nv@seed.rnd.V2.max\endcsname{0.0331}
\expandafter\def\csname nv@seed.rnd.V2.min\endcsname{0.0239}
\expandafter\def\csname nv@seed.rnd.V2.sd\endcsname{0.0035}
\expandafter\def\csname nv@seed.stdp.IT.max\endcsname{0.0105}
\expandafter\def\csname nv@seed.stdp.IT.min\endcsname{0.0059}
\expandafter\def\csname nv@seed.stdp.IT.sd\endcsname{0.0018}
\expandafter\def\csname nv@seed.stdp.LOC.max\endcsname{0.0058}
\expandafter\def\csname nv@seed.stdp.LOC.min\endcsname{0.0029}
\expandafter\def\csname nv@seed.stdp.LOC.sd\endcsname{0.0011}
\expandafter\def\csname nv@seed.stdp.V1.max\endcsname{0.0304}
\expandafter\def\csname nv@seed.stdp.V1.min\endcsname{0.0218}
\expandafter\def\csname nv@seed.stdp.V1.sd\endcsname{0.0040}
\expandafter\def\csname nv@seed.stdp.V2.max\endcsname{0.0170}
\expandafter\def\csname nv@seed.stdp.V2.min\endcsname{0.0111}
\expandafter\def\csname nv@seed.stdp.V2.sd\endcsname{0.0026}
\expandafter\def\csname nv@seed5.bp.IT.min\endcsname{0.00865}
\expandafter\def\csname nv@seed5.fa.IT.max\endcsname{0.00862}
\expandafter\def\csname nv@seed5.rnd.IT.max\endcsname{0.00725}
\expandafter\def\csname nv@seedsd.it.max\endcsname{0.0020}
\expandafter\def\csname nv@seedsd.it.min\endcsname{0.0005}
\expandafter\def\csname nv@seedsd.v12.max\endcsname{0.006}
\expandafter\def\csname nv@seedsd.v12.min\endcsname{0.001}
\expandafter\def\csname nv@sens.maxdiff\endcsname{0.002}
\expandafter\def\csname nv@sub.s1.bp.IT\endcsname{0.011}
\expandafter\def\csname nv@sub.s1.bp.IT.hi\endcsname{0.018}
\expandafter\def\csname nv@sub.s1.bp.IT.lo\endcsname{0.004}
\expandafter\def\csname nv@sub.s1.bp.LOC\endcsname{0.006}
\expandafter\def\csname nv@sub.s1.bp.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@sub.s1.bp.LOC.lo\endcsname{-0.001}
\expandafter\def\csname nv@sub.s1.bp.V1\endcsname{0.021}
\expandafter\def\csname nv@sub.s1.bp.V1.hi\endcsname{0.035}
\expandafter\def\csname nv@sub.s1.bp.V1.lo\endcsname{0.009}
\expandafter\def\csname nv@sub.s1.bp.V2\endcsname{0.011}
\expandafter\def\csname nv@sub.s1.bp.V2.hi\endcsname{0.021}
\expandafter\def\csname nv@sub.s1.bp.V2.lo\endcsname{0.001}
\expandafter\def\csname nv@sub.s1.fa.IT\endcsname{0.009}
\expandafter\def\csname nv@sub.s1.fa.IT.hi\endcsname{0.018}
\expandafter\def\csname nv@sub.s1.fa.IT.lo\endcsname{0.000}
\expandafter\def\csname nv@sub.s1.fa.LOC\endcsname{0.005}
\expandafter\def\csname nv@sub.s1.fa.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@sub.s1.fa.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s1.fa.V1\endcsname{0.003}
\expandafter\def\csname nv@sub.s1.fa.V1.hi\endcsname{0.016}
\expandafter\def\csname nv@sub.s1.fa.V1.lo\endcsname{-0.009}
\expandafter\def\csname nv@sub.s1.fa.V2\endcsname{-0.000}
\expandafter\def\csname nv@sub.s1.fa.V2.hi\endcsname{0.009}
\expandafter\def\csname nv@sub.s1.fa.V2.lo\endcsname{-0.009}
\expandafter\def\csname nv@sub.s1.pc.IT\endcsname{0.009}
\expandafter\def\csname nv@sub.s1.pc.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@sub.s1.pc.IT.lo\endcsname{0.001}
\expandafter\def\csname nv@sub.s1.pc.LOC\endcsname{0.005}
\expandafter\def\csname nv@sub.s1.pc.LOC.hi\endcsname{0.014}
\expandafter\def\csname nv@sub.s1.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s1.pc.V1\endcsname{0.007}
\expandafter\def\csname nv@sub.s1.pc.V1.hi\endcsname{0.020}
\expandafter\def\csname nv@sub.s1.pc.V1.lo\endcsname{-0.006}
\expandafter\def\csname nv@sub.s1.pc.V2\endcsname{0.003}
\expandafter\def\csname nv@sub.s1.pc.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@sub.s1.pc.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@sub.s1.rnd.IT\endcsname{0.001}
\expandafter\def\csname nv@sub.s1.rnd.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@sub.s1.rnd.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@sub.s1.rnd.LOC\endcsname{0.005}
\expandafter\def\csname nv@sub.s1.rnd.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@sub.s1.rnd.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s1.rnd.V1\endcsname{0.054}
\expandafter\def\csname nv@sub.s1.rnd.V1.hi\endcsname{0.075}
\expandafter\def\csname nv@sub.s1.rnd.V1.lo\endcsname{0.033}
\expandafter\def\csname nv@sub.s1.rnd.V2\endcsname{0.033}
\expandafter\def\csname nv@sub.s1.rnd.V2.hi\endcsname{0.049}
\expandafter\def\csname nv@sub.s1.rnd.V2.lo\endcsname{0.018}
\expandafter\def\csname nv@sub.s1.stdp.IT\endcsname{0.010}
\expandafter\def\csname nv@sub.s1.stdp.IT.hi\endcsname{0.018}
\expandafter\def\csname nv@sub.s1.stdp.IT.lo\endcsname{0.002}
\expandafter\def\csname nv@sub.s1.stdp.LOC\endcsname{0.007}
\expandafter\def\csname nv@sub.s1.stdp.LOC.hi\endcsname{0.015}
\expandafter\def\csname nv@sub.s1.stdp.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@sub.s1.stdp.V1\endcsname{0.024}
\expandafter\def\csname nv@sub.s1.stdp.V1.hi\endcsname{0.039}
\expandafter\def\csname nv@sub.s1.stdp.V1.lo\endcsname{0.011}
\expandafter\def\csname nv@sub.s1.stdp.V2\endcsname{0.013}
\expandafter\def\csname nv@sub.s1.stdp.V2.hi\endcsname{0.023}
\expandafter\def\csname nv@sub.s1.stdp.V2.lo\endcsname{0.003}
\expandafter\def\csname nv@sub.s2.bp.IT\endcsname{0.011}
\expandafter\def\csname nv@sub.s2.bp.IT.hi\endcsname{0.023}
\expandafter\def\csname nv@sub.s2.bp.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@sub.s2.bp.LOC\endcsname{0.014}
\expandafter\def\csname nv@sub.s2.bp.LOC.hi\endcsname{0.034}
\expandafter\def\csname nv@sub.s2.bp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@sub.s2.bp.V1\endcsname{0.037}
\expandafter\def\csname nv@sub.s2.bp.V1.hi\endcsname{0.057}
\expandafter\def\csname nv@sub.s2.bp.V1.lo\endcsname{0.019}
\expandafter\def\csname nv@sub.s2.bp.V2\endcsname{0.021}
\expandafter\def\csname nv@sub.s2.bp.V2.hi\endcsname{0.038}
\expandafter\def\csname nv@sub.s2.bp.V2.lo\endcsname{0.006}
\expandafter\def\csname nv@sub.s2.fa.IT\endcsname{0.011}
\expandafter\def\csname nv@sub.s2.fa.IT.hi\endcsname{0.024}
\expandafter\def\csname nv@sub.s2.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s2.fa.LOC\endcsname{0.007}
\expandafter\def\csname nv@sub.s2.fa.LOC.hi\endcsname{0.025}
\expandafter\def\csname nv@sub.s2.fa.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@sub.s2.fa.V1\endcsname{0.018}
\expandafter\def\csname nv@sub.s2.fa.V1.hi\endcsname{0.037}
\expandafter\def\csname nv@sub.s2.fa.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@sub.s2.fa.V2\endcsname{0.009}
\expandafter\def\csname nv@sub.s2.fa.V2.hi\endcsname{0.025}
\expandafter\def\csname nv@sub.s2.fa.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@sub.s2.pc.IT\endcsname{0.010}
\expandafter\def\csname nv@sub.s2.pc.IT.hi\endcsname{0.024}
\expandafter\def\csname nv@sub.s2.pc.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s2.pc.LOC\endcsname{0.007}
\expandafter\def\csname nv@sub.s2.pc.LOC.hi\endcsname{0.023}
\expandafter\def\csname nv@sub.s2.pc.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@sub.s2.pc.V1\endcsname{0.023}
\expandafter\def\csname nv@sub.s2.pc.V1.hi\endcsname{0.041}
\expandafter\def\csname nv@sub.s2.pc.V1.lo\endcsname{0.006}
\expandafter\def\csname nv@sub.s2.pc.V2\endcsname{0.012}
\expandafter\def\csname nv@sub.s2.pc.V2.hi\endcsname{0.028}
\expandafter\def\csname nv@sub.s2.pc.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s2.rnd.IT\endcsname{0.007}
\expandafter\def\csname nv@sub.s2.rnd.IT.hi\endcsname{0.020}
\expandafter\def\csname nv@sub.s2.rnd.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@sub.s2.rnd.LOC\endcsname{-0.009}
\expandafter\def\csname nv@sub.s2.rnd.LOC.hi\endcsname{0.007}
\expandafter\def\csname nv@sub.s2.rnd.LOC.lo\endcsname{-0.026}
\expandafter\def\csname nv@sub.s2.rnd.V1\endcsname{0.089}
\expandafter\def\csname nv@sub.s2.rnd.V1.hi\endcsname{0.117}
\expandafter\def\csname nv@sub.s2.rnd.V1.lo\endcsname{0.061}
\expandafter\def\csname nv@sub.s2.rnd.V2\endcsname{0.050}
\expandafter\def\csname nv@sub.s2.rnd.V2.hi\endcsname{0.071}
\expandafter\def\csname nv@sub.s2.rnd.V2.lo\endcsname{0.029}
\expandafter\def\csname nv@sub.s2.stdp.IT\endcsname{0.011}
\expandafter\def\csname nv@sub.s2.stdp.IT.hi\endcsname{0.023}
\expandafter\def\csname nv@sub.s2.stdp.IT.lo\endcsname{0.001}
\expandafter\def\csname nv@sub.s2.stdp.LOC\endcsname{0.007}
\expandafter\def\csname nv@sub.s2.stdp.LOC.hi\endcsname{0.021}
\expandafter\def\csname nv@sub.s2.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@sub.s2.stdp.V1\endcsname{0.048}
\expandafter\def\csname nv@sub.s2.stdp.V1.hi\endcsname{0.068}
\expandafter\def\csname nv@sub.s2.stdp.V1.lo\endcsname{0.029}
\expandafter\def\csname nv@sub.s2.stdp.V2\endcsname{0.028}
\expandafter\def\csname nv@sub.s2.stdp.V2.hi\endcsname{0.046}
\expandafter\def\csname nv@sub.s2.stdp.V2.lo\endcsname{0.012}
\expandafter\def\csname nv@sub.s3.bp.IT\endcsname{0.006}
\expandafter\def\csname nv@sub.s3.bp.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@sub.s3.bp.IT.lo\endcsname{-0.001}
\expandafter\def\csname nv@sub.s3.bp.LOC\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.bp.LOC.hi\endcsname{0.013}
\expandafter\def\csname nv@sub.s3.bp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@sub.s3.bp.V1\endcsname{0.009}
\expandafter\def\csname nv@sub.s3.bp.V1.hi\endcsname{0.018}
\expandafter\def\csname nv@sub.s3.bp.V1.lo\endcsname{0.002}
\expandafter\def\csname nv@sub.s3.bp.V2\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.bp.V2.hi\endcsname{0.013}
\expandafter\def\csname nv@sub.s3.bp.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@sub.s3.fa.IT\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.fa.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@sub.s3.fa.IT.lo\endcsname{-0.003}
\expandafter\def\csname nv@sub.s3.fa.LOC\endcsname{-0.001}
\expandafter\def\csname nv@sub.s3.fa.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@sub.s3.fa.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@sub.s3.fa.V1\endcsname{0.005}
\expandafter\def\csname nv@sub.s3.fa.V1.hi\endcsname{0.014}
\expandafter\def\csname nv@sub.s3.fa.V1.lo\endcsname{-0.002}
\expandafter\def\csname nv@sub.s3.fa.V2\endcsname{0.002}
\expandafter\def\csname nv@sub.s3.fa.V2.hi\endcsname{0.010}
\expandafter\def\csname nv@sub.s3.fa.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@sub.s3.pc.IT\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.pc.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@sub.s3.pc.IT.lo\endcsname{-0.002}
\expandafter\def\csname nv@sub.s3.pc.LOC\endcsname{0.000}
\expandafter\def\csname nv@sub.s3.pc.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@sub.s3.pc.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@sub.s3.pc.V1\endcsname{0.006}
\expandafter\def\csname nv@sub.s3.pc.V1.hi\endcsname{0.015}
\expandafter\def\csname nv@sub.s3.pc.V1.lo\endcsname{-0.001}
\expandafter\def\csname nv@sub.s3.pc.V2\endcsname{0.002}
\expandafter\def\csname nv@sub.s3.pc.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@sub.s3.pc.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@sub.s3.rnd.IT\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.rnd.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@sub.s3.rnd.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@sub.s3.rnd.LOC\endcsname{-0.004}
\expandafter\def\csname nv@sub.s3.rnd.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@sub.s3.rnd.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@sub.s3.rnd.V1\endcsname{0.017}
\expandafter\def\csname nv@sub.s3.rnd.V1.hi\endcsname{0.028}
\expandafter\def\csname nv@sub.s3.rnd.V1.lo\endcsname{0.007}
\expandafter\def\csname nv@sub.s3.rnd.V2\endcsname{0.003}
\expandafter\def\csname nv@sub.s3.rnd.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@sub.s3.rnd.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@sub.s3.stdp.IT\endcsname{0.005}
\expandafter\def\csname nv@sub.s3.stdp.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@sub.s3.stdp.IT.lo\endcsname{-0.001}
\expandafter\def\csname nv@sub.s3.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@sub.s3.stdp.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@sub.s3.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@sub.s3.stdp.V1\endcsname{0.007}
\expandafter\def\csname nv@sub.s3.stdp.V1.hi\endcsname{0.017}
\expandafter\def\csname nv@sub.s3.stdp.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@sub.s3.stdp.V2\endcsname{0.002}
\expandafter\def\csname nv@sub.s3.stdp.V2.hi\endcsname{0.011}
\expandafter\def\csname nv@sub.s3.stdp.V2.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s1.bp.fa.IT\endcsname{+0.002}
\expandafter\def\csname nv@subd.s1.bp.fa.IT.hi\endcsname{0.011}
\expandafter\def\csname nv@subd.s1.bp.fa.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s1.bp.fa.LOC\endcsname{+0.001}
\expandafter\def\csname nv@subd.s1.bp.fa.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s1.bp.fa.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.bp.fa.V1\endcsname{+0.018}
\expandafter\def\csname nv@subd.s1.bp.fa.V1.hi\endcsname{0.025}
\expandafter\def\csname nv@subd.s1.bp.fa.V1.lo\endcsname{0.012}
\expandafter\def\csname nv@subd.s1.bp.fa.V2\endcsname{+0.012}
\expandafter\def\csname nv@subd.s1.bp.fa.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@subd.s1.bp.fa.V2.lo\endcsname{0.007}
\expandafter\def\csname nv@subd.s1.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@subd.s1.bp.pc.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@subd.s1.bp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s1.bp.pc.LOC\endcsname{+0.001}
\expandafter\def\csname nv@subd.s1.bp.pc.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s1.bp.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.bp.pc.V1\endcsname{+0.014}
\expandafter\def\csname nv@subd.s1.bp.pc.V1.hi\endcsname{0.020}
\expandafter\def\csname nv@subd.s1.bp.pc.V1.lo\endcsname{0.008}
\expandafter\def\csname nv@subd.s1.bp.pc.V2\endcsname{+0.008}
\expandafter\def\csname nv@subd.s1.bp.pc.V2.hi\endcsname{0.012}
\expandafter\def\csname nv@subd.s1.bp.pc.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@subd.s1.bp.stdp.IT\endcsname{+0.001}
\expandafter\def\csname nv@subd.s1.bp.stdp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s1.bp.stdp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.bp.stdp.LOC\endcsname{-0.000}
\expandafter\def\csname nv@subd.s1.bp.stdp.LOC.hi\endcsname{0.007}
\expandafter\def\csname nv@subd.s1.bp.stdp.LOC.lo\endcsname{-0.008}
\expandafter\def\csname nv@subd.s1.bp.stdp.V1\endcsname{-0.004}
\expandafter\def\csname nv@subd.s1.bp.stdp.V1.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s1.bp.stdp.V1.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s1.bp.stdp.V2\endcsname{-0.002}
\expandafter\def\csname nv@subd.s1.bp.stdp.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s1.bp.stdp.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.fa.pc.IT\endcsname{+0.000}
\expandafter\def\csname nv@subd.s1.fa.pc.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s1.fa.pc.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s1.fa.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@subd.s1.fa.pc.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s1.fa.pc.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s1.fa.pc.V1\endcsname{-0.004}
\expandafter\def\csname nv@subd.s1.fa.pc.V1.hi\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.fa.pc.V1.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s1.fa.pc.V2\endcsname{-0.004}
\expandafter\def\csname nv@subd.s1.fa.pc.V2.hi\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.fa.pc.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.fa.stdp.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@subd.s1.fa.stdp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s1.fa.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s1.fa.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s1.fa.stdp.V1\endcsname{-0.022}
\expandafter\def\csname nv@subd.s1.fa.stdp.V1.hi\endcsname{-0.015}
\expandafter\def\csname nv@subd.s1.fa.stdp.V1.lo\endcsname{-0.030}
\expandafter\def\csname nv@subd.s1.fa.stdp.V2\endcsname{-0.014}
\expandafter\def\csname nv@subd.s1.fa.stdp.V2.hi\endcsname{-0.009}
\expandafter\def\csname nv@subd.s1.fa.stdp.V2.lo\endcsname{-0.019}
\expandafter\def\csname nv@subd.s1.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.pc.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s1.pc.stdp.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.pc.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.pc.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s1.pc.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s1.pc.stdp.V1\endcsname{-0.018}
\expandafter\def\csname nv@subd.s1.pc.stdp.V1.hi\endcsname{-0.012}
\expandafter\def\csname nv@subd.s1.pc.stdp.V1.lo\endcsname{-0.024}
\expandafter\def\csname nv@subd.s1.pc.stdp.V2\endcsname{-0.010}
\expandafter\def\csname nv@subd.s1.pc.stdp.V2.hi\endcsname{-0.006}
\expandafter\def\csname nv@subd.s1.pc.stdp.V2.lo\endcsname{-0.015}
\expandafter\def\csname nv@subd.s1.rnd.bp.IT\endcsname{-0.010}
\expandafter\def\csname nv@subd.s1.rnd.bp.IT.hi\endcsname{0.000}
\expandafter\def\csname nv@subd.s1.rnd.bp.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@subd.s1.rnd.bp.LOC\endcsname{-0.002}
\expandafter\def\csname nv@subd.s1.rnd.bp.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s1.rnd.bp.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@subd.s1.rnd.bp.V1\endcsname{+0.033}
\expandafter\def\csname nv@subd.s1.rnd.bp.V1.hi\endcsname{0.051}
\expandafter\def\csname nv@subd.s1.rnd.bp.V1.lo\endcsname{0.016}
\expandafter\def\csname nv@subd.s1.rnd.bp.V2\endcsname{+0.022}
\expandafter\def\csname nv@subd.s1.rnd.bp.V2.hi\endcsname{0.036}
\expandafter\def\csname nv@subd.s1.rnd.bp.V2.lo\endcsname{0.009}
\expandafter\def\csname nv@subd.s1.rnd.fa.IT\endcsname{-0.008}
\expandafter\def\csname nv@subd.s1.rnd.fa.IT.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s1.rnd.fa.IT.lo\endcsname{-0.018}
\expandafter\def\csname nv@subd.s1.rnd.fa.LOC\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.rnd.fa.LOC.hi\endcsname{0.007}
\expandafter\def\csname nv@subd.s1.rnd.fa.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s1.rnd.fa.V1\endcsname{+0.052}
\expandafter\def\csname nv@subd.s1.rnd.fa.V1.hi\endcsname{0.071}
\expandafter\def\csname nv@subd.s1.rnd.fa.V1.lo\endcsname{0.033}
\expandafter\def\csname nv@subd.s1.rnd.fa.V2\endcsname{+0.034}
\expandafter\def\csname nv@subd.s1.rnd.fa.V2.hi\endcsname{0.048}
\expandafter\def\csname nv@subd.s1.rnd.fa.V2.lo\endcsname{0.020}
\expandafter\def\csname nv@subd.s1.rnd.pc.IT\endcsname{-0.008}
\expandafter\def\csname nv@subd.s1.rnd.pc.IT.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s1.rnd.pc.IT.lo\endcsname{-0.016}
\expandafter\def\csname nv@subd.s1.rnd.pc.LOC\endcsname{-0.001}
\expandafter\def\csname nv@subd.s1.rnd.pc.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s1.rnd.pc.LOC.lo\endcsname{-0.008}
\expandafter\def\csname nv@subd.s1.rnd.pc.V1\endcsname{+0.047}
\expandafter\def\csname nv@subd.s1.rnd.pc.V1.hi\endcsname{0.064}
\expandafter\def\csname nv@subd.s1.rnd.pc.V1.lo\endcsname{0.031}
\expandafter\def\csname nv@subd.s1.rnd.pc.V2\endcsname{+0.030}
\expandafter\def\csname nv@subd.s1.rnd.pc.V2.hi\endcsname{0.043}
\expandafter\def\csname nv@subd.s1.rnd.pc.V2.lo\endcsname{0.018}
\expandafter\def\csname nv@subd.s1.rnd.stdp.IT\endcsname{-0.009}
\expandafter\def\csname nv@subd.s1.rnd.stdp.IT.hi\endcsname{-0.000}
\expandafter\def\csname nv@subd.s1.rnd.stdp.IT.lo\endcsname{-0.018}
\expandafter\def\csname nv@subd.s1.rnd.stdp.LOC\endcsname{-0.002}
\expandafter\def\csname nv@subd.s1.rnd.stdp.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s1.rnd.stdp.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V1\endcsname{+0.030}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V1.hi\endcsname{0.046}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V1.lo\endcsname{0.013}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V2\endcsname{+0.020}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V2.hi\endcsname{0.033}
\expandafter\def\csname nv@subd.s1.rnd.stdp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@subd.s2.bp.fa.IT\endcsname{-0.000}
\expandafter\def\csname nv@subd.s2.bp.fa.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@subd.s2.bp.fa.IT.lo\endcsname{-0.012}
\expandafter\def\csname nv@subd.s2.bp.fa.LOC\endcsname{+0.007}
\expandafter\def\csname nv@subd.s2.bp.fa.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@subd.s2.bp.fa.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s2.bp.fa.V1\endcsname{+0.019}
\expandafter\def\csname nv@subd.s2.bp.fa.V1.hi\endcsname{0.028}
\expandafter\def\csname nv@subd.s2.bp.fa.V1.lo\endcsname{0.011}
\expandafter\def\csname nv@subd.s2.bp.fa.V2\endcsname{+0.012}
\expandafter\def\csname nv@subd.s2.bp.fa.V2.hi\endcsname{0.020}
\expandafter\def\csname nv@subd.s2.bp.fa.V2.lo\endcsname{0.005}
\expandafter\def\csname nv@subd.s2.bp.pc.IT\endcsname{+0.000}
\expandafter\def\csname nv@subd.s2.bp.pc.IT.hi\endcsname{0.013}
\expandafter\def\csname nv@subd.s2.bp.pc.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@subd.s2.bp.pc.LOC\endcsname{+0.007}
\expandafter\def\csname nv@subd.s2.bp.pc.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@subd.s2.bp.pc.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s2.bp.pc.V1\endcsname{+0.014}
\expandafter\def\csname nv@subd.s2.bp.pc.V1.hi\endcsname{0.022}
\expandafter\def\csname nv@subd.s2.bp.pc.V1.lo\endcsname{0.007}
\expandafter\def\csname nv@subd.s2.bp.pc.V2\endcsname{+0.010}
\expandafter\def\csname nv@subd.s2.bp.pc.V2.hi\endcsname{0.017}
\expandafter\def\csname nv@subd.s2.bp.pc.V2.lo\endcsname{0.004}
\expandafter\def\csname nv@subd.s2.bp.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s2.bp.stdp.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s2.bp.stdp.IT.lo\endcsname{-0.011}
\expandafter\def\csname nv@subd.s2.bp.stdp.LOC\endcsname{+0.008}
\expandafter\def\csname nv@subd.s2.bp.stdp.LOC.hi\endcsname{0.022}
\expandafter\def\csname nv@subd.s2.bp.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s2.bp.stdp.V1\endcsname{-0.011}
\expandafter\def\csname nv@subd.s2.bp.stdp.V1.hi\endcsname{-0.004}
\expandafter\def\csname nv@subd.s2.bp.stdp.V1.lo\endcsname{-0.018}
\expandafter\def\csname nv@subd.s2.bp.stdp.V2\endcsname{-0.007}
\expandafter\def\csname nv@subd.s2.bp.stdp.V2.hi\endcsname{-0.001}
\expandafter\def\csname nv@subd.s2.bp.stdp.V2.lo\endcsname{-0.013}
\expandafter\def\csname nv@subd.s2.fa.pc.IT\endcsname{+0.001}
\expandafter\def\csname nv@subd.s2.fa.pc.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s2.fa.pc.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@subd.s2.fa.pc.LOC\endcsname{-0.000}
\expandafter\def\csname nv@subd.s2.fa.pc.LOC.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s2.fa.pc.LOC.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s2.fa.pc.V1\endcsname{-0.005}
\expandafter\def\csname nv@subd.s2.fa.pc.V1.hi\endcsname{-0.000}
\expandafter\def\csname nv@subd.s2.fa.pc.V1.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s2.fa.pc.V2\endcsname{-0.003}
\expandafter\def\csname nv@subd.s2.fa.pc.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s2.fa.pc.V2.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s2.fa.stdp.IT\endcsname{-0.000}
\expandafter\def\csname nv@subd.s2.fa.stdp.IT.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s2.fa.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@subd.s2.fa.stdp.LOC\endcsname{+0.000}
\expandafter\def\csname nv@subd.s2.fa.stdp.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s2.fa.stdp.LOC.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s2.fa.stdp.V1\endcsname{-0.030}
\expandafter\def\csname nv@subd.s2.fa.stdp.V1.hi\endcsname{-0.021}
\expandafter\def\csname nv@subd.s2.fa.stdp.V1.lo\endcsname{-0.039}
\expandafter\def\csname nv@subd.s2.fa.stdp.V2\endcsname{-0.019}
\expandafter\def\csname nv@subd.s2.fa.stdp.V2.hi\endcsname{-0.012}
\expandafter\def\csname nv@subd.s2.fa.stdp.V2.lo\endcsname{-0.027}
\expandafter\def\csname nv@subd.s2.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s2.pc.stdp.IT.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s2.pc.stdp.IT.lo\endcsname{-0.008}
\expandafter\def\csname nv@subd.s2.pc.stdp.LOC\endcsname{+0.001}
\expandafter\def\csname nv@subd.s2.pc.stdp.LOC.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s2.pc.stdp.LOC.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s2.pc.stdp.V1\endcsname{-0.025}
\expandafter\def\csname nv@subd.s2.pc.stdp.V1.hi\endcsname{-0.018}
\expandafter\def\csname nv@subd.s2.pc.stdp.V1.lo\endcsname{-0.033}
\expandafter\def\csname nv@subd.s2.pc.stdp.V2\endcsname{-0.017}
\expandafter\def\csname nv@subd.s2.pc.stdp.V2.hi\endcsname{-0.011}
\expandafter\def\csname nv@subd.s2.pc.stdp.V2.lo\endcsname{-0.023}
\expandafter\def\csname nv@subd.s2.rnd.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@subd.s2.rnd.bp.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@subd.s2.rnd.bp.IT.lo\endcsname{-0.024}
\expandafter\def\csname nv@subd.s2.rnd.bp.LOC\endcsname{-0.024}
\expandafter\def\csname nv@subd.s2.rnd.bp.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@subd.s2.rnd.bp.LOC.lo\endcsname{-0.047}
\expandafter\def\csname nv@subd.s2.rnd.bp.V1\endcsname{+0.052}
\expandafter\def\csname nv@subd.s2.rnd.bp.V1.hi\endcsname{0.076}
\expandafter\def\csname nv@subd.s2.rnd.bp.V1.lo\endcsname{0.026}
\expandafter\def\csname nv@subd.s2.rnd.bp.V2\endcsname{+0.029}
\expandafter\def\csname nv@subd.s2.rnd.bp.V2.hi\endcsname{0.050}
\expandafter\def\csname nv@subd.s2.rnd.bp.V2.lo\endcsname{0.008}
\expandafter\def\csname nv@subd.s2.rnd.fa.IT\endcsname{-0.004}
\expandafter\def\csname nv@subd.s2.rnd.fa.IT.hi\endcsname{0.015}
\expandafter\def\csname nv@subd.s2.rnd.fa.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@subd.s2.rnd.fa.LOC\endcsname{-0.016}
\expandafter\def\csname nv@subd.s2.rnd.fa.LOC.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s2.rnd.fa.LOC.lo\endcsname{-0.034}
\expandafter\def\csname nv@subd.s2.rnd.fa.V1\endcsname{+0.070}
\expandafter\def\csname nv@subd.s2.rnd.fa.V1.hi\endcsname{0.098}
\expandafter\def\csname nv@subd.s2.rnd.fa.V1.lo\endcsname{0.043}
\expandafter\def\csname nv@subd.s2.rnd.fa.V2\endcsname{+0.041}
\expandafter\def\csname nv@subd.s2.rnd.fa.V2.hi\endcsname{0.064}
\expandafter\def\csname nv@subd.s2.rnd.fa.V2.lo\endcsname{0.018}
\expandafter\def\csname nv@subd.s2.rnd.pc.IT\endcsname{-0.003}
\expandafter\def\csname nv@subd.s2.rnd.pc.IT.hi\endcsname{0.016}
\expandafter\def\csname nv@subd.s2.rnd.pc.IT.lo\endcsname{-0.022}
\expandafter\def\csname nv@subd.s2.rnd.pc.LOC\endcsname{-0.017}
\expandafter\def\csname nv@subd.s2.rnd.pc.LOC.hi\endcsname{-0.001}
\expandafter\def\csname nv@subd.s2.rnd.pc.LOC.lo\endcsname{-0.032}
\expandafter\def\csname nv@subd.s2.rnd.pc.V1\endcsname{+0.066}
\expandafter\def\csname nv@subd.s2.rnd.pc.V1.hi\endcsname{0.091}
\expandafter\def\csname nv@subd.s2.rnd.pc.V1.lo\endcsname{0.041}
\expandafter\def\csname nv@subd.s2.rnd.pc.V2\endcsname{+0.039}
\expandafter\def\csname nv@subd.s2.rnd.pc.V2.hi\endcsname{0.059}
\expandafter\def\csname nv@subd.s2.rnd.pc.V2.lo\endcsname{0.017}
\expandafter\def\csname nv@subd.s2.rnd.stdp.IT\endcsname{-0.004}
\expandafter\def\csname nv@subd.s2.rnd.stdp.IT.hi\endcsname{0.012}
\expandafter\def\csname nv@subd.s2.rnd.stdp.IT.lo\endcsname{-0.021}
\expandafter\def\csname nv@subd.s2.rnd.stdp.LOC\endcsname{-0.016}
\expandafter\def\csname nv@subd.s2.rnd.stdp.LOC.hi\endcsname{-0.000}
\expandafter\def\csname nv@subd.s2.rnd.stdp.LOC.lo\endcsname{-0.031}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V1\endcsname{+0.041}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V1.hi\endcsname{0.064}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V1.lo\endcsname{0.016}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V2\endcsname{+0.022}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V2.hi\endcsname{0.042}
\expandafter\def\csname nv@subd.s2.rnd.stdp.V2.lo\endcsname{0.000}
\expandafter\def\csname nv@subd.s3.bp.fa.IT\endcsname{+0.003}
\expandafter\def\csname nv@subd.s3.bp.fa.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s3.bp.fa.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.bp.fa.LOC\endcsname{+0.005}
\expandafter\def\csname nv@subd.s3.bp.fa.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@subd.s3.bp.fa.LOC.lo\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.bp.fa.V1\endcsname{+0.004}
\expandafter\def\csname nv@subd.s3.bp.fa.V1.hi\endcsname{0.009}
\expandafter\def\csname nv@subd.s3.bp.fa.V1.lo\endcsname{0.000}
\expandafter\def\csname nv@subd.s3.bp.fa.V2\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.fa.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s3.bp.fa.V2.lo\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.bp.pc.IT\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.pc.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@subd.s3.bp.pc.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s3.bp.pc.LOC\endcsname{+0.003}
\expandafter\def\csname nv@subd.s3.bp.pc.LOC.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s3.bp.pc.LOC.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s3.bp.pc.V1\endcsname{+0.003}
\expandafter\def\csname nv@subd.s3.bp.pc.V1.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s3.bp.pc.V1.lo\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.bp.pc.V2\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.pc.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s3.bp.pc.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.bp.stdp.IT\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.stdp.IT.hi\endcsname{0.007}
\expandafter\def\csname nv@subd.s3.bp.stdp.IT.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s3.bp.stdp.LOC\endcsname{+0.004}
\expandafter\def\csname nv@subd.s3.bp.stdp.LOC.hi\endcsname{0.012}
\expandafter\def\csname nv@subd.s3.bp.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.bp.stdp.V1\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.stdp.V1.hi\endcsname{0.007}
\expandafter\def\csname nv@subd.s3.bp.stdp.V1.lo\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.bp.stdp.V2\endcsname{+0.002}
\expandafter\def\csname nv@subd.s3.bp.stdp.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s3.bp.stdp.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.fa.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@subd.s3.fa.pc.IT.hi\endcsname{0.005}
\expandafter\def\csname nv@subd.s3.fa.pc.IT.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s3.fa.pc.LOC\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.fa.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s3.fa.pc.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.fa.pc.V1\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.fa.pc.V1.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s3.fa.pc.V1.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.fa.pc.V2\endcsname{-0.000}
\expandafter\def\csname nv@subd.s3.fa.pc.V2.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s3.fa.pc.V2.lo\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.fa.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.fa.stdp.IT.hi\endcsname{0.004}
\expandafter\def\csname nv@subd.s3.fa.stdp.IT.lo\endcsname{-0.007}
\expandafter\def\csname nv@subd.s3.fa.stdp.LOC\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.fa.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s3.fa.stdp.LOC.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.fa.stdp.V1\endcsname{-0.002}
\expandafter\def\csname nv@subd.s3.fa.stdp.V1.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s3.fa.stdp.V1.lo\endcsname{-0.006}
\expandafter\def\csname nv@subd.s3.fa.stdp.V2\endcsname{-0.000}
\expandafter\def\csname nv@subd.s3.fa.stdp.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s3.fa.stdp.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.pc.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.pc.stdp.IT.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s3.pc.stdp.IT.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.pc.stdp.LOC\endcsname{+0.001}
\expandafter\def\csname nv@subd.s3.pc.stdp.LOC.hi\endcsname{0.005}
\expandafter\def\csname nv@subd.s3.pc.stdp.LOC.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.pc.stdp.V1\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.pc.stdp.V1.hi\endcsname{0.001}
\expandafter\def\csname nv@subd.s3.pc.stdp.V1.lo\endcsname{-0.004}
\expandafter\def\csname nv@subd.s3.pc.stdp.V2\endcsname{-0.000}
\expandafter\def\csname nv@subd.s3.pc.stdp.V2.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s3.pc.stdp.V2.lo\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.rnd.bp.IT\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.rnd.bp.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s3.rnd.bp.IT.lo\endcsname{-0.015}
\expandafter\def\csname nv@subd.s3.rnd.bp.LOC\endcsname{-0.008}
\expandafter\def\csname nv@subd.s3.rnd.bp.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s3.rnd.bp.LOC.lo\endcsname{-0.019}
\expandafter\def\csname nv@subd.s3.rnd.bp.V1\endcsname{+0.007}
\expandafter\def\csname nv@subd.s3.rnd.bp.V1.hi\endcsname{0.016}
\expandafter\def\csname nv@subd.s3.rnd.bp.V1.lo\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.rnd.bp.V2\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.rnd.bp.V2.hi\endcsname{0.005}
\expandafter\def\csname nv@subd.s3.rnd.bp.V2.lo\endcsname{-0.008}
\expandafter\def\csname nv@subd.s3.rnd.fa.IT\endcsname{+0.000}
\expandafter\def\csname nv@subd.s3.rnd.fa.IT.hi\endcsname{0.010}
\expandafter\def\csname nv@subd.s3.rnd.fa.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s3.rnd.fa.LOC\endcsname{-0.003}
\expandafter\def\csname nv@subd.s3.rnd.fa.LOC.hi\endcsname{0.004}
\expandafter\def\csname nv@subd.s3.rnd.fa.LOC.lo\endcsname{-0.010}
\expandafter\def\csname nv@subd.s3.rnd.fa.V1\endcsname{+0.012}
\expandafter\def\csname nv@subd.s3.rnd.fa.V1.hi\endcsname{0.020}
\expandafter\def\csname nv@subd.s3.rnd.fa.V1.lo\endcsname{0.004}
\expandafter\def\csname nv@subd.s3.rnd.fa.V2\endcsname{+0.001}
\expandafter\def\csname nv@subd.s3.rnd.fa.V2.hi\endcsname{0.008}
\expandafter\def\csname nv@subd.s3.rnd.fa.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.rnd.pc.IT\endcsname{-0.000}
\expandafter\def\csname nv@subd.s3.rnd.pc.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@subd.s3.rnd.pc.IT.lo\endcsname{-0.009}
\expandafter\def\csname nv@subd.s3.rnd.pc.LOC\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.rnd.pc.LOC.hi\endcsname{0.002}
\expandafter\def\csname nv@subd.s3.rnd.pc.LOC.lo\endcsname{-0.012}
\expandafter\def\csname nv@subd.s3.rnd.pc.V1\endcsname{+0.011}
\expandafter\def\csname nv@subd.s3.rnd.pc.V1.hi\endcsname{0.018}
\expandafter\def\csname nv@subd.s3.rnd.pc.V1.lo\endcsname{0.003}
\expandafter\def\csname nv@subd.s3.rnd.pc.V2\endcsname{+0.001}
\expandafter\def\csname nv@subd.s3.rnd.pc.V2.hi\endcsname{0.007}
\expandafter\def\csname nv@subd.s3.rnd.pc.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@subd.s3.rnd.stdp.IT\endcsname{-0.001}
\expandafter\def\csname nv@subd.s3.rnd.stdp.IT.hi\endcsname{0.009}
\expandafter\def\csname nv@subd.s3.rnd.stdp.IT.lo\endcsname{-0.010}
\expandafter\def\csname nv@subd.s3.rnd.stdp.LOC\endcsname{-0.004}
\expandafter\def\csname nv@subd.s3.rnd.stdp.LOC.hi\endcsname{0.003}
\expandafter\def\csname nv@subd.s3.rnd.stdp.LOC.lo\endcsname{-0.011}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V1\endcsname{+0.009}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V1.hi\endcsname{0.017}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V1.lo\endcsname{0.003}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V2\endcsname{+0.001}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V2.hi\endcsname{0.006}
\expandafter\def\csname nv@subd.s3.rnd.stdp.V2.lo\endcsname{-0.005}
\expandafter\def\csname nv@ub.all.IT\endcsname{0.563}
\expandafter\def\csname nv@ub.all.IT.hi\endcsname{0.566}
\expandafter\def\csname nv@ub.all.IT.lo\endcsname{0.560}
\expandafter\def\csname nv@ub.all.LOC\endcsname{0.566}
\expandafter\def\csname nv@ub.all.LOC.hi\endcsname{0.569}
\expandafter\def\csname nv@ub.all.LOC.lo\endcsname{0.563}
\expandafter\def\csname nv@ub.all.V1\endcsname{0.575}
\expandafter\def\csname nv@ub.all.V1.hi\endcsname{0.581}
\expandafter\def\csname nv@ub.all.V1.lo\endcsname{0.569}
\expandafter\def\csname nv@ub.all.V2\endcsname{0.568}
\expandafter\def\csname nv@ub.all.V2.hi\endcsname{0.572}
\expandafter\def\csname nv@ub.all.V2.lo\endcsname{0.564}
\expandafter\def\csname nv@ub.cr.IT\endcsname{0.556}
\expandafter\def\csname nv@ub.cr.IT.hi\endcsname{0.560}
\expandafter\def\csname nv@ub.cr.IT.lo\endcsname{0.553}
\expandafter\def\csname nv@ub.cr.LOC\endcsname{0.558}
\expandafter\def\csname nv@ub.cr.LOC.hi\endcsname{0.562}
\expandafter\def\csname nv@ub.cr.LOC.lo\endcsname{0.555}
\expandafter\def\csname nv@ub.cr.V1\endcsname{0.572}
\expandafter\def\csname nv@ub.cr.V1.hi\endcsname{0.579}
\expandafter\def\csname nv@ub.cr.V1.lo\endcsname{0.565}
\expandafter\def\csname nv@ub.cr.V2\endcsname{0.563}
\expandafter\def\csname nv@ub.cr.V2.hi\endcsname{0.568}
\expandafter\def\csname nv@ub.cr.V2.lo\endcsname{0.559}
\expandafter\def\csname nv@ub.crb.IT\endcsname{0.556}
\expandafter\def\csname nv@ub.crb.IT.hi\endcsname{0.560}
\expandafter\def\csname nv@ub.crb.IT.lo\endcsname{0.553}
\expandafter\def\csname nv@ub.crb.LOC\endcsname{0.559}
\expandafter\def\csname nv@ub.crb.LOC.hi\endcsname{0.562}
\expandafter\def\csname nv@ub.crb.LOC.lo\endcsname{0.555}
\expandafter\def\csname nv@ub.crb.V1\endcsname{0.572}
\expandafter\def\csname nv@ub.crb.V1.hi\endcsname{0.579}
\expandafter\def\csname nv@ub.crb.V1.lo\endcsname{0.565}
\expandafter\def\csname nv@ub.crb.V2\endcsname{0.564}
\expandafter\def\csname nv@ub.crb.V2.hi\endcsname{0.568}
\expandafter\def\csname nv@ub.crb.V2.lo\endcsname{0.560}
\expandafter\def\csname nv@ubexcess.cr.IT\endcsname{0.010}
\expandafter\def\csname nv@ubexcess.cr.LOC\endcsname{0.008}
\expandafter\def\csname nv@ubexcess.cr.V1\endcsname{0.024}
\expandafter\def\csname nv@ubexcess.cr.V2\endcsname{0.011}
\expandafter\def\csname nv@ubnull.cr.IT.mean\endcsname{0.547}
\expandafter\def\csname nv@ubnull.cr.IT.q\endcsname{0.548}
\expandafter\def\csname nv@ubnull.cr.IT.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.cr.LOC.mean\endcsname{0.550}
\expandafter\def\csname nv@ubnull.cr.LOC.q\endcsname{0.552}
\expandafter\def\csname nv@ubnull.cr.LOC.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.cr.V1.mean\endcsname{0.548}
\expandafter\def\csname nv@ubnull.cr.V1.q\endcsname{0.550}
\expandafter\def\csname nv@ubnull.cr.V1.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.cr.V2.mean\endcsname{0.553}
\expandafter\def\csname nv@ubnull.cr.V2.q\endcsname{0.554}
\expandafter\def\csname nv@ubnull.cr.V2.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.crb.IT.mean\endcsname{0.547}
\expandafter\def\csname nv@ubnull.crb.IT.q\endcsname{0.548}
\expandafter\def\csname nv@ubnull.crb.IT.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.crb.LOC.mean\endcsname{0.550}
\expandafter\def\csname nv@ubnull.crb.LOC.q\endcsname{0.552}
\expandafter\def\csname nv@ubnull.crb.LOC.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.crb.V1.mean\endcsname{0.548}
\expandafter\def\csname nv@ubnull.crb.V1.q\endcsname{0.550}
\expandafter\def\csname nv@ubnull.crb.V1.sd\endcsname{0.001}
\expandafter\def\csname nv@ubnull.crb.V2.mean\endcsname{0.553}
\expandafter\def\csname nv@ubnull.crb.V2.q\endcsname{0.554}
\expandafter\def\csname nv@ubnull.crb.V2.sd\endcsname{0.001}
\expandafter\def\csname nv@v2acc.bp\endcsname{82.4}
\expandafter\def\csname nv@v2acc.fa\endcsname{39.0}
\expandafter\def\csname nv@v2acc.pc\endcsname{56.6}
\expandafter\def\csname nv@v2acc.rnd\endcsname{10.0}
\expandafter\def\csname nv@v2acc.stdp\endcsname{63.2}
\expandafter\def\csname nv@v2c.Conv1.bp.fa\endcsname{+0.0087}
\expandafter\def\csname nv@v2c.Conv1.bp.fa.hi\endcsname{0.0125}
\expandafter\def\csname nv@v2c.Conv1.bp.fa.lo\endcsname{0.0053}
\expandafter\def\csname nv@v2c.Conv1.pc.fa\endcsname{+0.0021}
\expandafter\def\csname nv@v2c.Conv1.pc.fa.hi\endcsname{0.0037}
\expandafter\def\csname nv@v2c.Conv1.pc.fa.lo\endcsname{0.0005}
\expandafter\def\csname nv@v2c.Conv1.rnd.bp\endcsname{+0.0165}
\expandafter\def\csname nv@v2c.Conv1.rnd.bp.hi\endcsname{0.0261}
\expandafter\def\csname nv@v2c.Conv1.rnd.bp.lo\endcsname{0.0072}
\expandafter\def\csname nv@v2c.Conv1.rnd.fa\endcsname{+0.0252}
\expandafter\def\csname nv@v2c.Conv1.rnd.fa.hi\endcsname{0.0361}
\expandafter\def\csname nv@v2c.Conv1.rnd.fa.lo\endcsname{0.0150}
\expandafter\def\csname nv@v2c.Conv1.stdp.fa\endcsname{+0.0110}
\expandafter\def\csname nv@v2c.Conv1.stdp.fa.hi\endcsname{0.0146}
\expandafter\def\csname nv@v2c.Conv1.stdp.fa.lo\endcsname{0.0077}
\expandafter\def\csname nv@v2c.Conv2.bp.fa\endcsname{-0.0213}
\expandafter\def\csname nv@v2c.Conv2.bp.fa.hi\endcsname{-0.0148}
\expandafter\def\csname nv@v2c.Conv2.bp.fa.lo\endcsname{-0.0274}
\expandafter\def\csname nv@v2c.Conv2.pc.fa\endcsname{-0.0005}
\expandafter\def\csname nv@v2c.Conv2.pc.fa.hi\endcsname{0.0027}
\expandafter\def\csname nv@v2c.Conv2.pc.fa.lo\endcsname{-0.0035}
\expandafter\def\csname nv@v2c.Conv2.rnd.bp\endcsname{+0.0526}
\expandafter\def\csname nv@v2c.Conv2.rnd.bp.hi\endcsname{0.0656}
\expandafter\def\csname nv@v2c.Conv2.rnd.bp.lo\endcsname{0.0401}
\expandafter\def\csname nv@v2c.Conv2.rnd.fa\endcsname{+0.0313}
\expandafter\def\csname nv@v2c.Conv2.rnd.fa.hi\endcsname{0.0413}
\expandafter\def\csname nv@v2c.Conv2.rnd.fa.lo\endcsname{0.0212}
\expandafter\def\csname nv@v2c.Conv2.stdp.fa\endcsname{+0.0097}
\expandafter\def\csname nv@v2c.Conv2.stdp.fa.hi\endcsname{0.0152}
\expandafter\def\csname nv@v2c.Conv2.stdp.fa.lo\endcsname{0.0047}
\expandafter\def\csname nv@v2quote.0\endcsname{0.076}
\expandafter\def\csname nv@v2quote.1\endcsname{0.034}
\expandafter\def\csname nv@v2quote.2\endcsname{0.019}
\expandafter\def\csname nv@v2quote.3\endcsname{.023}
\expandafter\def\csname nv@v2quote.4\endcsname{+0.044}
\expandafter\def\csname nv@v2quote.5\endcsname{2.00}
\expandafter\def\csname nv@v2quote.6\endcsname{0.003--0.007}
\expandafter\def\csname nv@v2quote.7\endcsname{30}
\expandafter\def\csname nv@v2quote.8\endcsname{$p \le 0.014$}
\makeatother
\newcommand{\NV}[1]{\ifcsname nv@#1\endcsname\csname nv@#1\endcsname\else\errmessage{Undefined number: #1}\fi}

